Neural Attention Models in Deep Learning: Survey and Taxonomy

Attention is a state of arousal capable of dealing with limited processing bottlenecks in human beings by focusing selectively on one piece of information while ignoring other perceptible information. For decades, concepts and functions of attention have been studied in philosophy, psychology, neuroscience, and computing. Currently, this property has been widely explored in deep neural networks. Many different neural attention models are now available and have been a very active research area over the past six years. From the theoretical standpoint of attention, this survey provides a critical analysis of major neural attention models. Here we propose a taxonomy that corroborates with theoretical aspects that predate Deep Learning. Our taxonomy provides an organizational structure that asks new questions and structures the understanding of existing attentional mechanisms. In particular, 17 criteria derived from psychology and neuroscience classic studies are formulated for qualitative comparison and critical analysis on the 51 main models found on a set of more than 650 papers analyzed. Also, we highlight several theoretical issues that have not yet been explored, including discussions about biological plausibility, highlight current research trends, and provide insights for the future.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> PART_0_APP.tex <==
\section*{Appendix}
\label{sec:systematic_review}

This survey employs a systematic review (SR) approach aiming to collect, critically evaluate, and synthesize the results of multiple primary studies concerning Attention in Deep Learning. The selection and evaluation of the works should be meticulous and easily reproducible. Also, SR should be objective, systematic, transparent, and replicable. Although recent, the use of attention in Deep Learning is extensive. Therefore, we systematically reviewed the literature, collecting works from a variety of sources. SR consists of the following steps: defining the scientific questions, identifying the databases, establishing the criteria for selecting papers, searching the databases, performing a critical analysis to choose the most relevant works, and preparing a critical summary of the most relevant papers, as shown Figure \ref{fig:systematic_review_steps}. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{img/systematic_review.pdf}
  \caption{Steps of the systematic review used in this survey.}
  \label{fig:systematic_review_steps}
\end{figure}

This survey covers the following aspects: 1) The uses of attention in Deep Learning; 2) Attention mechanisms; 3) Uses of attention; 4) A taxonomy for attention models; 5) Attention applications; 6) Attention and interpretability; 7) Trends and challenges. These aspects provide the main topics regarding attention in Deep Learning, which can help understand the field's fundamentals. The second step identifies the main databases in the machine learning area, such as arXiv, DeepMind, Google AI, OpenAI, Facebook AI research, Microsoft research, Amazon research, Google Scholar, IEEE Xplore, DBLP, ACM, NIPS, ICML, ICLR, AAAI, CVPR, ICCV, CoRR, IJCNN, Neurocomputing, and Google general search (including blogs, distill, and Quora). Our searching period comprises 01/01/2014 to 06/30/2019 (first stage) and 07/01/2019 to 02/15/2021 (second stage), and the search was performed via a Phyton script \footnote{Download link: \url{https://github.com/larocs/attention_dl}}. The papers' title, abstract, year, DOI, and source publication were downloaded and stored in a JSON file. The most appropriate set of keywords to perform the searches was defined by partially searching the field with expert knowledge from our research group. The final set of keywords wore: attention, attentional, and attentive. 



However, these keywords are also relevant in psychology and visual attention. Hence, we performed a second selection to eliminate these papers and remmove duplicate papers unrelated to the DL field. After removing duplicates, 18,257 different papers remained. In the next selection step, we performed a sequential combination of three types of filters: 1) Filter I: Selecting the works with general terms of attention (i.e., attention, attentive, attentional, saliency, top-down, bottom-up, memory, focus, and mechanism); 2) Filter II: Selecting the works with terms related to DL (i.e. deep learning, neural network, ann, dnn deep neural, encoder, decoder, recurrent neural network, recurrent network, rnn, long short term memory, long short-term memory, lstm, gated recurrent unit, gru, autoencoder, ae, variational autoencoder, vae, denoising ae, dae, sparse ae, sae, markov chain, mc, hopfield network, boltzmann machine, em, restricted boltzmann machine, rbm, deep belief network, dbn, deep convolutional network, dcn, deconvolution network, dn, deep convolutional inverse graphics network, dcign, generative adversarial network, gan, liquid state machine, lsm, extreme learnng, machine, elm, echo state network, esn, deep residual network, drn, konohen network, kn, turing machine, ntm, convolutional network, cnn, and capsule network); 3) Filter III: Selecting the works with specific words of attention in Deep Learning (i.e., attention network, soft attention, hard attention, self-attention, self attention deep attention, hierarchical attention, transformer, local attention, global attention, coattention, co-attention, flow attention, attention-over-attention, way attention, intra-attention, self-attentive, and self attentive).

The decision tree with the second selection is shown in Figure \ref{fig:filter_papers_steps}. The third filtering selects works with at least one specific term of attention in deep learning. In the next filtering, we remove papers without abstract, the collection of filters verify if there is at least one specific term of Deep Learning and remove the works with the following keywords: visual attention, saliency, and eye-tracking. For the papers with abstract, the selection is more complex, requiring three cascade conditions: 1) First condition: Selecting the works that have more than five filter terms from filter II; 2) Second condition: selecting the works that have between three and five terms from filter II and where there is at least one of the following: attention model, attention mechanism, attention, or attentive; 3) Third condition: Selecting the works with one or two terms from filter II; without the terms: salience, visual attention, attentive, and attentional mechanism. A total of 6,338 works remained for manual selection. We manually excluded the papers without a title, abstract, or introduction related to the DL field. After manual selection, 3,567 works were stored in \textbf {Zotero}. Given the number of papers, we grouped them by year and chose those above a threshold (average citations in the group). Only works above average were read and classified as relevant or not for critical analysis. To find the number of citations, we automated the process with a Python script. 650 papers were considered relevant for this survey's critical analysis, and 6,567 were used to perform quantitative analyzes. 

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{img/systematic_review_tree.pdf}
  \caption{The filter strategies for selecting the relevant works. Search I corresponds to articles collected between 01/01/2014 to 06/30/2019 (first stage), and Search II corresponds to papers collected between 07/01/2019 to 02/15/2021 (second stage).}
  \label{fig:filter_papers_steps}
\end{figure}



==> PART_III_APPLICATIONS.tex <==
%% esther: check 1
\section{Applications}
\label{sec:applications}
In a few years, neural attention networks have been used in numerous domains due to versatility, interpretability, and significance of results. These networks have been explored mainly in computer vision, natural language processing, and multi-modal tasks, as shown in figure \ref{fig:applications}. In some applications, these models transformed the area entirely (i.e., question-answering, machine translation, document representations/embeddings, graph embeddings), mainly due to significant performance impacts on the task in question. In others, they helped learn better representations and deal with temporal dependencies over long distances. This section explores a list of application domains and subareas, mainly discussing each domain's main models and how it benefits from attention. We also present the most representative instances within each area and list them with reference approaches in a wide range of applications. %We mainly describe the following domains: Natural language processing (Section \ref{sec:application_nlp}), computer vision (Section \ref{sec:application_cv}), multimodal tasks (Section \ref{sec:application_cv_nlp}), recommender systems (Section \ref{sec:application_recommender}), robotics (Section \ref{sec:applications_robotics}), and interpretability (Section \ref{sec:applications_interpretability}).%, and others (Section \ref{sec:others}). 



\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.95\textwidth]{img/applications.pdf}
  \caption{Diagram showing the main existing applications of neural attention networks. The main areas are Natural language processing (NLP), Computer Vision (CV), multimodal tasks (mainly with images and texts - CV/NLP), reinforcement learning (RL), robotics, recommendation systems, and others (e.i., graph embeddings, interpretability.).}
  \label{fig:applications}
\end{figure*}

%In each area, the use of attention has different motivations, improving the results of the applications. One of the most significant contributions of attention is the alignment of sentences in machine translation tasks in Natural Language Processing. The main contribution to computer vision is the generation of more robust image classification systems. In robotics, attention can help to improve the ability to handle long-term events. In visual question answering tasks, attention allocates resources correctly to generate words in the most natural way. Besides these examples, there are several benefits of attention in numerous applications in the literature. There is an increasing discussion regarding attention as a tool for interpreting neural networks in a more general contribution. In sections  we present the main references for each application area, the motivations, and contributions of the attention mechanisms in each one of them.

\input{PART_III_subs/nlp}
\input{PART_III_subs/computer_vision}
\input{PART_III_subs/cv_nlp}
\input{PART_III_subs/recommender}
\input{PART_III_subs/rl}
%\input{PART_III_subs/il}
\input{PART_III_subs/robotics}
\input{PART_III_subs/interpretability}
%\input{PART_III_subs/others}


==> PART_III_subs/computer_vision.tex <==
%% esther: check 1

\subsection{Computer Vision (CV)} 
\label{sec:application_cv}

%As tarefas de Visão Computacional envolvem a manipulação de dados de imagens para produzir alguma informação. Atualmente existem várias aplicações que utilizam atenção. A tabela \ref{tab:main_cv_applications} apresenta as principais aplicações existentes, e a tabela \ref{tab:other_cv_application} apresenta aplicações que possuem menos artigos publicados. Em cada aplicação os mecanismos atencionais são utilizados com diferentes propósitos.
Visual attention has become popular in many CV tasks. Action recognition, counting crowds, image classification, image generation, object detection, person recognition, segmentation, saliency detection, text recognition, and tracking targets are the most explored sub-areas, as shown in table \ref{tab:main_cv_app}. Applications in other sub-areas still have few representative works, such as clustering, compression, deblurring, depth estimation, image restoration, among others, as shown in table \ref{tab:other_cv_application}.

%Na classificação de imagens a atenção tem um papel fundamental em fine-grained recognition. Nessa tarefa, existem métodos iterativos que utilizam "glimpses" com redes neurais recorrentes, há também mecanismos feed-forward para aumentar as CNNs e melhorar o resultado da classificação quando as imagens sofrem mudanças bruscas. De modo geral, os mecanismos de atenção atuam descobrindo as partes mais discriminativas de uma imagem a ser processada com mais detalhes, ignorando a confusão e concentrando-se nas características mais distintas. Essas partes são centrais para o reconhecimento refinado, onde a variação entre classes é pequena e a variação entre classes é alta.

Visual attention in \textbf{image classification} tasks was first addressed by Graves et al. \cite{mnih_recurrent_2014}. In this domain, there are sequential approaches inspired by human saccadic movements \cite{mnih_recurrent_2014} and feedforward-augmented structures CNNs (Section \ref{sub:attention_classic_architectures}). The general goal is usually to amplify fine-grained recognition, improve classification in the presence of occlusions, sudden variations in points of view, lighting, and rotation. Some approaches aim to learn to \textit{look} at the most relevant parts of the input image, while others try to discern between discriminating regions through feature recalibration and ensemble predictors via attention. To \textbf{fine-grained recognition}, important advances have been achieved through recurrent convolutional networks in the classification of bird subspecies \cite{fu_look_2017} and architectures trained via RL to classify vehicle subtypes \cite{zhao_deep_2017}.

\begin{table}[!htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{
\begin{tabular*}{\linewidth}{ll}
\hline
\textbf{Task}       & \textbf{References}       \\ \hline

\textbf{Action Recognition} & \begin{tabular}[c]{@{}l@{}} \cite{sharma_action_2015}\cite{girdhar2019video}\cite{girdhar_attentional_2017}\cite{song_end--end_2016}\cite{zhang2018adding}\cite{chen_^2-nets:_2018}\cite{liu_global_2017}\cite{bazzani2016recurrent}\cite{du2017rpan}\cite{li2018videolstm}\\ \cite{ma_attend_2017}\cite{wang_eidetic_2018}\cite{dong_li;ting_yao;ling-yu_duan;tao_mei;yong_rui_unified_2019}\cite{p._zhang;_c._lan;_j._xing;_w._zeng;_j._xue;_n._zheng_view_nodate}\cite{wu_zheng;lin_li;zhaoxiang_zhang;yan_huang;liang_wang_relational_2019}\cite{harshala_gammulle;simon_denman;sridha_sridharan;clinton_fookes_two_2017}\cite{x._wang;_l._gao;_j._song;_h._shen_beyond_2017}\cite{zhaoxuan_fan;xu_zhao;tianwei_lin;haisheng_su_attention-based_2019}\cite{chenyang_si;wentao_chen;wei_wang;liang_wang;tieniu_tan_attention_2019}\\ \cite{swathikiran_sudhakaran;sergio_escalera;oswald_lanz_lsta:_2019}\cite{noauthor_skeleton_nodate} \end{tabular} \\ \hline

\textbf{Counting Crowds}  & \begin{tabular}[c]{@{}l@{}} \cite{liu_decidenet:_2018}\cite{lingbo_liu;hongjun_wang;guanbin_li;wanli_ouyang;liang_lin_crowd_2018}\cite{mohammad_asiful_hossain;mehrdad_hosseinzadeh;omit_chanda;yang_wang_crowd_2019}\cite{youmei_zhang_chunluan_zhou_faliang_chang_alex_c._kot:_multi-resolution_nodate}\cite{ning_liu;yongchao_long;changqing_zou;qun_niu;li_pan;hefeng_wu_adcrowdnet:_2019} \end{tabular} \\ \hline


\textbf{Image Classification}    &                          \begin{tabular}[c]{@{}l@{}} \cite{fu_look_2017}\cite{serra_overcoming_2018}\cite{han_attribute-aware_2019}\cite{sermanet_attention_2014}\cite{hackel_inference_2018}\cite{kang_deep_2018}\cite{mnih_recurrent_2014}\cite{chen_^2-nets:_2018}\cite{ke_sparse_2018}\cite{rodriguez_painless_2018}\\ \cite{wang_residual_2017}\cite{jaderberg_spatial_2015}\cite{seo_hierarchical_2016}\cite{vinyals_matching_2016}\cite{hu_squeeze-and-excitation_2017}\cite{z._wang;_t._chen;_g._li;_r._xu;_l._lin_multi-label_nodate}\cite{irwan_bello;barret_zoph;ashish_vaswani;jonathon_shlens;quoc_v._le_attention_2019}\cite{lin_wu;yang_wang;xue_li;junbin_gao_deep_2019}\cite{bo_zhao;xiao_wu;jiashi_feng;qiang_peng;shuicheng_yan_diversified_2017}\cite{bo_zhao;xiao_wu;jiashi_feng;qiang_peng;shuicheng_yan_diversified_2017}\\ \cite{han-jia_ye;hexiang_hu;de-chuan_zhan;fei_sha_learning_2019}\cite{emanuele_pesce;petros-pavlos_ypsilantis;samuel_withey;robert_bakewell;vicky_goh;giovanni_montana_learning_2019}\cite{xiaoguang_mei;erting_pan;yong_ma;xiaobing_dai;jun_huang;fan_fan;qinglei_du;hong_zheng;jiayi_ma_spectral-spatial_2019}\cite{bin_zhao;xuelong_li;xiaoqiang_lu;zhigang_wang_cnn-rnn_2019}\cite{q._yin;_j._wang;_x._luo;_j._zhai;_s._k._jha;_y._shi_quaternion_2019}\cite{tianjun_xiao;_yichong_xu;_kuiyuan_yang;_jiaxing_zhang;_yuxin_peng;_z._zhang_application_nodate}\cite{hiroshi_fukui;tsubasa_hirakawa;takayoshi_yamashita;hironobu_fujiyoshi_attention_2019}\cite{sanghyun_woo;jongchan_park;joon-young_lee;in_so_kweon_cbam:_2018}\cite{hailin_hu;an_xiao;sai_zhang;yangyang_li;xuanling_shi;tao_jiang;linqi_zhang;lei_zhang;jianyang_zeng_deephint:_2019}\cite{qingji_guan;yaping_huang;zhun_zhong;zhedong_zheng;liang_zheng;yi_yang_diagnose_2018}\\\cite{bei_fang;ying_li;haokui_zhang;jonathan_cheung-wai_chan_hyperspectral_2019}\cite{jianming_zhang;sarah_adel_bargal;zhe_lin;jonathan_br;t;xiaohui_shen;stan_sclaroff_top-down_2018}\cite{w._wang;_w._wang;_y._xu;_j._shen;_s._zhu_attentive_2018}\cite{wonsik_kim;bhavya_goyal;kunal_chawla;jungmin_lee;keunjoo_kwon_attention-based_2018}\cite{mengye_ren;renjie_liao;ethan_fetaya;richard_s._zemel_incremental_2019}\cite{yuxin_peng;xiangteng_he;junjie_zhao_object-part_2018}\cite{qi_wang;shaoteng_liu;jocelyn_chanussot;xuelong_li_scene_2019}\cite{hazel_doughty;walterio_mayol-cuevas;dima_damen_pros_2019}\cite{noauthor_object-part_nodate}\end{tabular}   
\\ \hline

\textbf{Image Generation}  &   
\multicolumn{1}{l}{\begin{tabular}[l]{@{}l@{}}\cite{draw}\cite{zhang2018self}\cite{kastaniotis_attention-aware_2018}\cite{yu_generative_2018}\cite{bornschein2017variational}\cite{reed_few-shot_2017}\cite{parmar2018image}\cite{xinyuan_chen;chang_xu;xiaokang_yang;dacheng_tao_attention-gan_2018}\cite{rewon_child;scott_gray;alec_radford;ilya_sutskever_generating_2019}\cite{jianan_li;jimei_yang;aaron_hertzmann;jianming_zhang;tingfa_xu_layoutgan:_2019}\\
\cite{hao_tang;dan_xu;nicu_sebe;yanzhi_wang;jason_j._corso;yan_yan_multi-channel_2019} \end{tabular}} \\ \hline

\textbf{Object Recognition}  &                          \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\cite{q._chu;_w._ouyang;_h._li;_x._wang;_b._liu;_n._yu_online_nodate}\cite{zheng2017learning}\cite{zhedong_zheng;liang_zheng;yi_yang_pedestrian_2017}\cite{x._liu;_h._zhao;_m._tian;_l._sheng;_j._shao;_s._yi;_j._yan;_x._wang_hydraplus-net:_nodate}\cite{he;_anfeng;luo;_chong;tian;_xinmei;zeng;_wenjun_twofold_2018}\cite{xinlei_chen;li-jia_li;li_fei-fei;abhinav_gupta_iterative_2018}\cite{jianlou_si;honggang_zhang;chun-guang_li;jason_kuen;xiangfei_kong;alex_c._kot;gang_wang_dual_2018}\cite{chunfeng_song;yan_huang;wanli_ouyang;liang_wang_mask-guided_2018}\cite{yi_zhou;ling_shao_viewpoint-aware_2018} \end{tabular}} \\ \hline

\textbf{Object Detection}                               &                          \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\cite{zhang_progressive_2018}\cite{tao_kong;fuchun_sun;wenbing_huang;huaping_liu_deep_2018}\cite{guanbin_li;yukang_gan;hejun_wu;nong_xiao;liang_lin_cross-modal_2019}\cite{shuhan_chen;xiuli_tan;ben_wang;xuelong_hu_reverse_2019}\cite{hao_chen;youfu_li_three-stream_2019}\cite{xudong_wang;zhaowei_cai;dashan_gao;nuno_vasconcelos_towards_2019} \end{tabular}} \\ \hline


\textbf{Person Recognition}      &                          \multicolumn{1}{l}{\begin{tabular}[l]{@{}l@{}}\cite{li_harmonious_2018}\cite{hao_liu;jiashi_feng;meibin_qi;jianguo_jiang;shuicheng_yan_end--end_2017}\cite{xingyu_liao;lingxiao_he;zhouwang_yang;chi_zhang_video-based_2019}\cite{d._chen;_h._li;_t._xiao;_s._yi;_x._wang_video_2018}\cite{l._zhao;_x._li;_y._zhuang;_j._wang_deeply-learned_nodate}\cite{z._zhou;_y._huang;_w._wang;_l._wang;_t._tan_see_nodate}\cite{jing_xu;rui_zhao;feng_zhu;huaming_wang;wanli_ouyang_attention-aware_2018}\cite{shuang_li;slawomir_bak;peter_carr;xiaogang_wang_diversity_2018}\cite{meng_zheng;srikrishna_karanam;ziyan_wu;richard_j._radke_re-identification_2019}\cite{deqiang_ouyang;yonghui_zhang;jie_shao_video-based_2019} \\ \cite{cheng_wang;qian_zhang;chang_huang;wenyu_liu;xinggang_wang_mancs:_2018}\cite{noauthor_jointly_nodate}\cite{noauthor_scan_nodate} \end{tabular}} \\ \hline

\textbf{Segmentation}                                                                                                    &                          
\multicolumn{1}{l}{\begin{tabular}[l]{@{}l@{}}\cite{fu_dual_2018}\cite{li_tell_2018}\cite{ren_end--end_2017}\cite{zhang_deep_2019}\cite{chen_attention_2016}\cite{jetley_learn_2018}\cite{shikun_liu;edward_johns;andrew_j._davison_end--end_2019}\cite{yuhui_yuan;jingdong_wang_ocnet:_2019}\cite{hanchao_li;pengfei_xiong;jie_an;lingxue_wang_pyramid_2018}\cite{xiaowei_hu;chi-wing_fu;lei_zhu;jing_qin;pheng-ann_heng_direction-aware_2019} \\ \cite{z._zeng;_w._xie;_y._zhang;_y._lu_ric-unet:_2019}\cite{b._shuai;_z._zuo;_b._wang;_g._wang_scene_2018}\cite{xinxin_hu;kailun_yang;lei_fei;kaiwei_wang_acnet:_2019}\cite{ozan_oktay;jo_schlemper;loic_le_folgoc;matthew_lee;mattias_heinrich;kazunari_misawa;kensaku_mori;steven_mcdonagh;nils_y_hammerla;bernhard_kainz;ben_glocker;daniel_rueckert_attention_2018}\cite{xueying_chen;rong_zhang;pingkun_yan_feature_2019}\cite{ruirui_li;mingming_li;jiacheng_li;yating_zhou_connection_2019}\cite{shu_kong;charless_c._fowlkes_pixel-wise_2019}\cite{xiaoxiao_li;chen_change_loy_video_2018}\cite{hengshuang_zhao;yi_zhang;shu_liu;jianping_shi;chen_change_loy;dahua_lin;jiaya_jia_psanet:_2018} \end{tabular}} \\ \hline


\textbf{Saliency Detection}  &                   \cite{j._kuen;_z._wang;_g._wang_recurrent_nodate}\cite{nian_liu;junwei_han;ming-hsuan_yang_picanet:_2018}\cite{nian_liu;junwei_han;ming-hsuan_yang_picanet:_2018}\cite{marcella_cornia;lorenzo_baraldi;giuseppe_serra;rita_cucchiara_predicting_2018}\cite{xiaowei_hu;chi-wing_fu;lei_zhu;pheng-ann_heng_sac-net:_2019}                                      \\ \hline

\textbf{Text Recognition}   &    \cite{he_end--end_2018}\cite{cheng_focusing_2017}\cite{canjie_luo;lianwen_jin;zenghui_sun_moran:_2019}\cite{hongtao_xie;shancheng_fang;zheng-jun_zha;yating_yang;yan_li;yongdong_zhang_convolutional_2019}\cite{hui_li;peng_wang;chunhua_shen;guyu_zhang_show_2019}\cite{noauthor_focusing_nodate}             \\ \hline

\textbf{Tracking Targets}   &                            
\multicolumn{1}{l}{\begin{tabular}[l]{@{}l@{}}\cite{fu_dual_2018}\cite{li_tell_2018}\cite{ren_end--end_2017}\cite{zhang_deep_2019}\cite{chen_attention_2016}\cite{jetley_learn_2018}\cite{shikun_liu;edward_johns;andrew_j._davison_end--end_2019}\cite{yuhui_yuan;jingdong_wang_ocnet:_2019}\cite{hanchao_li;pengfei_xiong;jie_an;lingxue_wang_pyramid_2018}\cite{xiaowei_hu;chi-wing_fu;lei_zhu;jing_qin;pheng-ann_heng_direction-aware_2019} \\ \cite{z._zeng;_w._xie;_y._zhang;_y._lu_ric-unet:_2019}\cite{b._shuai;_z._zuo;_b._wang;_g._wang_scene_2018}\cite{xinxin_hu;kailun_yang;lei_fei;kaiwei_wang_acnet:_2019}\cite{ozan_oktay;jo_schlemper;loic_le_folgoc;matthew_lee;mattias_heinrich;kazunari_misawa;kensaku_mori;steven_mcdonagh;nils_y_hammerla;bernhard_kainz;ben_glocker;daniel_rueckert_attention_2018}\cite{xueying_chen;rong_zhang;pingkun_yan_feature_2019} \end{tabular}} \\ \hline
\end{tabular*}
\caption{Summary state-of-art approaches in computer vision sub-areas.}
\label{tab:main_cv_app}
\end{table}




Visual attention also provides significant benefits for \textbf{action recognition} tasks by capturing spatio-temporal relationships. The biggest challenge's classical approaches are capturing discriminative features of movement in the sequences of images or videos. The attention allows the network to focus the processing only on the relevant joints or on the movement features easily. Generally, the main approaches use the following strategies: 1) \textbf{saliency maps}: spatiotemporal attention models learn \textit{where to look} in video directly human fixation data. These models express the probability of saliency for each pixel. Deep 3D CNNs extract features only high saliency regions to represent spatial and short time relations at clip level, and LSTMs expand the temporal domain from few frames to seconds \cite{bazzani2016recurrent}; 2) \textbf{self-attention}: modeling context-dependencies. The person being classified is the Query (Q), and the clip around the person is the memory, represented by keys (K) and values (V) vectors. The network process the query and memory to generate an updated query vector. Intuitively self-attention adds context to other people and objects in the clip to assist in subsequent classification \cite{girdhar2019video}; 3) \textbf{recurrent attention mechanisms}: captures relevant positions of joints or movement features and, through a recurring structure, refines the attentional focus at each time step \cite{liu2017global}\cite{du2017rpan}; and 4) \textbf{temporal attention}: captures relevant spatial-temporal locations \cite{li2018videolstm}\cite{meng2018and}\cite{li2018videolstm}\cite{song_end--end_2016}\cite {xin2016recurrent}\cite {zang2018attention}\cite{pei2017temporal}.
%pega recurrent 



%pega duas de temporal attention
Liu et al. \cite{liu2017global} model is a recurrent attention approach to capturing the person's relevant positions. This model presented a pioneering approach using two layers of LSTMs and the context memory cell that recurrently interact with each other, as shown in figure \ref{fig:cv_apps}a. First, a layer of LSTMs generates an encoding of a skeleton sequence, initializing the context memory cell. The memory representation is input to the second layer of LSTMs and helps the network selectively focus on each frame's informational articulations. Finally, attentional representation feeds back the context memory cell to refine the focus's orientation again by paying attention more reliably.
Similarly, Du et al. \cite{du2017rpan} proposed RPAN - a recurrent attention approach between sequentially modeling by LSTMs and convolutional features extractors. First, CNNs extract features from the current frame, and the attentional mechanism guided by the LSTM's previous hidden state estimates a series of features related to human articulations related to the semantics of movements of interest. Then, these highly discriminative features feed LSTM time sequences.

\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{img/computer_vision_apps.pdf}  
  \caption{Illustration of Global Context-Aware Attention \cite{liu2017global} for action recognition, and DRAW \cite{draw} for image generation. a) The Context-Aware Attention Network. The first LSTM layer encodes the skeleton sequence and generates an initial global context memory. The second layer performs attention over the inputs with global context memory assistance and generates a refined representation. The refine representation is then used back to the global context. Multiple attention iterations are carried out to refine the global context progressively. Finally, memory information is used for classification. b) The DRAW architecture. At each time step $t$, the input is read by attention and passed to the encoder RNN. The encoder's output is used to compute the approximate posterior over the latent variables. On the right, an illustration shows the iterative process of generating some images. Each row shows successive stages in the generation of a single digit. The network guided by attention draws and refine regions successively. The red rectangle delimits the area attended to by the network at each time-step.}
  \label{fig:cv_apps}
\end{figure}










%No reconhecimento de ações a atenção ajuda a eliminar distrações em vídeos e imagens capturando dinamicamente relações espaço-temporais entre os dados. Para isso, existem abordagens utilizando diretamente mapas de saliência que aprendem as fixações humanas \cite{bazzani2016recurrent} \cite{wang2016beyond}, blocos de atenção dupla \cite{chen20182}, arquiteturas atencionais completas baseadas na Transformer \cite{girdhar2019video}, attentional pooling \cite{girdhar2017attentional}, recurrent attention mechanism \cite{liu2017skeleton}, motion-based attention \cite{li2018videolstm}, global context-Aware attention \cite{liu2017global}, soft temporal attention \cite{meng2018and}, temporal attention-gated \cite{pei2017temporal}, soft attention \cite{sharma2015action}, spatio-temporal attention \cite{song2017end}, gate-controlled self-attention \cite{wang2018eidetic}, temporal attention \cite{xin2016recurrent}, attention-based temporal weighted \cite{zang2018attention}, element-wise-attention gate \cite{zhang2018adding} e pose-attention \cite{du2017rpan}.




%No problema de síntese de imagens as redes adversariais generativas (GANs) são bem-sucedidas. No entanto, as amostras geradas por esses modelos tem bastante dificuldade para modelar algumas classes de imagem que outras, quando treinados em conjuntos de dados de várias classes. Normalmente as GANs se destacam na síntese de classes de imagens com poucas restrições estruturais, por exemplo, na geração do oceano, céu e paisagens naturais. Esses elementos se distinguem mais pela textura que pela geometria, falhando na captura de padrões geométricos ou estruturais que existem em algumas classes. O que ocorre é que as arquiteruras tradicionais dependem da convolução para modelar as dependências entre diferentes regiões da imagem. Assim, longas dependências só podem ser processadas após a passagem de várias camadas convolucionais. Isso pode impedir o aprendizado sobre dependências de longo prazo porque um modelo pequeno pode não ser capaz de representá-los, e os algoritmos de otimização podem não conseguir convergir completamente utilizando modelos complexos. Além disso, aumentar o tamanho dos kernels de convolução pode aumentar a capacidade representacional da rede, mas diminuir a eficiência computacional e estatística do modelo. Nesse sentido, os mecanimos de atenção, com especial ênfase no mecanimo self-attention, oferecem um melhor equilíbrio entre a capacidade de modelar dependências de longo alcance e a eficiência computacional e estatística. Tornando possível a geração de imagens nos quais detalhes finos são bem desenhados.


In \textbf{image generation}, there were also notable benefits. DRAW \cite{draw} introduced visual attention with an innovative approach - image patches are generated sequentially and gradually refined, in which to generate the entire image in a single pass (figure \ref{fig:cv_apps}b). Subsequently, attentional mechanisms emerged in generative adversarial networks (GANs) to minimize the challenges in modeling images with structural constraints. Naturally, GANs efficiently synthesize elements differentiated by texture (i.e., oceans, sky, natural landscapes) but suffer to generate geometric patterns (i.e., faces, animals, people, fine details). The central problem is the convolutions that fail to model dependencies between distant regions. Besides, the statistical and computational efficiency of the model suffers from the stacking of many layers. The attentional mechanisms, especially self-attention, offered a computationally inexpensive alternative to model long-range dependencies easily. Self-attention as a complement to convolution contributes significantly to the advancement of the area with approaches capable of generating fine details \cite{zhang2018self}, high-resolution images, and with intricate geometric patterns \cite{chen2020generative}.


\begin{table}[htb]
\tiny
\fontfamily{pcr}\selectfont
\textcolor{tabgrey}{

\begin{tabular*}{\linewidth}{lll}
\hline
\textbf{Task}           & \textbf{References}                                     \\ \hline
\textbf{Clustering}    & \begin{tabular}[c]{@{}l@{}} \cite{lee2018set} \end{tabular} \\ \hline

\textbf{Compression}    &  \cite{meng2018mganet}   \\\hline


\textbf{Deblurring}   &  \cite{park2019down}  \\ \hline


\textbf{Depth Estimation}         &  \cite{xu2018structured}\cite{liu2019end}  \\ \hline


\textbf{Image Restoration}      &   \cite{zhang2019residual}\cite{suganuma2019attention}\cite{qian2018attentive}                                                      \\ \hline


\textbf{Image-to-Image Translation}      & \cite{mejjati2018unsupervised}\cite{tang2019attention} \\ \hline


\textbf{Information Retriever}        & \cite{ji2018stacked}\cite{jin2018deep}\cite{yang2019deep} \\ \hline


\textbf{Medical Image Analysis}    &             \cite{kastaniotis_attention-aware_2018}\cite{schlemper_attention_2018}\cite{huiyan_jiang;tianyu_shi;zhiqi_bai;liangliang_huang_ahcnet:_2019}                                   \\ \hline


\textbf{Multiple Instance Learning}     &    \cite{ilse2018attention}    \\ \hline


\textbf{Ocr}      &                 \cite{lee2016recursive}                 \\ \hline

\textbf{One-Shot Learning}     &                 \cite{rezende2016one}                                    \\ \hline


\textbf{Pose Estimation}    &                 \cite{chu2017multi}                                    \\ \hline


\textbf{Super-Resolution}      &                   \cite{zhang2018image}                  \\ \hline


\textbf{Transfer Learning}     &                   \cite{zagoruyko_paying_2016}\cite{xiao-yu_zhang;haichao_shi;changsheng_li;kai_zheng;xiaobin_zhu;lixin_duan_learning_2019}\cite{xingjian_li;haoyi_xiong;hanchao_wang;yuxuan_rao;liping_liu;jun_huan_delta:_2019}                                      \\ \hline


\textbf{Video Classification}     &                   \cite{bielski2018pay}\cite{long2018attention}        \\ \hline


\textbf{Facial Detection}      &                   \cite{tian2018learning}\cite{yundong_zhang;xiang_xu;xiaotao_liu_robust_2019}\cite{shengtao_xiao;jiashi_feng;junliang_xing;hanjiang_lai;shuicheng_yan;ashraf_a._kassim_robust_2016}                                      \\ \hline


\textbf{Fall Detection}   &                   \cite{lu2018deep}                                      \\ \hline


\textbf{Person Detection}      &                   \cite{zhang2019cross}\cite{zhang2018occluded}         \\ \hline


\textbf{Sign Detection}    &                   \cite{yuan2019vssa}                                      \\ \hline


\textbf{Text Detection}   &                   \cite{he_end--end_2018}\cite{wojna_attention-based_2017}\cite{he_single_2017}\cite{bhunia_script_2019}                                      \\ \hline


\textbf{Face Recognition}     &                   \cite{yang2017neural}                 \\ \hline



\textbf{Facial Expression Recognition}   &                   \cite{siyue_xie;haifeng_hu;yongbo_wu_deep_2019}\cite{shervin_minaee;amirali_abdolrashidi_deep-emotion:_2019}\cite{yong_li;jiabei_zeng;shiguang_shan;xilin_chen_occlusion_2019} \\ \hline


\textbf{Sequence Recognition}        &                   \cite{yang2019fully}                                    \\ \hline

\end{tabular(}
}
\caption{Summary others applications of attention in computer vision.}
\label{tab:other_cv_application}
\end{table}


In \textbf{expression recognition}, attention optimizes the entire segmentation process by scanning input as a whole sequence, choosing the most relevant region to describe a segmented symbol or implicit space operator \cite{zhang2017gru}. In \textbf{information retriever}, attention helps obtain appropriate semantic resources using individual class semantic resources to progressively orient visual aids to generate an attention map to ponder the importance of different local regions. \cite{ji2018stacked}.  


In \textbf{medical image analysis}, attention helps implicitly learn to suppress irrelevant areas in an input image while highlighting useful resources for a specific task. This allows us to eliminate the need to use explicit external tissue/organ localization modules using convolutional neural networks (CNNs). Besides, it allows generating both images and maps of attention in unsupervised learning useful for data annotation. For this, there are the ATA-GANS \cite{kastaniotis_attention-aware_2018} and attention gate \cite{schlemper_attention_2018} modules that work with unsupervised and supervised learning, respectively.





%Em Tracking Targets as aplicações estão voltadas para person-recognition (re-id). Re-id visa procurar pessoas vistas a partir de uma câmera de vigilância implantadas em locais diferentes. O principal problema dessa área é que as caixas delimitadoras das pessoas detectadas automaticamente não são otimizadas para re-identificação devido ao desalinhamento e desordem do fundo, oclusão e partes do corpo ausentes. Além disso, as pessoas são frequentemente capturadas em várias poses, dando origem ao desafio de desalinhamento da imagem para comparação e rei-identificação. Consequentemente surge a necessidade de utilizar atenção dentro das caixas delimitadoras é inevitável para promover o alinhamento automático entre as imagens.

For \textbf{person recognition}, attention has become essential in in-person re-identification (re-id) \cite{han_attribute-aware_2019} \cite{ meng_zheng;srikrishna_karanam;ziyan_wu;richard_j._radke_re-identification_2019} \cite{li_harmonious_2018}. Re-id aims to search for people seen from a surveillance camera implanted in different locations. In classical approaches, the bounding boxes of detected people were not optimized for re-identification suffering from misalignment problems, background disorder, occlusion, and absent body parts. Misalignment is one of the biggest challenges, as people are often captured in various poses, and the system needs to compare different images. In this sense, neural attention models started to lead the developments mainly with multiple attentional mechanisms of alignment between different bounding boxes. 


There are still less popular applications, but for which attention plays an essential role. Self-attention models iterations between the input set for clustering tasks \cite{lee2018set}. Attention refines and merges multi-scale feature maps in-depth estimation and edge detection \cite {xu2017learning}\cite{xu2018structured}. In video classification, attention helps capture global and local resources generating a comprehensive representation \cite{xie2019semantic}. It also measures each time interval's relevance in a sequence \cite{pei2017temporal}, promoting a more intuitive interpretation of the impact of content on the video's popularity, providing the regions that contribute the most to the prediction \cite{bielski2018pay}. In face detection, attention dynamically selects the main reference points of the face \cite{shengtao_xiao;jiashi_feng;junliang_xing;hanjiang_lai;shuicheng_yan;ashraf_a._kassim_robust_2016}. It improves deblurring in each convolutional layer in deblurring, preserving fine details \cite{park2019down}. Finally, in emotion recognition, it captures complex relationships between audio and video data by obtaining regions where both signals relate to emotion \cite{zhang2019deep}.




%Existem ainda aplicações menos propulares na literatura, mas que a atenção desempenha um papel essencial: em Clustering atenção modela iterações entre os conjuntos de entrada. Para isso, existe uma abordagem baseada em self-attention, uma modificação da arquitetura clássica Transformer \cite{lee2018set}. Em Depth Estimation ela regula a quantidade de informação transferida entre features correspondentes em diferentes escalas \cite{xu2018structured}. Em Edge Detection ela refina e funde os multi-scale feature maps de forma robusta \cite{xu2017learning}. Na detecção de Faces o principal papel da atenção é selecionar de forma adaptativa os principais pontos de referência da face \cite{xiao2016robust}. Em Deblurring ela Melhora o resultado do deblurring em cada escala da rede convolucional, preservando detalhes finos da imagem \cite{park2019down}. Em Emotion Recognition: ela captura relações complexas entre dados de aúdio e vídeo obtendo regiões de ambos os sinais relacionados a emoção \cite{zhang2019deep}.



%Em aplicações de reconhecimento de expressões a atenção otimiza todo o processo de segmentação varrendo toda a sequência de entrada e escolhendo a região mais relevante para descrever um símbolo segmentado ou operador espacial implícito \cite{zhang2017gru}. Em information retriever a atenção ajuda a obter recursos semânticos relevantes usando recursos semânticos de classe individual para orientar progressivamente os recursos visuais para gerar um mapa de atenção para ponderar a importância de diferentes regiões locais. \cite{ji2018stacked}. E na análise de imagens médicas a atenção ajuda a aprender implicitamente a suprimir regiões irrelevantes em uma imagem de entrada enquanto destacam recursos úteis para uma tarefa específica. Isso nos permite eliminar a necessidade de usar módulos explícitos externos de localização de tecidos/órgãos utilizando redes neurais convolucionais (CNNs). Além disso, no aprendizado não-supervisionado permite gerar tanto imagens quanto mapas de atenção que são úteis para a anotação de dados. Para isso, existem os módulos de atenção Teacher-Network \cite{kastaniotis2018attention} e attention gate \cite{schlemper2019attention} que trabalham com aprendizado supervisionado e não supervisionado, respectivamente.




%Além dessas aplicações em vídeo classification a atenção ajuda a capturar a recursos globais e locais gerando uma abrangente representação para o vídeo \cite{xie2019semantic}. Medir a relevância de cada intervalo de tempo de uma sequência \cite{pei2017temporal}. Promover uma interpretação mais intuitiva do impacto do conteúdo na popularidade do vídeo, fornecendo as regiões que contribuem mais para a predição \cite{bielski2018pay}. Propor uma estrutura de integração de features locais \cite{long2018attention}.



    
   


==> PART_III_subs/cv_nlp.tex <==
%% esther: check 1

\subsection{Multimodal Tasks (CV/NLP)}
\label{sec:application_cv_nlp}

Attention has been used extensively in multimodal learning, mainly for mapping complex relationships between different sensory modalities. In this domain, the importance of attention is quite intuitive, given that communication and human sensory processing are completely multimodal. The first approaches emerged from 2015 inspired by an attentive encoder-decoder framework entitled ``Show, attend and tell: Neural image caption generation with visual attention'' by Xu et al. \cite{xu_show_2015}. In this framework, depicted in figure \ref{fig:multimodal_apps}a at each time step $t$, attention generates a vector with a dynamic context of visual features based on the words previously generated - a principle very similar to that presented in RNNSearch \cite{bahdanau_neural_2014}. Later, more elaborate methods using visual and textual sources were developed mainly in image captioning, video captioning, and visual question answering, as shown in the table \ref{table:cv_nlp_applications}.

\begin{table}[htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{

\begin{tabular*}{\linewidth}{ll}
\hline
\textbf{Task}  & \textbf{References}  \\ \hline

\textbf{Emotion Recognition} & \cite{tan2019multimodal}\cite{zadeh2018memory}\cite{zadeh2018multi} \\ \hline


\textbf{Expression Comprehension} & \cite{yu2018mattnet}     \\ \hline

\textbf{Image Classification} & \cite{wang2018tienet}     \\ \hline

\textbf{Text-to-Image Generation} & \cite{xu2018attngan}     \\ \hline

\textbf{Image-to-Text Generation} & \cite{poulos2017character}     \\ \hline

\textbf{Image Captioning}  & \begin{tabular}[c]{@{}l@{}} \cite{noauthor_bottom-up_nodate}\cite{zhu_image_2018}\cite{xu_show_2015}\cite{ma_da-gan:_2018-1}\cite{lu_knowing_2017}\cite{you_image_2016}\cite{chen_sca-cnn:_2017}\cite{he_vd-san:_2019}\\ \cite{noauthor_bi-directional_nodate}\cite{fang_captions_2015}\cite{yang_review_2016}\cite{pedersoli_areas_2016}\cite{ting_yao;yingwei_pan;yehao_li;tao_mei_exploring_2018}\cite{yehao_li;ting_yao;yingwei_pan;hongyang_chao;tao_mei_pointing_2019}\cite{x._liang;_z._hu;_h._zhang;_c._gan;_e._p._xing_recurrent_nodate}\cite{xiangrong_zhang;xin_wang;xu_tang;huiyu_zhou;chen_li_description_2019}\cite{anna_rohrbach;marcus_rohrbach;ronghang_hu;trevor_darrell;bernt_schiele_grounding_2017}\\ \cite{lukasz_kaiser;aidan_n._gomez;noam_shazeer;ashish_vaswani;niki_parmar;llion_jones;jakob_uszkoreit_one_2017}\cite{kuang-huei_lee;xi_chen;gang_hua;houdong_hu;xiaodong_he_stacked_2018}\cite{pan2020x}\cite{noauthor_bottom-up_nodate} \end{tabular} 
\\ \hline                                  


\textbf{Video Captioning}   & 
\begin{tabular}[c]{@{}l@{}}\cite{cho_describing_2015}\cite{wu_hierarchical_2018}\cite{zhou2018end}\cite{zhu2020actbert}\cite{pu_adaptive_2018}\cite{yao_describing_2015}\cite{yu_video_2015}\cite{hori_attention-based_2017}\cite{krishna_dense-captioning_2017} \\\cite{ma_attend_2017}\cite{yi_bin;yang_yang;fumin_shen;ning_xie;heng_tao_shen;xuelong_li_describing_2019}\cite{zhou2018end}\cite{l._baraldi;_c._grana;_r._cucchiara_hierarchical_nodate}\cite{silvio_olivastri;gurkirt_singh;fabio_cuzzolin_end--end_2019}\cite{zhong_ji;kailin_xiong;yanwei_pang;xuelong_li_video_2018}\cite{jingkuan_song;zhao_guo;lianli_gao;wu_liu;dongxiang_zhang;heng_tao_shen_hierarchical_2017}\cite{xiangpeng_li;zhilong_zhou;lijiang_chen;lianli_gao_residual_2019}\cite{lianli_gao;zhao_guo;hanwang_zhang;xing_xu;heng_tao_shen_video_2017}\\
\cite{jingwen_wang;wenhao_jiang;lin_ma;wei_liu;yong_xu_bidirectional_2018} \end{tabular} \\ \hline
\textbf{Visual Question Answering}  & \begin{tabular}[c]{@{}l@{}} \cite{kim2020modality}\cite{jiangfantastic}\cite{liang_focal_2018}\cite{hudson_compositional_2018}\cite{gulcehre_hyperbolic_2018}\cite{osman_dual_2018}\cite{lu_hierarchical_2016}\\ \cite{nam_dual_2017}\cite{deng_latent_2018}\cite{kim_bilinear_2018}\cite{nguyen_improved_2018}\cite{andreas_deep_2015}\cite{kim_multimodal_2016}\cite{shih_where_2015}\cite{xiong_dynamic_2016}\cite{zhu_visual7w:_2015}\\ \cite{jiasen_lu;anitha_kannan;jianwei_yang;devi_parikh;dhruv_batra_best_2017}\cite{zhou_yu;jun_yu;chenchao_xiang;jianping_fan;dacheng_tao_beyond_2019}\cite{aishwarya_agrawal;dhruv_batra;devi_parikh;aniruddha_kembhavi_dont_2018}\cite{yan_zhang;jonathon_hare;adam_prugel-bennett_learning_2018}\cite{zhe_gan;yu_cheng;ahmed_el_kholy;linjie_li;jingjing_liu;jianfeng_gao_multi-step_2019}\cite{kan_chen;jiang_wang;liang-chieh_chen;haoyuan_gao;wei_xu;ram_nevatia_abc-cnn:_2016}\cite{huijuan_xu;kate_saenko_ask;_2016}\cite{yundong_zhang;juan_carlos_niebles;alvaro_soto_interpretable_2019}\cite{zheng_zhang;lizi_liao;minlie_huang;xiaoyan_zhu;tat-seng_chua_neural_2019}\\ \cite{noauthor_focal_nodate}\cite{kim2020hypergraph}\cite{yang_stacked_2016}\cite{yu_multi-level_2017}\cite{noauthor_bottom-up_nodate}\cite{z._yu;_j._yu;_j._fan;_d._tao_multi-modal_nodate}\end{tabular} 
\\ \hline
\end{tabular*}
\caption{Summary of state-of-art approaches in multimodal tasks (CV/NLP).}
\label{table:cv_nlp_applications}
\end{table}


For image captioning, Yan et al. \cite{yang_review_2016} extended the seminal framework by Xu et al. \cite{xu_show_2015} with review attention, a sequence of modules that capture global information in various stages of reviewing hidden states and generate more compact, abstract, and global context vectors.
Zhu et al. \cite{zhu_image_2018} presented a triple attention model which enhances object information at the text generation stage. Two attention mechanisms capture semantic visual information in input, and a mechanism in the prediction stage integrates word and image information better. Lu et al. \cite{lu_knowing_2017} presented an adaptive attention encoder-decoder framework that decides when to trust visual signals and when to trust only the language model. Specifically, their mechanism has two complementary elements: the \textit{visual sentinel} vector decides when to look at the image, and the \textit{sentinel gate} decides how much new information the decoder wants from the image. Recently, Pan et al. \cite{pan2020x} created attentional mechanisms based on bilinear pooling capable of capturing high order interactions between multi-modal features, unlike the classic mechanisms that capture only first-order feature interactions.

Similarly, in visual question-answering tasks, methods seek to align salient textual features with visual features via feedforward or recurrent soft attention methods \cite{noauthor_bottom-up_nodate}\cite{osman_dual_2018}\cite{lu_hierarchical_2016}\cite{yang_stacked_2016}. More recent approaches aim to generate complex inter-modal representations. In this line, Kim et al. \cite{kim2020hypergraph} proposed Hypergraph Attention Networks (HANs), a solution to minimize the disparity between different levels of abstraction from different sensory sources. So far, HAN is the first approach to define a common semantic space with symbolic graphs of each modality and extract an inter-modal representation based on co-attention maps in the constructed semantic space, as shown in figure \ref{fig:multimodal_apps}b. Liang et al. \cite{liang_focal_2018} used attention to capture hierarchical relationships between sequences of image-text pairs not directly related. The objective is to answer questions and justify what results in the system were based on answers.

For video captioning most approaches generally align textual features and spatio-temporal representations of visual features via simple soft attention mechanisms \cite{cho_describing_2015} \cite{yu_video_2015} \cite{yao_describing_2015} \cite{hori_attention-based_2017}. For example, Pu et al. \cite{pu_adaptive_2018} design soft attention to adaptively emphasize different CNN layers while also imposing attention within local spatiotemporal regions of the feature maps at particular layers. These mechanisms define the importance of regions and layers to produce a word based on word-history information. Recently, self-attention mechanisms have also been used to capture more complex and explicit relationships between different modalities. Zhu et al. \cite{zhu2020actbert} introduced ActBERT, a transformer-based approach trained via self-supervised learning to encode complex relations between global actions and local, regional objects and linguistic descriptions. Zhou et al. \cite{zhou2018end} proposed a multimodal transformer via supervised learning, which employs a masking network to restrict its attention to the proposed event over the encoding feature.

\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{img/multimodal_apps.pdf}  
  \caption{Illustration of classic attentive encoder-decoder framework by Xu et al. \cite{xu_show_2015} and Hypergraph Attention Network \cite{kim2020hypergraph} for question answering tasks. a) The \textit{show, attend and tell} framework. At each time step $t$, attention takes as input visual feature maps and previous hidden state of the decoder and produces a dynamic context vector with essential visual features to predict the next word. b) The Hypergraph Attention Network. For a given pair of images and questions, two symbolic graphs $G_{i}$, and $G_{q}$ are constructed. After, two hypergraphs $HG_{i}$, and $HG_{q}$ with random-walk hyperedge are constructed and combined via co-attention map $A$. Finally, the final representation $Z_{s}$ is used to predict an answer for the given question.}
  \label{fig:multimodal_apps}
\end{figure}


Other applications also benefit from the attention. In the emotion recognition domain, the main approaches use memory fusion structures inspired by the human brain's communication understanding mechanisms. Biologically, different regions process and understand different modalities connected via neural links to integrate multimodal information over time. Similarly, in existing approaches, an attentional component models view-specific dynamics within each modality via recurrent neural networks, and a second component simultaneously finds multiple cross-view dynamics in each recurrence timestep by storing them in hybrid memories. Memory updates occur based on all the sequential data seen. Finally, to generate the output, the predictor integrates the two levels of information: view-specific and multiple cross-view memory information \cite{zadeh2018memory} \cite{zadeh2018multi}.


There are still few multimodal methods for classification. Whang et al. \cite{wang2018tienet} presented a pioneering framework for classifying and describing image regions simultaneously from textual and visual sources. Their framework detects, classifies, and generates explanatory reports regarding abnormalities observed in chest X-ray images through multi-level attentional modules end-to-end in LSTMs and CNNs. In LSTMs, attention combines all hidden states and generates a dynamic context vector, then a spatial mechanism guided by a textual mechanism highlights the regions of the image with more meaningful information. Intuitively, the salient features of the image are extracted based on high-relevance textual regions.


















==> PART_III_subs/il.tex <==
%% esther: check 1

\subsubsection{\textbf{Imitation Learning}} 
\label{sec:application_imitation}
%falar mais sobre a relacao entre imitation e RL

Usually, imitation learning is applied to solve isolated tasks, including manual work and a significant number of samples. One of the challenges is learning with a few samples and generalizing the model to new situations of the same task without requiring specific tasks. In this sense, attention proved to be a useful tool for generalizing the model in a meta-learning structure in \cite{duan2017one}. Despite the good results of this work, there are no other relevant literature approaches that involve attention and learning by imitation, demonstrating to be a good field for the development of new research.

==> PART_III_subs/interpretability.tex <==
%% esther: check 1

\subsection{\textbf{Interpretability}}
\label{sec:applications_interpretability}

A long-standing criticism of neural network models is
their lack of interpretability. Academia and industry have a great interest in the development of interpretable models mainly for the following aspects: 1) \textbf{critical decisions}: when critical decisions need to be made (e.i., medical analysis, stock market, autonomous cars), it is essential to provide explanations to increase the confidence of the specialist human results; 2) \textbf{failure analysis}: an interpretable model can retrospectively inspect where bad decisions were made and understand how to improve the system; 3) \textbf{verification}: there is no evidence of the models' robustness and convergence even with small errors in the test set. It is difficult to explain the influence of spurious correlations on performance and why the models are sometimes excellent in some test cases and flawed in others; and 4) \textbf{model improvements}: interpretability can guide improvements in the model's structure if the results are not acceptable.

Attention as an interpretability tool is still an open discussion. For some researchers, it allows to inspect the models' internal dynamics -- the hypothesis is that the attentional weights' magnitude is correlated with the data's relevance for predicting the output. Li et al. \cite{li2016understanding} proposed a general methodology to analyze the effect of erasing particular representations of neural networks' input. When analyzing the effects of erasure, they found that attentional focuses are essential to understand networks' internal functioning. In \cite{serrano2019attention} the results showed that higher attentional weights generally contribute with more significant impact to the model's decision, but multiple weights generally do not fully identify the most relevant representations for the final decision. In this investigation, the researchers concluded that attention is an ideal tool to identify which elements are responsible for the output but do not yet fully explain the model's decisions. 

Some studies have also shown that attention encodes linguistic notions relevant to understanding NLP models \cite{vig2019analyzing} \cite{tenney2019bert} \cite{clark2019does}. However, Jain et al. \cite{attention_is_not_explanation} showed that although attention improves NLP results, its ability to provide transparency or significant explanations for the model's predictions is questionable. Specifically, the researchers investigated the relationship between attentional weights and model results by answering the following questions: (i) to what extent do weights of attention correlate with metrics of the importance of features, specifically those resulting from gradient? Moreover, (ii) do different attentional maps produce different predictions? The results showed that the correlation between intuitive metrics about the features' importance (e.i., gradient approaches, erasure of features) and attentional weights is low in recurrent encoders. Besides, the selection of features other than the attentional distribution did not significantly impact the output as attentional weights exchanged at random also induced minimal output changes. The researchers also concluded that such results depend significantly on the type of architecture, given that feedforward encoders obtained more coherent relationships between attentional weights and output than other models.


Vashishth et al. \cite{vashishth2019attention} systematically investigated explanations for the researchers' distinct views through experiments on NLP tasks with single sequence models, pair sequence models, and self-attentive neural networks. The experiments showed that attentional weights in single sequences tasks work like gates and do not reflect the reasoning behind the model's prediction, justifying the observations made by Jain et al. \cite{attention_is_not_explanation}. However, for pair sequence tasks, attentional weights were essential to explaining the model's reasoning. Manual tests have also shown that attentional weights are highly similar to the manual assessment of human observers' attention. Recently, Wiegreffe et al. \cite{wiegreffe2019attention} also investigated these issues in depth through an extensive protocol of experiments. The authors observed that attention as an explanation depends on the definition of explainability considered. If the focus is on plausible explainability, the authors concluded that attention could help interpret model insights. However, if the focus is a faithful and accurate interpretation of the link that the model establishes between inputs and outputs, results are not always positive. These authors confirmed that good alternatives distributions could be found in LSTMs and classification tasks, as hypothesized by Jain et al. \cite{attention_is_not_explanation}. However, in some experiments, adversarial training's alternative distributions had poor performances concerning attention's traditional mechanisms. These results indicate that the attention mechanisms trained mainly in RNNs learn something significant about the relationship between tokens and prediction, which cannot be easily hacked. In the end, they showed that attention efficiency as an explanation depends on the data set and the model's properties.
















==> PART_III_subs/nlp.tex <==
%% esther: check 1

\subsection{\textbf{Natural Language Processing (NLP)}}
\label{sec:application_nlp}

%As tarefas de NLP envolvem a geração de texto ou aúdio em linguagem natural como resultado. Como ilustra a Figura \ref{fig:applications} praticamente todas as subáreas desse domínio se beneficiam com o uso de mecanismos atencionais. No entanto, existem mais aplicações em tarefas de Language Modeling, Machine Translation, Natural Language Inference, Question Answering, sentiment analysis, semantic analysis, speech recognition, and text summarization (Table \ref{tab:main_nlp_applications}). Existem ainda outras aplicações em menor escala na área que também utilizam atenção, elas são descritas na Tabela \ref{tab:others_nlp_applications}.

In the NLP domain, attention plays a vital role in many sub-areas, as shown in figure \ref{fig:applications}. There are several state-of-the-art approaches, mainly in language modeling, machine translation, natural language inference, question answering, sentiment analysis, semantic analysis, speech recognition, and text summarization. Table \ref{tab:main_nlp_app} groups works developed in each of these areas. Several applications have been facing an increasing expansion, with few representative works, such as emotion recognition, speech classification, sequence prediction, semantic matching, and grammatical correction, as shown in table \ref{tab:others_nlp_applications}.


%\begin{table}\centering
%\ra{1.3}
%\tiny
%\begin{tabular*}{0.98\linewidth}{@{}llccccccccc@{}}\toprule
%Architecture & Field & \multicolumn{3}{c}{Mechanism} && \multicolumn{5}{c}{Attention Use}\\   \cmidrule{3-5} \cmidrule{7-11}
% &  & soft & hard & self & & I  & II & III & IV & V \\ \midrule
%Chen [158] & Sentiment classification & \checkmark &  & & &  & \checkmark & \checkmark & &  \\
%RNNSearch [44] & Machine
%translation & \checkmark &  & & &  \checkmark&  & & & \checkmark  \\
%Cheng [156] & Natural language inference & \checkmark &  & & &  \checkmark&  & & & \checkmark  \\
%Sdnet[159] & Question-answering & \checkmark &  & & &  & \checkmark & \checkmark & &  \\
%SAB[160] & Image classification &  & \checkmark & & &  &  &  &\checkmark & \checkmark \\
%TCAN[161] & Recommender systems & \checkmark &  & & &  & \checkmark & \checkmark & &  \\
%AVS[162] & Video Summarization & \checkmark &  & &  & \checkmark &  &\checkmark  & &  \\
%HAN[52] & Document Classification & \checkmark &  & &  &  &  &\checkmark  & &  \\
%BiDAF[51] & Question-answering & \checkmark &  & &  &  & \checkmark &\checkmark  & &  \\
%\bottomrule
%\end{tabular*}
%\caption{Caption}
%\end{table}

\begin{table}[htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{
\begin{tabular*}{\linewidth}{ll}
\hline
\textbf{Task}   & \textbf{References}   \\ \hline

\textbf{Language Modeling} & \begin{tabular}[c]{@{}l@{}}\cite{dehghani_universal_2018}\cite{joulin_inferring_2015}\cite{ke_sparse_2018}\cite{cheng2016long}\cite{vinyals_matching_2016}\cite{dai_transformer-xl:_2019}\cite{sainbayar_sukhbaatar;edouard_grave;piotr_bojanowski;armand_joulin_adaptive_2019}\cite{alexei_baevski;michael_auli_adaptive_2019}\cite{michal_daniluk_tim_rocktaschel_johannes_welbl_sebastian_riedel:_frustratingly_nodate}\end{tabular} \\ \hline


\textbf{Machine Translation} &                                          \begin{tabular}[c]{@{}l@{}} \cite{kim_structured_2017}\cite{vaswani_attention_2017}\cite{gulcehre_hyperbolic_2018}\cite{feng_neural_2018}\cite{dehghani_universal_2018}\cite{bahdanau_neural_2014}\cite{luong_effective_2015}\cite{shaw_self-attention_2018}\cite{raffel_online_2017} \\ \cite{cho_learning_2014}\cite{sennrich_neural_2016}\cite{thomas_zenkel;joern_wuebker;john_denero_adding_2019}\cite{baosong_yang;jian_li;derek_wong;lidia_s._chao;xing_wang;zhaopeng_tu_context-aware_2019}\cite{baosong_yang;longyue_wang;derek_f._wong;lidia_s._chao;zhaopeng_tu_convolutional_2019}\cite{jie_hao;xing_wang;baosong_yang;longyue_wang;jinfeng_zhang;zhaopeng_tu_modeling_2019}\cite{felix_hieber;tobias_domhan;michael_denkowski;david_vilar;artem_sokolov;ann_clifton;matt_post_sockeye:_2018}\cite{xiangwen_zhang;jinsong_su;yue_qin;yang_liu;rongrong_ji;hongji_wang_asynchronous_2018}\cite{joost_bastings;ivan_titov;wilker_aziz;diego_marcheggiani;khalil_simaan_graph_2017}\\
\cite{jie_zhou;ying_cao;xuguang_wang;peng_li;wei_xu_deep_2016}\cite{yonghui_wu;mike_schuster;zhifeng_chen;quoc_v._le;mohammad_norouzi;wolfgang_macherey;maxim_krikun;yuan_cao;qin_gao;klaus_macherey;jeff_klingner;apurva_shah;melvin_johnson;xiaobing_liu;lukasz_kaiser;stephan_gouws;yoshikiyo_kato;taku_kudo;hideto_kazawa;keith_stevens;george_kurian;nishant_patil;wei_wang;cliff_young;jason_smith_googles_2016}\cite{akiko_eriguchi_kazuma_hashimoto_yoshimasa_tsuruoka:_tree--sequence_nodate}\cite{jian_li;baosong_yang;zi-yi_dou;xing_wang;michael_r._lyu;zhaopeng_tu_information_2019}\cite{orhan_firat;kyunghyun_cho;yoshua_bengio_multi-way;_2016}\cite{deng_latent_2018}\cite{h._zhang;_j._li;_y._ji;_h._yue_understanding_2017} \end{tabular} \\ \hline

\textbf{Natural Language Inference}  &                                      \begin{tabular}[c]{@{}l@{}}\cite{kim_structured_2017}\cite{parikh_decomposable_2016}\cite{shen_disan:_nodate}\cite{cheng2016long}\cite{tao_shen_tianyi_zhou_guodong_long_jing_jiang_chengqi_zhang:_bi-directional_nodate}\cite{qipeng_guo;xipeng_qiu;pengfei_liu;yunfan_shao;xiangyang_xue;zheng_zhang_star-transformer_2019}\cite{shuohang_wang;jing_jiang_learning_2016}\cite{yang_liu;chengjie_sun;lei_lin;xiaolong_wang_learning_2016}\end{tabular} \\ \hline


\textbf{Question Answering}  &                                          
\begin{tabular}[c]{@{}l@{}}\cite{kim_structured_2017}\cite{neelakantan_neural_2015}\cite{wu_hierarchical_2017}\cite{dehghani_universal_2018}\cite{weston_2014_memory}\cite{kumar_ask_2015}\cite{vinyals_neural_nodate}\cite{yang_anmm:_2018} \\ \cite{tay_densely_2018}\cite{seo_bidirectional_2016}\cite{adams_wei_yu_david_dohan_minh-thang_luong_rui_zhao_kai_chen_mohammad_norouzi_quoc_v._le:_qanet:_nodate}\cite{wei_wang_chen_wu_ming_yan:_multi-granularity_nodate}\cite{xiangyang_zhou_lu_li_daxiang_dong_yi_liu_ying_chen_wayne_xin_zhao_dianhai_yu_hua_wu:_multi-turn_nodate}\cite{cicero_dos_santos;ming_tan;bing_xiang;bowen_zhou_attentive_2016}\cite{victor_zhong;caiming_xiong;nitish_shirish_keskar;richard_socher_coarse-grain_2019}\cite{louis_shao;stephan_gouws;denny_britz;anna_goldie;brian_strope;ray_kurzweil_generating_2017}\cite{chenguang_zhu;michael_zeng;xuedong_huang_sdnet:_2019}\\ \cite{ming_tan;cicero_dos_santos;bing_xiang;bowen_zhou_lstm-based_2016}\cite{bhuwan_dhingra_hanxiao_liu_zhilin_yang_william_w._cohen_ruslan_salakhutdinov:_gated-attention_nodate}\cite{yanchao_hao_yuanzhe_zhang_kang_liu_shizhu_he_zhanyi_liu_hua_wu_jun_zhao:_end--end_nodate}\cite{rudolf_kadlec_martin_schmid_ondrej_bajgar_jan_kleindienst:_text_nodate}\cite{sukhbaatar2015end}\cite{tsendsuren_munkhdalai;hong_yu_neural_2017}\cite{seonhoon_kim;inho_kang;nojun_kwak_semantic_2018}\cite{lisa_bauer;yicheng_wang;mohit_bansal_commonsense_2019}\cite{qiu_ran;peng_li;weiwei_hu;jie_zhou_option_2019} \\ \cite{hermann2015teaching}\cite{huang_fusionnet:_2018}\cite{chen_xing;wei_wu;yu_wu;jie_liu;yalou_huang;ming_zhou;wei-ying_ma_topic_2016}\cite{sordoni_iterative_2017}\cite{bingning_wang_kang_liu_jun_zhao:_inner_nodate}  \end{tabular} \\ \hline

\textbf{Sentiment Analysis}    &                  
\begin{tabular}[c]{@{}l@{}}\cite{wang_attention-based_2017}\cite{shen_disan:_nodate}\cite{cheng2016long}\cite{dehong_ma;sujian_li;xiaodong_zhang;houfeng_wang_interactive_2017}\cite{kai_shuang_xintao_ren_qianqian_yang_rui_li_jonathan_loo:_aela-dlstms:_nodate}\cite{christos_baziotis_nikos_pelekis_christos_doulkeridis:_datastories_nodate}\cite{wei_xue;tao_li_aspect_2018}\cite{shi_feng;yang_wang;liran_liu;daling_wang;ge_yu_attention_2019}\cite{youwei_song;jiahai_wang;tao_jiang;zhiyue_liu;yanghui_rao_attentional_2019} \\ \cite{bonggun_shin;timothy_lee;jinho_d._choi_lexicon_2017}\cite{minchae_song;hyunjung_park;kyung-shik_shin_attention-based_2019}\cite{jiachen_du;lin_gui;yulan_he;ruifeng_xu;xuan_wang_convolution-based_2019}\cite{peng_chen;zhongqian_sun;lidong_bing;wei_yang_recurrent_2017}\cite{yukun_ma;haiyun_peng;erik_cambria_targeted_2018}\cite{yue_zhang;jiangming_liu_attention_2017}\cite{huimin_chen;maosong_sun;cunchao_tu;yankai_lin;zhiyuan_liu_neural_2016}\cite{jiangfeng_zeng;xiao_ma;ke_zhou_enhancing_2019}  \end{tabular} \\ \hline

\textbf{Semantic Analysis} &                  \begin{tabular}[c]{@{}l@{}}\cite{rocktaschel_reasoning_2015}\cite{she_distant_2018}\cite{zhang_learning_2018}\cite{shen_reinforced_2018}\cite{zhixing_tan;mingxuan_wang;jun_xie;yidong_chen;xiaodong_shi_deep_2017}\cite{li_dong_mirella_lapata:_language_nodate}\cite{wenya_wu;yufeng_chen;jinan_xu;yujie_zhang_attention-based_2018} \end{tabular} \\ \hline                                       


\textbf{Speech Recognition} &                                          \begin{tabular}[c]{@{}l@{}} \cite{chorowski_attention-based_2015}\cite{raffel_online_2017}\cite{prabhavalkar_minimum_2018}\cite{kazuki_irie;albert_zeyer;ralf_schluter;hermann_ney_language_2019}\cite{christoph_luscher;eugen_beck;kazuki_irie;markus_kitza;wilfried_michel;albert_zeyer;ralf_schluter;hermann_ney_rwth_2019}\cite{linhao_dong;feng_wang;bo_xu_self-attention_2019}\cite{julian_salazar;katrin_kirchhoff;zhiheng_huang_self-attention_2019}\cite{xiaofei_wang;ruizhi_li;sri_harish_mallid;takaaki_hori;shinji_watanabe;hynek_hermansky_stream_2019}\cite{shiyu_zhou;linhao_dong;shuang_xu;bo_xu_syllable-based_2018} \\ \cite{shinji_watanabe;takaaki_hori;suyoun_kim;john_r._hershey;tomoki_hayashi_hybrid_2017}\cite{dzmitry_bahdanau;jan_chorowski;dmitriy_serdyuk;philemon_brakel;yoshua_bengio_end--end_2016}\cite{jan_chorowski;dzmitry_bahdanau;kyunghyun_cho;yoshua_bengio_end--end_2014}\cite{f_a_rezaur_rahman_chowdhury;quan_wang;ignacio_lopez_moreno;li_wan_attention-based_2018}\cite{yiming_wang;xing_fan;i-fan_chen;yuzong_liu;tongfei_chen;bjorn_hoffmeister_end--end_2019}\cite{albert_zeyer;kazuki_irie;ralf_schluter;hermann_ney_improved_2018}\cite{suyoun_kim;takaaki_hori;shinji_watanabe_joint_2017}\cite{koji_okabe;takafumi_koshinaka;koichi_shinoda_attentive_2018}\cite{takaaki_hori;shinji_watanabe;yu_zhang;william_chan_advances_2017} \end{tabular} \\ \hline


\textbf{Text Summarization} &       
\begin{tabular}[c]{@{}l@{}}\cite{chopra_abstractive_2016}\cite{paulus_deep_2017}\cite{nallapati_abstractive_2016}\cite{see_get_2017}\cite{raffel_online_2017}\cite{alexander_m._rush;sumit_chopra;jason_weston_neural_2015}\cite{angela_fan;mike_lewis;yann_dauphin_hierarchical_2018}\cite{b._rekabdar;_c._mousas;_b._gupta_generative_2019}\cite{arman_cohan;franck_dernoncourt;doo_soon_kim;trung_bui;seokhwan_kim;walter_chang;nazli_goharian_discourse-aware_2018} \end{tabular} \\ \hline
\end{tabular*}
\caption{Summary state-of-the-art approaches in several natural language processing sub-areas.}
\label{tab:main_nlp_app}
\end{table}


For \textbf{machine translation} (MT), \textbf{question answering} (QA), and \textbf{automatic speech recognition} (ASR), attention works mainly in the alignment input and output sequences capturing long-range dependencies. For example, in ASR tasks, attention aligns acoustic frames extracting information from anchor words to recognize the main speaker while ignoring background noise and interfering speech. Hence, only information on the desired speech is used for the decoder as it provides a straightforward way to align each output symbol with different input frames with selective noise decoding. In MT, automatic alignment translates long sentences more efficiently. It is a powerful tool for \textbf{multilingual machine translation} (NMT), efficiently capturing subjects, verbs, and nouns in sentences of different languages that differ significantly in their syntactic structure and semantics.

%atencao em question and answering
In QA, alignment usually occurs between a query and the content, looking for key terms to answer the question. The classic QA approaches do not support very long sequences and fail to correctly model the meaning of context-dependent words. Different words can have different meanings, which increases the difficulty of extracting the essential semantic logical flow of each sentence in different paragraphs of context. These models are unable to address uncertain situations that require additional information to answer a particular question. In contrast, attention networks allow rich dialogues through addressing mechanisms for explicit memories or alignment structures in the query-context and context-query directions.

% colocar algumas citacoes de trabalho de QA
%colocar algumas citacoes de trabalhos usando alinhamento



% colocar algumas citacoes após o paragrafo

Attention also contributes to \textbf{summarize or classify texts/documents}. It mainly helps build more effective embeddings that generally consider contextual, semantic, and hierarchical information between words, phrases, and paragraphs. Specifically, in summarization tasks, attention minimizes critical problems involving: 1) modeling of keywords; 2) summary of abstract sentences; 3) capture of the sentence's hierarchical structure; 4) repetitions of inconsistent phrases; and 5) generation of short sentences preserving their meaning.



\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{img/nlp_apps_1.pdf}  
  \caption{Illustration of RNNSearch \cite{bahdanau_neural_2014} for machine translation, and End-to-End Memory Networks \cite{sukhbaatar2015end} for question answering. a) The RNNSearch architecture. The attention guided by the decoder's previous state dynamically searches for important source words for the next time step. b) The End-to-End Memory Networks. The architecture consists of external memory and several stacked attention modules. To generate a response, the model makes several hops in memory using only attentional layers.}
  \label{fig:nlp_apps_1}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{img/the_neural_transformer.pdf}  
  \caption{Illustration of Neural Transformer \cite{vaswani_attention_2017} for machine translation. The architecture consists of several stacked attentional encoders and decoders. The encoder process is massively parallel and eliminates recurrences, and the decoder generates the translated words sequentially. Each encoder uses multiple heads of the self-attention mechanism followed by fusion and normalization layers. Similarly, to generate the output, each decoder has multiple heads of self-attention and masked-self attention to mask words not yet generated.}
  \label{fig:nlp_apps_2}
\end{figure}


Figure \ref{fig:nlp_apps_1} 
illustrates two models working in NLP tasks: RNNSearch \cite{bahdanau_neural_2014}, in machine translation, and End-to-End Memory Networks \cite{sukhbaatar2015end} in question answering. In \textbf{RNNSearch}, the attention guided by the decoder's previous state dynamically searches for important source words for the next time step. It consists of an encoder followed by a decoder. The encoder is a bidirectional RNN (BiRNN) \cite{schuster1997bidirectional} that consists of forward and backward RNN's. The forward RNN reads the input sequence in order and calculates the forward hidden state sequence. The backward RNN reads the sequence in the reverse order, resulting in the backward hidden states sequence. The decoder has an RNN and an attention system that calculates a probability distribution for all possible output symbols from a context vector.


In \textbf{End-to-End Memory Networks}, attention looks for the memory elements most related to query $q$ using an alignment function that dispenses the RNNs' complex structure. It consists of a memory and a stack of identical attentional systems. Each layer $i$ takes as input set $\left \{ x_{1}, ..., x_{N} \right \}$ to store in the memory. The input set is converted in memory vectors $\left \{ m_{1}, ..., m_{N} \right \}$ and $\left \{ h_{1}, ..., h_{N} \right \}$, in the simplest case using the embedding matrix $A^{i} \in \mathbb{R}^{d \times V}$ to generate each $m_{i} \in \mathbb{R}^{d}$, and the matrix $C^{i} \in \mathbb{R}^{d \times V}$ to generate each $h_{i} \in \mathbb{R}^{d}$. In the first, layer the query $q$ is also embedded, via embedding matrix $B^{1}$ to obtain an internal state $u^{1}$. From the second layer, the internal state $u^{i+1}$ is the sum of the $i$ layer output and the internal state $u^{i}$. Finally, the last layer generates $\hat{a}$.

The \textbf{Neural Transformer} \cite{vaswani_attention_2017}, illustrated in figure \ref{fig:nlp_apps_2}, is the basis model for state-of-the-art results in NLP. The architecture consists of an arbitrary amount of stacked encoders and decoders. Each encoder has linear layers, an attention system, feed-forward neural networks, and normalization layers. The attention system has several parallel heads. Each head has $N$ attentional subsystems that perform the same task but have different contextual inputs. The encoder receives a word embedding matrix $I = \left \{ x_{1}, ..., x_{N} \right \}$, $I$ $\in \mathbb{R}^{N \times d_{emb}}$ as input. As the architecture does not use recurrences, the input tokens' position information is not explicit, but it is necessary. To represent the spatial position information, the Transformer adds a positional encoding to each embedding vector. Positional encoding is fixed and uses sinusoidal functions.

The input $I$ goes through linear layers and generates, for each word, a \textbf{query vector} ($q_{i}$), a \textbf{key vector} ($k_{i}$), and a \textbf{value vector} ($v_{i}$).The attentional system receives all $Q$, $K$, and $V$ arrays as input and uses several parallel attention heads. The motivation for using a multi-head structure is to explore multiple subspaces since each head gets a different projection of the data. Each head learns a different aspect of attention to the input, calculating different attentional distributions. Having multiple heads on the Transformer is similar to having multiple feature extraction filters on CNNs. The head outputs an attentional mask that relates all queries to a certain key. In a simplified way, the operation performed by a head is a matrix multiplication between a matrix of queries and keys.

Finally, the data is added to the residual output from the previous layer and normalized, representing the encoder output. This data is input to the next encoder. The last encoder's data are transformed into the attention matrices $K_{encdec}$ and $V_{encdec}$. They are input to all decoder layers. This data help the decoder to focus on the appropriate locations in the input sequence. The decoder has two layers of attention, Feed-Foward layers and normalization layers. The attentional layers are the masked multi-head attention and the decoder multi-head attention. 

The masked multi-head attention is very similar to the encoder multi-head attention, with the difference that the attention matrices $Q$, $K$, and $V$ are created only with the previous data words, masking future positions with $-\infty$ values before the softmax step. The decoder multi-head attention is equal to the encoder multi-head attention, except it creates the \textit{Q} matrix from the data of the previous layer and uses the $K_{encdec}$ and $V_{encdec}$ matrices of the encoder output. The $K_{encdec}$ and $V_{encdec}$ matrices are the memory structure of the network, storing context information of the input sequence, and given the previous words in the output decoder, the relevant information is selected in memory for the prediction of the next word. Finally, a linear layer followed by a softmax function projects the decoder vector by the last decoder into a probability vector in which each position defines the probability of the output word being a given vocabulary word. At each time step $t$, the position with the highest probability value is chosen, and the word associated with it is the output.

 
%falar um pouquinho de outras abordagens e finalizar

% atencao na captura de estruturas hierarquicas

%In document classification, attention contributes to creating more effective document representations, using attentional mechanisms at various levels. Text summarization helps to model critical summarization problems that are not adequately dealt by basic architectures, such as modeling keywords. It captures the sentence structure hierarchy, generating incoherent sentence repetitions, and difficulty summarizing abstract sentences. Also, attention contributes to producing a short version of a sentence while preserving its meaning. This ensures that the decoder focuses only on appropriate words from the input at each generation step.






%Inicialmente os mecanismos de atenção surgiram em tarefas de machine translation em redes do tipo encoder-decoder com o objetivo de realizar o alinhamento entre as sentenças de diferentes idiomas e de superar o problema da falta de capacidade dos modelos tradicionais para lidar com sequências muito longas. Dado o sucesso na área de machine translation e sua expansão, outras áreas posteriormente se benefeciaram do uso dos mecanismos atencionais, por exemplo, em Automatic Speech Recognition (ARS) a atenção contribui para o alinhamento dos quadros acústicos, extrai informações de palavras âncoras reconhecendo o falante principal e ignora ruídos de fundo e falas interferentes. Além disso, o mecanismo de atenção fornece uma maneira explícita de alinhar cada símbolo de saída com diferentes quadros da entrada, permitindo uma decodificação seletiva do ruído, ou seja, apenas informações do discurso desejado é utilizada na decodificação.


%Na classificação de documentos a atenção contribui para criar representações de documentos mais eficazes, utilizando mecanismos atencionais em vários níveis. Na sumarização de texto ela ajuda a modelar problemas críticos na summarização que não são adequadamente modelados pelas arquiteturas básicas, como modelar palavras-chave, capturar a hierárquia da estrutura da sentença, gerar repetições de frases incoerentes e dificuldade em resumir frases abstratas. Além disso, a atenção contribui para gerar uma versão curta de uma sentença preservando o seu significado, garantindo que o decodificador se concentre apenas em palavras apropriadas da entrada em cada etapa de geração.






\begin{table}[htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{
\begin{tabular*}{\linewidth}{lll}
\hline
\textbf{Task}                           & \textbf{References}                                     \\ \hline
\textbf{Code Summarization}          & \cite{allamanis2016convolutional} \\ \hline
\textbf{Language Recognition}     & \cite{huang2018video}               \\ \hline
\textbf{Emotion Recognition}     &                
\begin{tabular}[c]{@{}l@{}}\cite{seyedmahdad_mirsamadi;emad_barsoum;cha_zhang_automatic_2017}\cite{le_hoang_son;akshi_kumar;saurabh_raj_sangwan;anshika_arora;an;nayyar;mohamed_abdel-basset_sarcasm_2019}\cite{kun-yi_huang;chung-hsien_wu;ming-hsiang_su_attention-based_2019}\cite{navonil_majumder;soujanya_poria;devamanyu_hazarika;rada_mihalcea;alexander_gelbukh;erik_cambria_dialoguernn:_2019}\cite{yuanyuan_zhang;jun_du;zirui_wang;jianshu_zhang_attention_2019}\cite{michael_neumann;ngoc_thang_vu_attentive_2017}\cite{wenya_wang;sinno_jialin_pan;daniel_dahlmeier;xiaokui_xiao_coupled_2017} \end{tabular} \\ \hline

\textbf{Text Classification}   & \cite{liu2019bidirectional}\cite{qipeng_guo;xipeng_qiu;pengfei_liu;yunfan_shao;xiangyang_xue;zheng_zhang_star-transformer_2019} \\ \hline

\textbf{Speech Classification}  &                  \cite{norouzian2019exploring}\cite{li2019multi} \\ \hline

\textbf{Relation Classification}        &                  
\begin{tabular}[c]{@{}l@{}}\cite{patrick_verga;emma_strubell;andrew_mccallum_simultaneously_2018}\cite{xiaoyu_guo;hui_zhang;haijun_yang;lianyuan_xu;zhiwen_ye_single_2019}\cite{linlin_wang_zhu_cao_gerard_de_melo_zhiyuan_liu:_relation_nodate}\cite{peng_zhou_wei_shi_jun_tian_zhenyu_qi_bingchen_li_hongwei_hao_bo_xu:_attention-based_nodate}\cite{yankai_lin_shiqi_shen_zhiyuan_liu_huanbo_luan_maosong_sun:_neural_nodate}\cite{yuhao_zhang;victor_zhong;danqi_chen;gabor_angeli;christopher_d._manning_position-aware_2017}  \end{tabular} \\ \hline

\textbf{Intent Classification}   &                  \cite{chen2019bert}                                       \\ \hline


\textbf{Document Classification}      &                  \cite{choi2019aila}\cite{yang2016hierarchical}           \\ \hline

\textbf{Audio Classification}          &                  \cite{kong2018audio}                                       \\ \hline

\textbf{Transfer Learning}        &                  \cite{devlin2018bert}\cite{alt2019improving}              \\ \hline

\textbf{Text-to-Speech}            &                  \cite{yasuda2019investigation}\cite{zhang2019joint}\cite{li2019neural}      \\ \hline

\textbf{Syntax Analysis}       &                  \cite{kuncoro2016recurrent}                                \\ \hline

\textbf{Speech Translation}           &                  \cite{sperber2019attention}                                \\ \hline

\textbf{Speech Transcription}          &                  \cite{chan2015listen}                                       \\ \hline

\textbf{Speech Production}             &                  \cite{tachibana2018efficiently}                             \\ \hline

\textbf{Sequence Prediction}           &                  \cite{mensch2018differentiable}                             \\ \hline


\textbf{Semantic Matching}             &                  \cite{zhang2018multiresolution}                              \\ \hline


\textbf{Relation Extraction}           &                \cite{zhang2019long}                                     \\ \hline

\textbf{Reading Comprehension}         &                  \cite{tao_shen_tianyi_zhou_guodong_long_jing_jiang_chengqi_zhang:_bi-directional_nodate}\cite{wei_wang_chen_wu_ming_yan:_multi-granularity_nodate}\cite{yiming_cui_zhipeng_chen_si_wei_shijin_wang_ting_liu_guoping_hu:_attention-over-attention_nodate}\cite{s._liu;_s._zhang;_x._zhang;_h._wang_r-trans:_2019}\cite{yiming_cui;ting_liu;zhipeng_chen;shijin_wang;guoping_hu_consensus_2018}                                       \\ \hline

\textbf{Natural Language Understanding}   &                  \cite{kim2018efficient}                                       \\ \hline


\textbf{Natural Language Transduction}    &                   \cite{grefenstette2015learning}                              \\ \hline


\textbf{Natural Language Generation}     &                  \cite{xu2018graph2seq}                                       \\ \hline


\textbf{Machine Reading}               &                  \cite{yang2019leveraging}                                    \\ \hline

\textbf{Intent Detection}              &                  \cite{liu2016attention}                                       \\ \hline

\textbf{Grammatical Correction}        &                  \cite{ahmadi2018attention}                                    \\ \hline

\textbf{Entity Resolution}             &                  \cite{das2016chains}\cite{ganea2017deep}                     \\ \hline

\textbf{Entity Description}            &                  \cite{ji2017distant}                                          \\ \hline

\textbf{Embedding}                     &                  \cite{lin2017structured}\cite{schick2019attentive}\cite{zhu2018self}
\\ \hline

\textbf{Dependency Parsing}            &                  \cite{dozat2016deep}\cite{strubell2018linguistically}        \\ \hline

\textbf{Conversation Model}          &                  \cite{zhou2018commonsense}\cite{zhang2019sequence}           \\ \hline
\textbf{Automatic Question Tagging}    &                  \cite{sun2018automatic}                                       \\ \hline

\end{tabular*}
\caption{Summary others applications of attention in natural language processing.}
\label{tab:others_nlp_applications}
\end{table}

%Além da área de tradução de máquina, outra área que sofreu grande expansão com o uso de atenção foi a de question e answering (QA), com o objetivo de criar sistemas inteligentes capazes de se comunicar naturalmente com os seres humanos. As abordagens clássicas dessa área utilizam uma arquitetura encoder-decoder para mapear respostas e perguntas para vetores de comprimento fixo e o decoder atua gerando as saídas. No entanto, uma dificuldade clássica dessa área é que essas arquiteturas não suportam sequências muito longas, dificultando a geração de arquiteturas capazes de conversar sobre diálogos complexos. Além disso, esses modelos não conseguem modelar corretamente o significado das palavras dependentes do contexto. Palavras diferentes podem ter significados diferentes, o que aumenta a dificuldade de extrair o fluxo lógico semântico essencial de cada setença em parágrafos diferentes. Assim, os modelos não consegue abordar situações incertas que exigem informações adicionais do usuário para reunir informações completas para responder uma determinada pergunta. No entanto, cenários com informações incompletas aparecem naturalmente em diálogos humanos. Essas dificuldades dos modelos clássicos impulsionaram o desenvolvimento de redes neurais que utilizam memória externa explícita e atenção para controlar o acesso a memória. Essa nova abordagem consegue um sucesso notável nesse tipo de problema e introduz um novo tipo de arquitetura: as redes neurais que são capazes de manipular memória externa que conseguem lidar eficientemente com contextos longos e responder perguntas complexas que necessitam de uma análise global do contexto.




==> PART_III_subs/others.tex <==
\subsection{\textbf{Others}}
\label{sec:others}

==> PART_III_subs/recommender.tex <==
%%esther: check 1

\subsection{Recommender Systems (RS)}
\label{sec:application_recommender}

Attention has also been used in recommender systems for behavioral modeling of users. Capturing user interests is a challenging problem for neural networks, as some iterations are transient, some clicks are unintentional, and interests can change quickly in the same session. Classical approaches (i.e., Markov Chains and RNNs) have limited performance predicting the user's next actions, present different performances in sparse and dense datasets, and long-term memory problems. In this sense, attention has been used mainly to assign weights to a user's interacted items capturing long and short-term interests more effectively than traditional ones. Self-attention and memory approaches have been explored to improve the area's development. STAMP \cite{liu2018stamp} model, based on attention and memory, manages users' general interests in long-term memories and current interests in short-term memories resulting in behavioral representations that are more coherent. The Collaborative Filtering \cite{chen2017attentive} framework, and SASRec \cite{kang_deep_2018} explored self-attention in capturing long-term semantics for finding the most relevant items in user's history. 



==> PART_III_subs/rl.tex <==
%% esther: check 1

\subsection{\textbf{Reinforcement Learning (RL)}}
\label{sec:application_rl}

Attention has been gradually introduced in reinforcement learning to deal with unstructured environments in which rewards and actions depend on past states and where it is challenging guaranteeing the Markov property. Specifically, the goals are to increase the agent's generalizability and minimize long-term memory problems. Currently, the main attentional reinforcement learning approaches are computer vision, graph reasoning, natural language processing, and virtual navigation, as shown in table \ref{tab:rl_applications}.


\begin{table}[!htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{

\begin{tabular*}{\linewidth}{lll}
\hline
\textbf{Task}   & \textbf{References}           \\ \hline

\textbf{Computer Vision} & 
\begin{tabular}[c]{@{}l@{}}\cite{ba_multiple_2014}\cite{li_action_2019}\cite{rao_attention-aware_2017}\cite{stollenga_deep_2014}\cite{cao_attention-aware_2017} \\ \cite{zhao_deep_2017}\cite{donghui_hu;shengnan_zhou;qiang_shen;shuli_zheng;zhongqiu_zhao;yuqi_fan_digital_2019}\cite{marcus_edel;joscha_lausch_capacity_2016}\cite{yeung_end--end_2016} \end{tabular}
 \\ \hline


\textbf{Graph reasoning}   & \cite{lee2018graph}                                                         \\ \hline
\textbf{Natural Language Processing}  &  \cite{santoro2018relational} \\ \hline

\textbf{Navigation}     &  \cite{mishra_simple_2017}\cite{parisotto2017neural}\cite{zambaldi2018relational}\cite{santoro2018relational}\cite{baker2019emergent}
\\ \hline

\end{tabular*}
\caption{Summary of main state-of-art approaches in attentional reinforcement learning tasks.}
\label{tab:rl_applications}
\end{table}


%%%%% Navegacao

To increase the ability to generalize in partially observable environments, some approaches use attention in the policy network. Mishra et al. \cite{mishra_simple_2017} used attention to easily capture long-term temporal dependencies in convolutions in an agent's visual navigation task in random mazes. At each time step $t$, the model receives as input the current observation $o_ {t}$ and previous sequences of observations, rewards, and actions so that attention allows the policy to maintain a long memory of past episodes. Other approaches implement attention directly to the representation of the state. State representation is a classic and critical problem in RL, given that state space is one of the major bottlenecks for speed, efficiency, and generalization of training techniques. In this sense, the importance of attention on this topic is quite intuitive.

However, there are still few approaches exploring the representation of states. The neural map \cite{parisotto2017neural} maintains an internal memory in the agent controlled via attention mechanisms. While the agent navigates the environment, an attentional mechanism alters the internal memory, dynamically constructing a history summary. At the same time, another generates a representation $o_{t}$, based on the contextual information of the memory and the state's current observation. Then, the policy network receives $o_{t}$ as input and generates the distribution of shares. Some more recent approaches affect the representation of the current $o_{t}$ observation of the state via self attention in iterative reasoning between entities in the scene \cite{zambaldi2018relational} \cite{baker2019emergent}, or between the current observation $o_{t}$ and memory units \cite{santoro2018relational} to guide model-free policies.

The most discussed topic is the use of the policy network to guide the attentional focus of the agent's glimpses sensors on the environment so that the representation of the state refers to only a small portion of the entire operating environment. This approach emerged initially by Graves et al. \cite{mnih_recurrent_2014} using policy gradient methods (i.e., REINFORCE algorithm) in the hybrid training of recurrent networks in image classification tasks. Their model consists of a glimpse sensor that captures only a portion of the input image, a core network that maintains a summary of the history of patches seen by the agent, an action network that estimates the class of the image seen, and a location network trained via RL which estimates the focus of the glimpse on the next time step, as shown in figure \ref{fig:rl_applications_ok}a. This structure considers the network as the agent, the image as the environment, and the reward is the number of correct network ratings in an episode. Stollenga et al. \cite{stollenga_deep_2014} proposed a similar approach, however directly focused on CNNs, as shown in figure \ref{fig:rl_applications_ok}b. The structure allows each layer to influence all the others through attentional bottom-up and top-down connections that modulate convolutional filters' activity. After supervised training, the attentional connections' weights implement a control policy via RL and SNES \cite{schaul2011high}. The policy learns to suppress or enhance features at various levels by improving the classification of difficult cases not captured by the initial supervised training. Subsequently, variants similar to these approaches appeared in multiple image classification \cite{ba_multiple_2014} \cite{marcus_edel;joscha_lausch_capacity_2016} \cite{zhao_deep_2017}, action recognition \cite{yeung_end--end_2016}, and face hallucination \cite{cao_attention-aware_2017}.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\linewidth]{img/reinforcement_learning_apps.pdf}  
  \caption{Illustration of RAM \cite{mnih_recurrent_2014} and dasNet \cite{stollenga_deep_2014} for image classification tasks. a) The RAM framework. At each time step $t$, the glimpse networks extracts a retina-like representation based on input image and an focus location $l_{t-1}$. The core network takes the glimpse representation as input and combining it with the internal representation at the previous time step and produces the new internal state of the model $h_{t}$. The location network and action network use the $h_{t}$ to produce the next location $l_{t}$ to attend and the classification. b) The dasNet network. Each image is classified after $T$ passes through CNNs. After each forward propagation, the averages of feature maps are combined into an observation vector $o_{t}$ that is used by a deterministic policy to choose an action $a_{t}$ that changes the focus of all the feature maps for the next pass of the same image. Finally, after pass $T$ times, the output is used to classify the image.}
  \label{fig:rl_applications_ok}
\end{figure}














==> PART_III_subs/robotics.tex <==
%% esther: check 1

\subsection{\textbf{Robotics}} 
\label{sec:applications_robotics}
%Poucas aplicações em robótica envolvem redes neurais profundas e atenção. Além disso, como a robótica é uma área multidisciplinar é comum que todas essas aplicações envolvam outras grandes áreas, como processamento de linguagem natural, visão computacional e aprendizado por reforço ou imitação. A Figura X, ilustra as áreas existentes e a proporção de trabalhos em cada uma delas. Como mostra essa figura a maior parte dos trabalhos se concentra na área de navegação de robôs autônomos, seguida pela área de controle e de iteração homem-robô. A atenção tem sido utilizada em cada uma dessas áreas para minimizar os seguintes problemas:

In robotics, there are still few applications with neural attentional models. A small portion of current work is focused on control, visual odometry, navigation, and human-robot interaction, as shown in table \ref{tab:robotics_applications}. 


\begin{table}[!htb]
\tiny
\fontfamily{pcr}\selectfont
%\textcolor{tabgrey}{
\begin{tabular*}{\linewidth}{lll}
\hline
\textbf{Task}    &  \textbf{References} \\ \hline
\textbf{Control}   &  \cite{one_shot}\cite{pay_attention} \\ \hline
\textbf{Visual odometry}  & \cite{xue2020deep}\cite{johnston2020self}\cite{kuo2020dynamic}\cite{damirchi2020exploring}\cite{gao2020attentional}\cite{li2021transformer}     \\ \hline
\textbf{Navigation}  &  \cite{sophie}\cite{social_attention}\cite{crowd}\cite{scene_memory} \\ \hline
\textbf{Human-robot interaction}  &   \cite{translating_navigation}             \\ \hline
\end{tabular*}
\caption{Summary state-of-art main approaches in robotics.}
\label{tab:robotics_applications}
\end{table}

\textbf{Navigation} and visual odometry are the most explored domains, although still with very few published works. For classic DL approaches, navigating tasks in real or complex environments are still very challenging. These approaches have limited performance in dynamic and unstructured environments and over long horizon tasks. In real environments, the robot must deal with dynamic and unexpected changes in humans and other obstacles around it. Also, decision-making depends on the information received in the past and the ability to infer the future state of the environment. Some seminal approaches in the literature have demonstrated the potential of attention to minimizing these problems without compromising the techniques' computational cost. Sadeghian et al. \cite{sophie} proposed Sophie: an interpretable framework based on GANs for robotic agents in environments with human crowds. Their framework via attention extracts two levels of information: a physical extractor learns spatial and physical constraints generating a $C$ context vector that focuses on viable paths for each agent. In contrast, a social extractor learns the interactions between agents and their influence on each agent's future path. Finally, LSTMs based on GAN generate realistic samples capturing the nature of future paths, and the attentional mechanisms allow the framework to predict physically and socially feasible paths for agents, achieving cutting-edge performances on several different trajectories.

Vemula et al. \cite{social_attention} proposed a trajectory prediction model that captures each person's relative importance when navigating in the crowd, regardless of their proximity via spatio-temporal graphs. Chen et al. \cite{crowd} proposed the crowd-aware robot navigation with attention-based deep reinforcement learning. Specifically, a self-attention mechanism models interactions between human-robot and human-human pairs, improving the robot's inference capacity of future environment states. It also captures how human-human interactions can indirectly affect decision-making, as shown in figure \ref{fig:robotic_apps} in a). Fang et. al. \cite{scene_memory} proposed the novel memory-based policy (i.e., scene memory transformer - SMT) for embodied agents in long-horizon tasks. The SMT policy consists of two modules: 1) scene memory which stores all past observations in an embedded form, and 2) an attention-based policy network that uses the updated scene memory to compute a distribution over actions. The SMT model is based on an encoder-decoder Transformer and showed strong performance as the agent moves in a large environment, and the number of observations grows rapidly.

In \textbf{visual odometry} (VO), the classic learning-based methods consider the VO task a problem of pure tracking through the recovery of camera poses from fragments of the image, leading to the accumulation of errors. Such approaches often disregard crucial global information to alleviate accumulated errors. However, it is challenging to preserve this information in end-to-end systems effectively. Attention represents an alternative that is still little explored in this area to alleviate such disadvantages. Xue et al. \cite{xue2020deep} proposed an adaptive memory approach to avoid the network's catastrophic forgetfulness. Their framework consists mainly of a memory, a remembering, and a refining module, as shown in figure \ref{fig:robotic_apps}b). First, it remembers to select the main hidden states based on camera movement while preserving selected hidden states in the memory slot to build a global map. The memory stores the global information of the entire sequence, allowing refinements on previous results. Finally, the refining module estimates each view's absolute pose, allowing previously refined outputs to pass through recurrent units, thus improving the next estimate.

Another common problem in VO classical approaches is selecting the features to derive ego-motion between consecutive frames. In scenes, there are dynamic objects and non-textured surfaces that generate inconsistencies in the estimation of movement. Recently, self-attention mechanisms have been successfully employed in dynamic reweighting of features, and in the semantic selection of image regions to extract more refined egomotion \cite{kuo2020dynamic} \cite{damirchi2020exploring} \cite{gao2020attentional}. Additionally, self-attentive neural networks have been used to replace traditional recurrent networks that consume training time and are inaccurate in the temporal integration of long sequences \cite{li2021transformer}.



\begin{figure}[htb]
  \centering
  \includegraphics[width=\linewidth]{img/robotic_apps.pdf}  
  \caption{Illustration of deep visual odometry with Adaptive Memory \cite{xue2020deep} and Crowd-Robot Interaction \cite{crowd} for navigation. a) The deep visual odometry with adaptive memory framework. This framework introduces two important components called \textit{remembering} and \textit{refining}, as opposed to classic frameworks that treat VO as just a tracking task. \textit{Remembering} preserves long-time information by adopting an adaptive context selection, and \textit{refining} improves previous outputs using spatial-temporal feature reorganization mechanism. b) Crowd-Robot Interaction network. The network consists of three modules: interaction, pooling, and planning. Interaction extracts robot-human interactions in crowds. Pooling aggregates all interaction information, and planning estimates the state's value based on robots and humans for navigation in crowds.}
  \label{fig:robotic_apps}
\end{figure}




In \textbf{human-robot interaction}, Zang et al. \cite{translating_navigation} proposed a framework that interprets navigation instructions in natural language and finds a mapping of commands in an executable navigation plan. The attentional mechanisms correlate navigation instructions very efficiently with the commands to be executed by the robot in only one trainable end-to-end model, unlike the classic approaches that use decoupled training and external interference during the system's operation. In \textbf{control}, existing applications mainly use manipulator robots in visual-motor tasks. Duan et al. \cite{one_shot} used attention to improve the model's generalization capacity in imitation learning approaches with a complex manipulator arm. The objective is to build a one-shot learning system capable of successfully performing instances of tasks not seen in the training. Thus, it employs soft attention mechanisms to process a long sequence of (states, actions) demonstration pairs. Finally, Abolghasemi et al. \cite{pay_attention} proposed a deep visual engine policy through task-focused visual attention to make the policy more robust and to prevent the robot from releasing manipulated objects even under physical attacks.



%Na área de iteração homem-robô um dos principais objetivos é conseguir uma iteração rápida, segura e eficiente entre o ser humano e um robô. Isso é bastante útil no domínio da robótica de serviço, em que robôs podem seguir instruções de navegação para ajudar com a manipulação móvel e tarefas de entrega. No entanto, interpretar instruções de navegação em linguagem natural é difícil, pois há uma variedade de formas de descrever a mesma rota. Além disso, interpretar instruções e encontrar um mapeamento dos comandos em um plano de navegação executável é bastante complicado e muitos erros podem ocorrer nesse processo. Mecanismos de atenção nesse tipo de aplicação correlacionam de forma bastante eficiente as intruções de navegação com os comandos a serem realizados pelo robô em apenas um modelo treinável de ponta-a-ponta \cite{translating_navigation}.

%Na área de controle as aplicações existentes utilizam robôs manipuladores, cujo objetivo é utilizar atenção para melhorar a capacidade de generalização do modelo em abordagens de apredizado por imitação. O objetivo é construir um sistema de aprendizado com poucas amostras (one-shot learning) capaz de realizar com sucesso instâncias de tarefas que não foram vistas no treinamento. Para isso, mecanismos de soft attention são utilizados na arquitetura para processar uma sequência longa de estados e ações que correspondem à demonstração \cite{one_shot}. 

%In the control area, existing applications use manipulative robots that use attention to improve the model's generalization capacity in imitation learning approaches. The objective is to build a learning system with few samples (one-shot learning) capable of successfully performing instances of tasks that were not seen in the training. For that, soft attention mechanisms are used in the architecture to process a long sequence of states and actions that correspond to the demonstration \cite{one_shot}.

%Um outro problema de controle de manipuladores que vem sendo melhorado utilizando atenção é o de controle visual motor. Nesse tipo de tarefa, o controle do manipulador fica bastante vulnerável a distúrbios físicos soltando o objeto manipulado com facilidade. Mecanismos de atenção visual focados em tarefas tem sido utilizados para tornar a política mais robusta e fazer com o robô não solte os objetos manipulados mesmo sob ataques físicos \cite{pay_attention}.



%Although there are already some approaches using attention in robotics, few architectures and few problems are being explored, since robotics presents a vast field of new challenges.


==> PART_II_subs/bert.tex <==
\textbf{Bidirectional Encoder Representations from Transformers (BERT)}. BERT uses attention to language modelling. 
The architecture is a multi-layer bidirectional Transformer encoder based on the original implementation \cite{vaswani_attention_2017}. Do ponto de vista atencional a BERT não trás nenhuma novidade, ela apenas utilizar o encoder da Transformer em tarefas mais complexas. A distinctive feature of BERT is its unified architecture across different tasks. Há dois steps no framework -- pre-training and fine-tuning. Durante o pré-treino o modelo é treinado com dados não rotulados sobre diferentes tarefas de pré-treino. 


For finetuning, the BERT model is first initialized with
the pre-trained parameters, and all of the parameters are fine-tuned using labeled data from the  downstream tasks. Each downstream task has separate fine-tuned models, even though they are initialized with the same pre-trained parameters. The question-answering example in Figure X will serve as a running example for this section.



During pre-training, the model is trained on unlabeled data over different pre-training tasks. 


A arquitetura do modelo do BERT é um codificador Transformer bidirecional multicamadas com base na implementação original descrita em Vaswani et al. (2017) e lançado em
a biblioteca tensor2tensor.1 Porque o uso
de Transformers tornou-se comum e nossa implementação é quase idêntica à original,
vamos omitir uma descrição de fundo exaustiva da arquitetura do modelo e recomendar aos leitores
Vaswani et al. (2017), bem como excelentes guias
como “O transformador anotado”. 2
Neste trabalho, denotamos o número de camadas
(ou seja, blocos do Transformer) como L, o tamanho oculto como
H, e o número de cabeças de autoatenção como A.
3
Nós relatamos resultados principalmente em dois tamanhos de modelo:
BERTBASE (L = 12, H = 768, A = 12, Parâmetros totais = 110M) e BERTLARGE (L = 24, H = 1024,
A = 16, Parâmetros totais = 340M).
A BERTBASE foi escolhida para ter o mesmo modelo
tamanho como OpenAI GPT para fins de comparação.
Criticamente, no entanto, o transformador BERT usa
autoatenção bidirecional, enquanto o Transformer GPT usa autoatenção restrita onde cada
token só pode atender ao contexto à sua esquerda
Abrir no Google Tradutor	
Feed













A distinctive feature of BERT is its unified architecture across different tasks. There is minimal difference between the pre-trained architecture and the final downstream architecture.

BERT’s model architecture is a multi-layer bidirectional Transformer encoder based on the original implementation described in Vaswani [X] and released in the tensor2tensor library.1 Because the use of Transformers has become common and our implementation is almost identical to the original,
we will omit an exhaustive background description of the model architecture and refer readers to [X] as well as excellent guides such as “The Annotated Transformer.

\begin{figure}[h]
  \centering
  \includegraphics[width=100mm]{img/bert.jpg}
  \caption{BERT Architecture.}
  \label{fig:bert_arquitetura}
\end{figure}

To make BERT handle a variety of down-stream tasks, our input
representation is able to unambiguously represent
both a single sentence and a pair of sentences
(e.g., h Question, Answeri) in one token sequence.
Throughout this work, a “sentence” can be an arbitrary span of contiguous text, rather than an actual
linguistic sentence. A “sequence” refers to the input token sequence to BERT, which may be a single sentence or two sentences packed together.

Using WordPiece embeddings (Wu et al., 2016) with a 30,000 token vocabulary. The first token of every sequence is always a special classification token ([CLS]). The final hidden state corresponding to this token is used as the aggregate sequence representation for classification tasks. Sentence pairs are packed together into a single sequence. We differentiate the sentences in two ways. First, we separate them with a special token ([SEP]). Second, we add a learned embedding to every token indicating whether it belongs
to sentence A or sentence B. 

Unlike Peters [X] and Radford et al [X], we do not use traditional left-to-right or right-to-left language models to pre-train BERT.
Instead, we pre-train BERT using two unsupervised tasks, described in this section. This step is presented in the left part of Figure X.

Intuitively, it is reasonable to believe that a deep bidirectional model is
strictly more powerful than either a left-to-right
model or the shallow concatenation of a left-toright and a right-to-left model. Unfortunately,
standard conditional language models can only be
trained left-to-right or right-to-left, since bidirectional conditioning would allow each word to indirectly “see itself”, and the model could trivially
predict the target word in a multi-layered context.

In order to train a deep bidirectional representation, we simply mask some percentage of the input
tokens at random, and then predict those masked
tokens. We refer to this procedure as a “masked
LM” (MLM), although it is often referred to as a
Cloze task in the literature [X]. In this
case, the final hidden vectors corresponding to the
mask tokens are fed into an output softmax over
the vocabulary, as in a standard LM. In all of our
experiments, we mask $15\%$ of all WordPiece tokens in each sequence at random. In contrast to
denoising auto-encoders [X], we
only predict the masked words rather than reconstructing the entire input.

Although this allows us to obtain a bidirectional pre-trained model, a downside is that we
are creating a mismatch between pre-training and
fine-tuning, since the [MASK] token does not appear during fine-tuning. To mitigate this, we do
not always replace “masked” words with the actual [MASK] token. The training data generator
chooses $15\%$ of the token positions at random for
prediction. If the i-th token is chosen, we replace
the i-th token with (1) the [MASK] token $80\%$ of
the time (2) a random token $10\%$ of the time (3)
the unchanged i-th token $10\%$ of the time. Then,
Ti will be used to predict the original token with
cross entropy loss. 

Many important downstream tasks such as Question Answering (QA) and Natural Language Inference (NLI) are based on understanding the relationship between two sentences, which is not directly captured by language modeling. In order
to train a model that understands sentence relationships, we pre-train for a binarized next sentence prediction task that can be trivially generated from any monolingual corpus. Specifically, when choosing the sentences A and B for each pretraining example, $50\%$ of the time B is the actual next sentence that follows A (labeled as IsNext),
and $50\%$ of the time it is a random sentence from
the corpus (labeled as NotNext). As we show
in Figure X, C is used for next sentence prediction (NSP). Despite its simplicity.

The NSP task is closely related to representationlearning objectives used in [X] and [X]. However, in prior
work, only sentence embeddings are transferred to
down-stream tasks, where BERT transfers all parameters to initialize end-task model parameters.

The pre-training procedure largely follows the existing literature on language model pre-training. For the pre-training corpus we
use the BooksCorpus (800M words) [X] and English Wikipedia (2,500M words).
For Wikipedia we extract only the text passages
and ignore lists, tables, and headers. It is critical to use a document-level corpus rather than a
shuffled sentence-level corpus such as the Billion
Word Benchmark [X] in order to
extract long contiguous sequences.

Fine-tuning is straightforward since the selfattention mechanism in the Transformer allows BERT to model many downstream tasks—
whether they involve single text or text pairs—by
swapping out the appropriate inputs and outputs.
For applications involving text pairs, a common
pattern is to independently encode text pairs before applying bidirectional cross attention, such
as Parikh et al. [X]; Seo et al [X]. BERT
instead uses the self-attention mechanism to unify
these two stages, as encoding a concatenated text
pair with self-attention effectively includes bidirectional cross attention between two sentences.

For each task, we simply plug in the taskspecific inputs and outputs into BERT and finetune all the parameters end-to-end. At the input, sentence A and sentence B from pre-training
are analogous to (1) sentence pairs in paraphrasing, (2) hypothesis-premise pairs in entailment, (3)
question-passage pairs in question answering, and (4) a degenerate text-∅ pair in text classification
or sequence tagging. At the output, the token representations are fed into an output layer for tokenlevel tasks, such as sequence tagging or question
answering, and the [CLS] representation is fed
into an output layer for classification, such as entailment or sentiment analysis.



==> PART_II_subs/dynamic.tex <==
\textbf{Dynamic Coattention Networks [X]}. 

==> PART_II_subs/global_local_attention.tex <==
\subsection{Encoder-Decoder Global and Local Attention}
\label{sec:global_local_attention}


%A LSTM Global and Local utiliza uma pilha de LSTMs dentro do framework clássico Encoder-Decoder (Figura X). A implemtação da LSTM adotada é a mesma proposta em [X].
The architecture uses an encoder-decoder framework and attention system (Figure \ref{fig:local_global_arquitetura}) for machine translation. The structure is similar to RNNSearch \cite{bahdanau_neural_2014} with the difference of simplifying the framework using a stack of LSTMs and using the hidden states at the top LSTM layers in both the encoder and decoder. First, the encoder generates the set of hidden states $h = \left \{ h_{1}, h_{2}, ..., h_{N} \right \}$, and at each time step $t$, the decoder generates a target hidden state $s_{j}$. Given $s_{j}$ and the source-side context vector $c_{t_{decoder}}$ a concatenation to combine both vectors to produce an predict hidden state $\hat{s_{j}}$. The attentional vector $s_{j}$ is then fed through the softmax layer to produce the predictive distribution. Specifically,

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{img/local_gobal_attention.pdf}
  \caption{Local and global attention.}
  \label{fig:local_global_arquitetura}
\end{figure}

\begin{equation}
    (h_{1}, ..., h_{N}) = Encoder(x_{1}, ..., x_{N})
    \label{encoder_global_local}
\end{equation}

\begin{equation}
    \hat{s_{j}} = tanh(W_{c}[c_{t_{decoder}};h_{t}])
    \label{encoder_global_local_1}
\end{equation}

\begin{equation}
    p(y_{t}|y_{<t},x) = softmax(W_{s}\hat{s_{j}})
    \label{encoder_global_local_2}
\end{equation}

The attentional system generates a context vector $c_{t_{decoder}}$ that captures relevant source-side information to predict the current target word $y_{t}$. Given the set of hidden states $h$ of the encoder as focus targets $\tau_{t} = \left \{ \tau_{t}^{1} \right \} = \left \{ \tau_{t,1}^{1}, ..., \tau_{t,N}^{1} \right \} = \left \{ h_{1}, ..., h_{N} \right \}$ and the context information $c_{t} = \left \{ c_{t}^{1} \right \} = \left \{ c_{t,1}^{1} \right \} = \left \{ s_{t} \right \}$ generated by the decoder at time $t$, the attentional system generates a weight of attention $a_{t} = \left \{ a_{t}^{1} \right \} = \left \{ a_{t,1}^{1}, ..., a_{t,N}^{1} \right \} = \left \{ a_{1}, ..., a_{N} \right \}$, for each vector annotation $h_{j}$, where $s_{t} \in \mathbb{R}^{1 \times d}$ is a previous decoder state, $h_{j} \in \mathbb{R}^{1 \times d}$ is encoder annotation vector, $a_{t}^{1} \in \mathbb{R}^{1 \times N}$ is the weight of attention to a hidden state $h_{j}$. 

If the attentional system implements global attention, there is only one subsystem, and the inputs are processed by an alignment function $a(s_{t}, h_{j})$ followed by normalization. This system is very similar to that of RNNSearch \cite{bahdanau_neural_2014} and has the same selection characteristics - soft, divided, stateful, location-based, top-down, and cognitive. However, other alignment functions experiment. Specifically,

\begin{equation}
    e_{t,j} = a(s_{t}, h_{j})
    \label{global_att_1}
\end{equation}

\begin{equation}
    e_{t,j} = \left\{\begin{matrix}
    s_{t}^{T}\bar{h_{j}}\\ 
    s_{t}^{T}W_{a}h_{j}\\ 
    v_{a}^{T}tanh(W_{a}[s_{t} || h_{j}])\\
    W_{a}s_{t}\\
    \end{matrix}\right.
    \label{global_att_2}
\end{equation}

\begin{equation}
    a_{t} = \frac{e^{score(h_{t},\bar{h_{s}})}}{\sum_{s^{'}}e^{score(h_{t},\bar{h_{s^{'}}})}}
    \label{global_att_3}
\end{equation}

\begin{equation}
    a_{j} = \frac{e^{e_{t,j}}}{\sum_{j = 1}^{N}e^{e_{t,j}}}
    \label{global_att_3}
\end{equation}

\noindent where $a$ is the alignment function, $e_{t,j}$ é o score value, $a_{j}$ is the weight of attention for an annotation vector $h_{j}$. 


Global attention uses all words on the source side for each word in the target, which is computationally expensive and can make it impractical to translate longer sentences. On the other hand, local attention chooses to focus only on a small subset of the original positions per target word. This mechanism is a tradeoff between hard and soft attention \cite{xu_show_2015}, and is differentiable. Local attention has the advantage of avoiding the expensive calculation, and at the same time, it is easier to train than hard attention. There are two cascading attention subsystems, the first is identical to global attention, and the second is responsible for changing the focus. Despite the changes, the mechanism has the same selection characteristics as global attention.

The local attention model initially generates an aligned position $p_{t}$ for each target word in time \textit{t}. The context vector $c_{t_{decoder}}$ is derived as a weighted average of the set of hidden states of the source within the window defined in the range $[p_{t} - D, p_{t} + D]$, where \textit{D} is chosen empirically. There are basically two types of alignment for $p_{t}$: monotonic alignment \textbf{(pt-m)} and predictive alignment \textbf {(local-p)}. In monotonic alignment, simply $p_{t} = t$, that is, it is assumed that source and destination sequences are approximately monotically aligned, and in predictive alignment the model predicts the alignment position, as follows

\begin{equation}
    p_{t} = S\cdot sigmoid(v_{p}^{T}tanh(W_{p},s_{t}))
    \label{local_att_w}
\end{equation}

\begin{equation}
    a_{j} = a_{j}e^{\frac{-(s - p_{t})^{2}}{2\sigma^{2}}}
    \label{local_att_gaussian}
\end{equation}

\noindent where $ W_{p} $ and $ v_{p} $ are the parameters of the model that will be learned to predict positions. \textit{S} is the size of the source sentence and $ p_{t} \in [0, S] $. To favor the alignment points close to $ p_{t} $, a Gaussian distribution centered around $ p_{t} $ is placed. The $ \sigma = \frac{D}{2} $, $ p_{t} $ is a real number, and \textit{s} is an integer with a window centered on $ p_{t} $. 




==> PART_II_subs/han.tex <==
\subsection{Hierarchical Attention Network (HAN)}
\label{sec:han}

HAN uses attention for document classification. The architecture consists of word encoder, sentence encoder, and attention system (Figure \ref{fig:han_arquitetura}). The word encoder, at each time step $t$, take as input a sentence $i$ with words $w_{i,j}$ with $j \in [1,N_{w}]$, and uses a bidirectional GRU \cite{bahdanau_neural_2014} to get annotations from both directions. The annotation vector $h_{i,j} = \left [ \overrightarrow{h_{i,j}}; \overleftarrow{h_{i,j}} \right ]$ for each word $w_{i,j}$ is the concatenation of the forward hidden state $\overrightarrow{h_{i,j}}$ and the backward hidden state $\overleftarrow{h_{i,j}}$. Similarly, the sentence encoder takes as input sentence vectors $s_{i}, i \in \left [ 1,N_{s} \right ]$, and uses a bidirectional GRU for produces vector annotations $h_{i} = \left [ \overrightarrow{h_{i}}; \overleftarrow{h_{i}} \right ]$ for summarizes the neighbor around sentence $i$.


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{img/han.pdf}
  \caption{Hierarchical Attention Networks. Word attention extracts such words that are important to the meaning of the sentence and aggregate the representation of those informative words to form a sentence vector. Similarly, sentence attention  reward sentences that are clues to correctly classify a document.}
  \label{fig:han_arquitetura}
\end{figure}


The attentional system captures the hierarchical structure of the document, since words and phrases are differentially informative depending on the context. Intuitively, attention allows the model to give more or less importance to individual words and sentences when building the representation of a document. To include sensitivity to this fact, it has two identical subsystems -- word attention and sentence attention. Word attention generates a dynamic context vector at the word level, and takes as input a contextual $c_{t} = \left \{ c_{t}^{1} \right \} = \left \{ c_{t,1}^{1} \right \} = \left \{ u_{w} \right \}$, a focus target $\tau_{t} = \left \{ \tau_{t}^{1} \right \} = \left \{ \tau_{t,1}^{1}, ..., \tau_{t,N_{w}}^{1} \right \} = \left \{ h_{i,1}, ..., h_{i,N_{w}} \right \}$, and produces attention weights $a_{t} = \left \{ a_{t}^{1} \right \} = \left \{ a_{t,1}^{1}, ..., a_{t,N_{w}}^{1} \right \} = \left \{ a_{1}, ..., a_{N_{w}} \right \}$ as output, where $u_{w} \in \mathbb{R}^{1 \times d}$ is the context vector that can be seen as a high level representation of a query ``what is the informative word?'', $h_{i,j} \in \mathbb{R}^{1 \times d}$ is word encoder annotation vector, $a_{t}^{1} \in \mathbb{R}^{1 \times N_{w}}$ is the weight of attention to a hidden state $h_{i,j}$. Such inputs are processed by alignment function $e_{i,j} = tanh(W_{w}h_{i,j} + b_{w})^{T}u_{w}$ to obtain a set scores $e_{i,j}$ that reflects the importance of $h_{i,j}$ with respect $u_{w}$ in deciding of those informative words to form a sentence vector. The scores are normalized through a softmax function, so as to obtain a set of weights $a_{j} = \frac{ exp(e_{i,j}) }{ \sum_{j=1}^{N_{w}} exp(e_{i,j})}$. Finally, a sentence vector $s_{i} \sum_{j=1}^{N_{w}} a_{j}h_{i,j}$ is computed as a weighted sum of the word annotations.


Both subsystems are very similar to RNNSearch's attention \cite{bahdanau_neural_2014}, also presenting the same selection characteristics - soft, divided, stateful, location-based, top-down, and cognitive. However, sentence attention rewards sentences that are tips for correctly classifying a document. It again uses the same alignment function and other contextual information (i.e., sentence level context vector $u_{s}$) to generate a document vector $v$ which summarizes all sentences informations. Finally, $v$ is input for document classification layers. Note that the two subsystems are internally equal but the context and focus target determine different actions, demonstrating the plasticity of the attentional interfaces.


%\begin{equation}
%c_{t} = \left \{ c_{t}^{1} \right \} = \left \{ c_{t,1}^{1} \right \} = \left %\{ u_{w} \right \}
%\end{equation}

%\begin{equation}
%\tau_{t} = \left \{ \tau_{t}^{1} \right \} = \left \{ \tau_{t,1}^{1}, ..., %\tau_{t,N_{w}}^{1} \right \} = \left \{ h_{i,1}, ..., h_{i,N_{w}} \right \}
%\end{equation}

%\begin{equation}
%    a_{t} = \left \{ a_{t}^{1} \right \} = \left \{ a_{t,1}^{1}, ..., %a_{t,N_{w}}^{1} \right \} = \left \{ a_{1}, ..., a_{N_{w}} \right \}
%\end{equation}



  





%\begin{equation}
%    e_{i,s} = a(h_{i}, u_{s})
%    \label{reward_1}
%\end{equation}

%\begin{equation}
%    e_{i,s} = tanh(W_{w}h_{i} + b_{w})^{T}u_{s} 
%    \label{reward_2}
%\end{equation} 

%\begin{equation}
%    a_{j} = \frac{ exp(e_{i,s}) }{ \sum_{i=1}^{N_{s}} exp(e_{i,s})}
%    \label{reward_3}
%\end{equation} 

%\begin{equation}
%    v = \sum_{i=1}^{N_{s}} a_{j}h_{i}
%    \label{reward_4}
%\end{equation}

%\noindent where $v$ is the document vector that summarizes all the information %of sentences in a document, and .

%Finally, the document vector $v$ can be used as features for document %classification:

%\begin{equation}
%    p = softmax(W_{c}v + b_{c})
%    \label{reward_4}
%\end{equation}




==> PART_II_subs/pointer_network.tex <==
\subsection{Pointer Networks (Ptr-Nets)}
\label{sec:pointer_network}

%A Pointer Networks (Ptr-Nets) é um modelo do tipo sequence-to-sequence em que a saída são tokens discretos correspondentes às posições em uma sequência de entrada. Existem duas diferenças principais entre essa arquitetura e as seq2seq clássicas. A Primeira é que a saída da Ptr-Nets é discreta e corresponde às posições na sequência de entrada. Além disso, o número de classes de destino em cada etapa da saída depende do comprimento da entrada, que é variável. Esse tipo de abordagem é ideal para problemas de classificação, ordenaçÃo de palavras, problemas linguísticos computacionais como o convex hull e o problema do vendedor ambulante. 
Pointer Networks \cite{vinyals2015pointer} uses attention for approximate solutions to challenging geometric problems. The architecture is a sequence-to-sequence model with two main differences -- uses attention as a pointer to select input as output, and the number of target classes depends on the input's length, which is variable. The classic sequece-to-sequence model receives as input a pair $\left ( P,C^{P} \right )$ and computes the conditional probability $P\left ( C^{P}|P;\theta \right ) = \prod_{i=1}^{m\left ( P \right )} P\left ( C_{i} | C_{1}, ..., C_{i-1}, P; \theta \right )$, where $P = \left \{ P_{1}, ..., P_{N} \right \}$ is a sequence of $N$ vectors, $C^{P} = \left \{ C_{1}, ..., C_{m\left ( P \right )} \right \}$ is a sequence of $m\left ( P \right )$ indexes, each between 1 and $N$, and $\theta$ is RNN's parameters. During the inference the model predicting the optimal sequence $\widehat{C}^{P}$ with highest probability, i.e., 
$\widehat{C}^{P} = \argmax\limits_{C^{P}} p\left ( C^{P}|P;\theta^{*} \right )$. The combinatorial number of possible output sequences makes it computationally impractical find the optimal sequence $C^{P}$, and it is not possible to learn solutions that have the size of the output dictionary dependent on the size of the input. Instead, Ptr-Net uses an attention system to find the best possible sequence given a beam size. 

Ptr-Net consists of three main components - the attentional system, the encoder, and the decoder. 
The attentional system has two subsystems. The first takes as a focus target $\tau_{t} = \left \{ \tau_{t}^{1} \right \} = \left \{ \tau_{t,1}^{1}, ..., \tau_{t,N}^{1} \right \} = \left \{ h_{1}, ..., h_{N} \right \}$ all hidden states of the encoder, and as contextual input $c_{t} = \left \{ c_{t}^{1} \right \} = \left \{ c_{t,1}^{1} \right \} = \left \{ s_{t} \right \}$ the hidden state of the decoder in time $t$. 
Inputs through $a$ alignment function and normalization generating attentional weights that represent $p(C_{i} | C_{1}, ..., C_{i-1}, P)$. This subsystem makes a \textbf{oriented}, \textbf{soft}, \textbf{divided}, \textbf{cognitive}, \textbf{location-based}, and \textbf{top-down statefull} selection similar to RNNSearch \cite{bahdanau_neural_2014}. The second subsystem performs a \textbf{hard selection} taking as input the same focus target $\tau_{t}$ and as contextual input the attentional mask of the previous subsystem, that is, $c_{t} = \left \{ c_{t}^{1} \right \} = \left \{ c_{t,1}^{1} \right \} = \left \{ u_{t} \right \}$, outputting a binary mask $ a_{t} $ which is one only in the position of the highest value context vector, and zero in the other positions. Intuitively, the hard mechanism makes the attentional system a pointer and makes it possible to use dictionaries of varying sizes. Specifically, 


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{img/pointer_networks.pdf}
  \caption{Pointer Networks Architecture. An encoding RNN (pink) converts the input sequence, and at each step $t$, the decoder network (green) produces a vector that modulates a content-based attention mechanism over inputs. The output's attention system is a softmax distribution with a dictionary size equal to the input length.}
  \label{fig:pointer_networks_arquitetura}
\end{figure}


\begin{equation}
    u_{t,j} = v^{T}tanh(W_{1}h_{j} + W_{2}s_{t}) 
    \label{reward_0}
\end{equation}

\begin{equation}
    p(C_{i}|C_{1},...,C_{i-1},P) = softmax(u)
    \label{reward_1}
\end{equation}

\noindent where softmax normalizes the vector $u \in \mathbb{R}^{N}$ to be an output distribution over the dictionary of inputs, $v$, $W_{1}$, and $W_{2}$ are parameters of the model.



==> PART_II_subs/spatial_transformer.tex <==
%\subsection{Spatial Transformer}
%\label{sec:spatial_transformer}


\textbf{Spatial Transformer (STN)}. Spatial Transformer consists of three main parts (Figure X): the localization network, the grid generator and the sampler. The localization network takes the feature map from the input and, through several layers, produces the spatial transformation parameters that must be applied to the feature map. Then the learned transformation parameters are used to create a sampling grid, which is a set of points at which the input map must be sampled to produce the transformed output. This process is done by the grid generator. Finally, the feature map and the sampling grid are taken as inputs to the sampler, producing the sampled output map.

O localisation network recebe como entrada um feature map The localisation network takes the input feature map U ∈ R
H×W×C with width W, height H and
C channels and outputs θ, the parameters of the transformation Tθ to be applied to the feature map:
θ = floc(U). The size of θ can vary depending on the transformation type that is parameterised,
e.g. for an affine transformation θ is 6-dimensional as in (10).
The localisation network function floc() can take any form, such as a fully-connected network or
a convolutional network, but should include a final regression layer to produce the transformation
parameters θ.
















O módulo da Spatial Transformer consiste de três componentes principais (Figure X): a localisation network, a grid generator e a sampler. 

O objetivo da localisation network é aprender os parâmetros da transformação afim que serão aplicados nos feature maps da entrada (Figura X). Ou seja, ela pega o feature map de entrada $U \in \mathbb{R}^{F \times W \times C}$ e a saída é uma matriz $\theta \in \mathbb{R}^{2 \times 3}$ com os parâmetros da transformação $\tau_{\theta}$:

\begin{equation}
    \theta = f_{loc}(U)
    \label{spatial_localisation}
\end{equation}

$U \in \mathbb{R}^{F \times W \times C}$, $\theta \in \mathbb{R}^{2 \times 3}$. \textit{H} é a largura, \textit{W} é a altura e \textit{C} é o número de canais do feature map. A função de localisation $f_{loc}$ pode assumir qualquer formato, ela pode ser uma rede totalmente conectada ou uma rede convolucional, mas deve incluir uma camada de regressão final para produzir os parâmetros $\theta$.

A função do grid generator é gerar uma grade de amostragem parametrizada, que é um conjunto de pontos nos quais o mapa de entrada deve ser amostrado para produzir a saída transformada desejada. Nesse módulo os pixels da saída são definidos 




Parametrised Sampling Grid
The grid generator’s job is to output a parametrised sampling grid, which is a set of points where the input map should be sampled to produce the desired transformed output.

Concretely, the grid generator first creates a normalized meshgrid of the same size as the input image U of shape (H, W), that is, a set of indices that cover the whole input feature map (the subscript t here stands for target coordinates in the output feature map). Then, since we’re applying an affine transformation to this grid and would like to use translations, we proceed by adding a row of ones to our coordinate vector to obtain its homogeneous equivalent. This is the little trick we also talked about last week. Finally, we reshape our 6 parameter to a 2x3 matrix and perform the following multiplication which results in our desired parametrised sampling grid.

The column vector consists in a set of indices that tell us where we should sample our input to obtain the desired transformed output.

But wait a minute, what if those indices are fractional? Bingo! That’s why we learned about bilinear interpolation and this is exactly what we do next.

Differentiable Image Sampling
Since bilinear interpolation is differentiable, it is perfectly suitable for the task at hand. Armed with the input feature map and our parametrised sampling grid, we proceed with bilinear sampling and obtain our output feature map V of shape (H’, W’, C’). Note that this implies that we can perform downsampling and upsampling by specifying the shape of our sampling grid. (take that pooling!) We definitely aren’t restricted to bilinear sampling, and there are other sampling kernels we can use, but the important takeaway is that it must be differentiable to allow the loss gradients to flow all the way back to our localisation network.

The above illustrates the inner workings of the Spatial Transformer. Basically it boils down to 2 crucial concepts we’ve been talking about all week: an affine transformation followed by bilinear interpolation. Take a moment and admire the elegance of such a mechanism! We’re letting our network learn the optimal affine transformation parameters that will help it ultimately succeed in the classification task all on its own.








==> PART_II_subs/summary.tex <==
\textbf{Summary}. PERGUNTAR 

==> PART_II_subs/two_away.tex <==
%\subsection{Two-Away Attention}
%\label{sec:two_away_attention}

\textbf{Two-Away Attention [X]}. Recurrent neural networks (RNNs) with long short-term memory (LSTM) units have been successfully applied to a wide range of NLP tasks, such as machine
translation, constituency parsing, language modeling and recently RTE. LSTMs encompass memory cells that can store information for a long period of time, as well as three types of gates that control the flow of information into and out of these cells: input gates, forget gates and output gates. Given an input vector $x_{t}$ at time step \textit{t}, the previous output $h_{t−1}$ and cell state $c_{t−1}$, an LSTM with hidden size \textit{k} computes the next output $h_{t}$ and cell state $c_{t}$ as:

\begin{equation}
    H = \begin{bmatrix}
    x_{t}\\ 
    h_{t-1}
    \end{bmatrix}
    \label{annotations}
\end{equation}

\begin{equation}
    i_{t} = \sigma(W^{i}H + b^{i})
    \label{annotations}
\end{equation}

\begin{equation}
    f_{t} = \sigma(W^{f}H + b^{f})
    \label{annotations}
\end{equation}

\begin{equation}
    o_{t} = \sigma(W^{o}H + b^{o})
    \label{annotations}
\end{equation}

\begin{equation}
    c_{t} = f_{t} \odot c_{t-1} + i_{t} \odot tanh(W^{c}H+b^{c})
    \label{annotations}
\end{equation}

\begin{equation}
    h_{t} = o_{t} \odot tanh(c_{t})
    \label{annotations}
\end{equation}

where $W^{i}, W^{f}, W^{o}, W^{c} \in \mathbb{R}^{2k \times k}$ are trained matrices and $b^{i}, b^{f}, b^{o}, b^{c} \in \mathbb{R}^{k}$ trained biases that parameterize the gates and transformations of the input, $\sigma$ denotes the element-wise application of the sigmoid function and $\odot$ the element-wise multiplication of two vectors.

In contrast to learning sentence representations, we are interested in neural models that read both sentences to determine entailment, thereby reasoning over entailments of pairs of words and phrases. Figure X shows the high-level structure of this model. The premise (left) is read by an LSTM. A second LSTM with different parameters is reading a delimiter and the hypothesis (right), but its memory state is initialized with the last cell state of the previous LSTM (c5 in the example), i.e. it is conditioned on the representation that the first LSTM built for the premise (A). We use word2vec vectors [X] as word representations, which we do not optimize during training. Out-of-vocabulary words in the training set are randomly initialized by sampling values uniformly from (−0.05, 0.05) and optimized during training.1 Out-of-vocabulary words encountered at inference
time on the validation and test corpus are set to fixed random vectors. By not tuning representations of words for which we have word2vec vectors, we ensure that at inference time their representation stays close to unseen similar words for which we have word2vec embeddings. We use a linear layer
to project word vectors to the dimensionality of the hidden size of the LSTM, yielding input vectors $x_{i}$. Finally, for classification we use a softmax layer over the output of a non-linear projection of the last output vector (h9 in the example) into the target space of the three classes (ENTAILMENT, NEUTRAL or CONTRADICTION), and train using the cross-entropy loss.

Attentive neural networks have recently demonstrated success in a wide range of tasks ranging from handwriting synthesis [X], digit classification [X], machine translation [X], image captioning [X], speech recognition [X] and sentence summarization [X], to geometric reasoning [X].
The idea is to allow the model to attend over past output vectors, thereby mitigating the LSTM’s cell state bottleneck. More precisely, an LSTM with attention for RTE does not need to capture the whole semantics of the premise in its cell state. Instead, it is sufficient to output vectors
while reading the premise and accumulating a representation in the cell state that informs the second LSTM which of the output vectors of the premise it needs to attend over to determine the RTE class.

Let Y $\in \mathbb{R}^{k \times L}$ be a matrix consisting of output vectors $[h_{1}, ..., h_{L}]$ that the first LSTM produced
when reading the L words of the premise, where \textit{k} is a hyperparameter denoting the size of embeddings and hidden layers. Furthermore, let e \textit{L} $\in \mathbb{R}^{L}$ be a vector of 1s and $h_{N}$ be the last output
vector after the premise and hypothesis were processed by the two LSTMs respectively. The attention mechanism will produce a vector $\alpha$ of attention weights and a weighted representation \textit{r} of the
premise via:

\begin{equation}
    M = tanh(W^{y}Y + W^{h}h_{N} \otimes e_{L})
    \label{annotations}
\end{equation}

\begin{equation}
    \alpha = softmax(W^{T}M)
    \label{annotations}
\end{equation}

\begin{equation}
    r = Y\alpha^{T}
    \label{annotations}
\end{equation}

where $W^{y}, W^{h} \in \mathbb{R}^{k \times k}$ are trained projection matrices, $W \in \mathbb{R}^{k}$ is a trained parameter vector and
$W^{T}$ denotes its transpose. Note that the outer product $W^{h}h_{N} \otimes e_{L}$ is repeating the linearly transformed $h_{N}$ as many times as there are words in the premise (i.e. \textit{L} times). Hence, the intermediate attention representation $m_{i}$ ($i_{th}$ column vector in \textit{M}) of the $i_{th}$ word in the premise is obtained from a non-linear combination of the premise's output vector $h_{i}$ ($i_{th}$ column vector in \textit{Y}) and the transformed $h_{N}$ . The attention weight for the $i_{th}$ word in the premise is the result of a weighted
combination (parameterized by w) of values in $m_{i}$.

The final sentence-pair representation is obtained from a non-linear combination of the attention weighted representation \textit{r} of the premise and the last output vector $h_{N}$ using

\begin{equation}
    h^{*} = tanh(W^{p}r + W^{x}h_{N})
    \label{annotations}
\end{equation}

where $h^{*} \in \mathbb{R}^{k}, W^{p}, W^{x} \in \mathbb{R}^{k \times k}$ are trained projection matrices.

For determining whether one sentence entails another it can be a good strategy to check for entailment or contradiction of individual word- and phrase-pairs. To encourage such behavior we employ neural word-by-word attention similar to [X], [X] and [X]. The difference is that we do not use attention to generate words, but to obtain a sentence-pair encoding from fine-grained reasoning via soft-alignment of words and phrases in
the premise and hypothesis. In our case, this amounts to attending over the first LSTM’s output vectors of the premise while the second LSTM processes the hypothesis one word at a time, thus generating attention weight-vectors αt over all output vectors of the premise for every word $x_{t}$ with
\textit{t} $\in (L + 1, N)$ in the hypothesis (Figure X). This can be modeled as follows:

\begin{equation}
    M = tanh(W^{y}Y + (W^{h}h_{t} + W^{r}t_{t-1}) \otimes e_{L})
    \label{annotations}
\end{equation}

\begin{equation}
    \alpha_{t} = softmax(W^{T}M_{t})
    \label{annotations}
\end{equation}

\begin{equation}
    r_{t} = Y\alpha^{T}_{t} + tanh(W^{T}r_{t-1})
    \label{annotations}
\end{equation}

Note that $r_{t}$ is dependent on the previous attention representation $r_{t−1}$ to inform the model about what was attended over in the previous step.

As in the previous section, the final sentence-pair representation is obtained from a non-linear combination of the last attention-weighted representation of the premise (here based on the last word of
the hypothesis) $r_{N}$ and the last output vector using

\begin{equation}
    h^{*} = tanh(W^{p}r_{N} + W^{x}h_{N})
    \label{annotations}
\end{equation}

where $h^{*} \in \mathbb{R}^{k}$.



==> PART_I_ATT_DL.tex <==
\section{Attention in Deep Learning}
\label{sec:attention_in_deep_learning}


\newpage
\input{PART_I_subs/overview}
\input{PART_I_subs/attention_mechanisms}
\input{PART_I_subs/attention_based_classic}








==> PART_I_subs/attention_based_classic.tex <==
\section{Attention-based Classic Deep Learning Architectures}
\label{sub:attention_classic_architectures}

This section introduces details about attentional interfaces in classic DL architectures. Specifically, we present the uses of attention in convolutional, recurrent networks and generative models.


\input{PART_I_subs/attention_based_cnns}
\input{PART_I_subs/attention_based_rnns}
\input{PART_I_subs/attention_based_generative}

==> PART_I_subs/attention_based_cnns.tex <==
%esther: check 1

\subsection{Attention-based Convolutional Neural Networks (CNNs)}
\label{attention_cnns}
Attention emerges in CNNs to filter information and allocate resources to the neural network efficiently. There are numerous ways to use attention on CNNs, which makes it very difficult to summarize how this occurs and the impacts of each use. We divided the uses of attention into six distinct groups (Figure \ref{fig:dcn_atention}): 1) DCN attention pool -- attention replaces the classic CNN pooling mechanism; 2) DCN attention input -- the attentional modules are filter masks for the input data. This mask assigns low weights to regions irrelevant to neural network processing and high weights to relevant areas; 3) DCN attention layer -- 
attention is between the convolutional layers; 4) DCN attention prediction -- attentional mechanisms assist the model directly in the prediction process; 5) DCN residual attention --  extracts information from the feature maps and presents a residual input connection to the next layer; 6) DCN attention out -- attention captures important stimuli of feature maps for other architectures, or other instances of the same architecture. To maintain consistency with the Deep Neural Network's area, we extend \textbf{The Neural Network Zoo} schematics\footnote{The Neural Network Zoo link: \url{https://www.asimovinstitute.org/neural-network-zoo/}} to accommodate attention elements. 
        

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.95\linewidth]{img/dcn_atencao_family.pdf}
\caption{Attention-based convolutional neural networks. DCN attention pool group uses an attention pool, instead of regular pooling, as a strategy to determine the importance of each individual in a given feature map window. The premise is that only a few of these windows are significant and must be selected concerning a particular objective. DCN attention input group uses structures similar to the human's visual attention. DCN attention layer group collects important stimuli of high (semantic level) and low level (saliency) for subsequent layers of architecture. DCN attention prediction group uses attention in the final stages of prediction, sometimes as an ensemble element. DCN residual attention group uses attention as a residual module between any convolutional layers to mitigate the vanishing problem, capturing only the relevant stimuli from each feature map. DCN attention out-group can represent the category of recurrent attention processes.}
\label{fig:dcn_atention}
\end{center}
\end{figure}

%falar aqui de algumas motivações e usos para incluir atenção em CNNs - learn to pay attention

 \textbf{DCN attention input} mainly uses attention to filter input data - a structure similar to the multi-glimpse mechanism and visual attention of human beings. Multi-glimpse refers to the ability to quickly scan the entire image and find the main areas relevant to the recognition process, while visual attention focuses on a critical area by extracting key features to understand the scene. When a person focuses on one part of the image, the different regions' internal relationship is captured, guiding eye movement to find the next relevant area—ignoring the irrelevant parts easy learning in the presence of disorder. For this reason, human vision has an incomparable performance in object recognition. The main contribution of attention at the CNNs' input is robustness. If our eyes see an object in a real-world scene, parts far from the object are ignored. Therefore, the distant background of the fixed object does not interfere in recognition. However, CNNs treat all parts of the image equally. The irrelevant regions confuse the classification and make it sensitive to visual disturbances, including background, changes in camera views, and lighting conditions. Attention in CNNs' input contributes to increasing robustness in several ways: 1) It makes architectures more scalable, in which the number of parameters does not vary linearly with the size of the input image; 2) Eliminates distractors; 3) Minimizes the effects of changing camera lighting, scale, and views. 4) It allows the extension of models for more complex tasks, i.e., fine-grained classification or segmentation. 5) Simplifies CNN encoding. 6) Facilitates learning by including relevant priorities for architecture.

% falo das abordagens da DCN Attention Input - 1 parágrafo

Zhao et al. \cite{zhao_deep_2017} used visual attention-based image processing to generate the focused image. Then, the focused image is input into CNN to be classified. According to the classification, the information entropy guides reinforcement learning agents to achieve a better image classification policy. Wang et al. \cite{x._wang;_l._gao;_j._song;_h._shen_beyond_2017} used attention to create representations rich in motion information for action recognition. The attention extracts saliency maps using both motion and appearance information to calculate the objectness scores. For a video, attention process frame by frame to generate a saliency-aware map for each frame. The classic pipeline uses only CNN sequence features as input for LSTMs, failing to capture adjacent frames' motion information. The saliency-aware maps capture only regions with relevant movements making CNN encoding simple and representative for the task. Liu et al. \cite{ning_liu;yongchao_long;changqing_zou;qun_niu;li_pan;hefeng_wu_adcrowdnet:_2019} used attention as input of a CNN to provide important priors in counting crowded tasks. An attention map generator first provides two types of priors for the system: candidate crowd regions and crowd regions' congestion degree. The priors guide subsequent CNNs to pay more attention to those regions with crowds and improving their capacity to be resistant to noise. Specifically, the congestion degree prior provides fine-grained density estimation for a system.

% DCN attention layer - 

In classic CNNs, the size of the receptive fields is relatively small. Most of them extract features locally with convolutional operations, which fail to capture long-range dependencies between pixels throughout the image. However, larger receptive fields allow for better use of training inputs, and much more context information is available at the expense of instability or even convergence in training. Also, traditional CNNs treat channel features equally. This naive treatment lacks the flexibility to deal with low and high-frequency information. Some frequencies may contain more relevant information for a task than others, but equal treatment by the network makes it difficult to converge the models. To mitigate such problems, most literature approaches use attention between convolutional layers (i.e., \textbf{DCN attention layer} and \textbf{DCN residual attention}), as shown in figure \ref{fig:dcns_architectures}.  Between layers, attention acts mainly for feature recalibration, capturing long-term dependencies, internalizing, and correctly using past experiences.


The pioneering approach to adopting attention between convolutional layers is the Squeeze-and-Excitation Networks \cite{hu_squeeze-and-excitation_2017} created in 2016 and winner of the ILSVRC in 2017. It is also the first architecture to model channel interdependencies to recalibrate filter responses in two steps, squeeze and excitation, i.e., SE blocks. To explore local dependencies, the squeeze module encodes spatial information into a channel descriptor. The output is a collection of local descriptors with expressive characteristics for the entire image. To make use of the information aggregated by the squeeze operation, excitation captures channel-wise dependencies by learning a non-linear and non-mutually exclusive relationship between channels, ensuring that multiple channels can be emphasized. In this sense, SE blocks intrinsically introduce attentional dynamics to boost feature discrimination between convolutional layers.


\begin{figure}[h]
\begin{center}
    \includegraphics[width=1\linewidth]{img/todas_as_dcns.pdf}
\caption{Attention-based convolutional neural networks main architectures by task and attention use.}
\label{fig:dcns_architectures}
\end{center}
\end{figure}

The inter-channel and intra-channel attention to capturing long-term dependencies and simultaneously taking advantage of high and low-level stimuli are widely explored in the literature. Zhang. et al. \cite{zhang2019residual} proposed residual local and non-local attention
blocks consisting of trunk and mask branches. Their attention mechanism helps to learn local and non-local information from the hierarchical features, further preserving low-level features while maintaining a representational quality of high-level features. The Cbam \cite{sanghyun_woo;jongchan_park;joon-young_lee;in_so_kweon_cbam:_2018} infers attentional maps in two separate dimensions, channel and spatial, for adaptive feature refinement. The double attention block in \cite{chen_^2-nets:_2018} aggregates and propagates global informational features considering the entire spatio-temporal context of images and videos, allowing subsequent convolution layers to access resources from across space efficiently. In the first stage, attention gathers features from all space into a compact set employing groupings. In the second stage, it selects and adaptively distributes the resources for each architectural location. Following similar exploration proposals, several attentional modules can be easily plugged into classic CNNs \cite{fukui2019attention}\cite{han20193dviewgraph}\cite{ji2017distant}\cite{yang2017neural}.


% parágrafo 1 DCN attention layer

Hackel et al. \cite{hackel_inference_2018} explored attention to preserving sparsity in convolutional operations. Convolutions with kernels greater than $1 \times 1$ generate fill-in, reducing feature maps' sparse nature. Generally, the change in data sparsity has little influence on the network output, but memory consumption and execution time considerably increase when it occurs in many layers. To guarantee low memory consumption, attention acts as a $k-selection$ filter, which has two different versions of selection: 1) it acts on the output of the convolution, preferring the largest $k$ positive responses similar to a rectified linear unit; 2) it chooses the $k$ highest absolute values, expressing a preference for responses of great magnitude. The parameter $k$ controls the level of sparse data and, consequently, computational resources during training and inference. Results point out that training with attentional control of data sparsity can reduce in more than $200\%$ the forward pass runtime in one layer.


To previous aggregate information and dynamically point to past experiences, SNAIL \cite{mishra_simple_2017} - a pioneering class of meta-learner based attention architectures - has proposed combining temporal convolutions with soft attention. This approach demonstrates that attention acts as a complement to the disadvantages of convolution. Attention allows precise access in an infinitely large context, while convolutions provide high-bandwidth access at the expense of a finite context. By merging convolutional layers with attentional layers, SNAIL can have unrestricted access to the number of previous experiences effectively, as well as the model can learn a more efficient representation of features. As additional benefits, SNAIL architectures become simpler to train than classic RNNs.

% DCN attention out
The \textbf{DCN attention out-group} uses attention to share relevant feature maps with other architectures or even with instances of the current architecture. Usually, the main objective is to facilitate the fusion of features, multimodality, and external knowledge. In some cases, attention regularly works by turning classic CNNs into recurrent convolutional neural networks - a new trend in Deep Learning to deal with challenging images' problems. RA-CNN \cite{fu_look_2017} is a pioneering framework for recurrent convolutional networks. In their framework, attention proceeds along two dimensions, i.e., discriminative feature learning and sophisticated part localization. Given an input image, a classic CNN extracts feature maps, and the attention proposal network maps convolutional features to a feature vector that could be matched with the category entries. Then, attention estimates the focus region for the next CNN instance, i.e., the next finer scale. Once the focus region is located, the system cuts and enlarges the region to a finer scale with higher resolution to extract more refined features. Thus, each CNN in the stack generates a prediction so that the stack's deepest layers generate more accurate predictions.

For merging features, Cheng. et. al. \cite{xueying_chen;rong_zhang;pingkun_yan_feature_2019} presented Feature-fusion Encoder-Decoder Network (FED-net) to image segmentation. Their model uses attention to fuse features of different levels of an encoder. At each encoder level, the attention module merges features from its current level with features from later levels. After the merger, the decoder performs convolutional upsampling with the information from each attention level, which contributes by modulating the most relevant stimuli for segmentation. Tian et al. \cite{tian2018learning} used feature pyramid-based attention to combine meaningful semantic features with semantically weak but visually strong features in a face detection task. Their goal is to learn more discriminative hierarchical features with enriched semantics and details at all levels to detect hard-to-detect faces, like tiny or partially occluded faces. Their attention mechanism can fuse different feature maps from top to bottom recursively by combining transposed convolutions and element-wise multiplication maximizing mutual information between the lower and upper-level representations.

%por uma coisa de transfer learning e por uma coisa de multimodalidade
Delta \cite{xingjian_li;haoyi_xiong;hanchao_wang;yuxuan_rao;liping_liu;jun_huan_delta:_2019} framework presented an efficient strategy for transfer learning. Their attention system acts as a behavior regulator between the source model and the target model. The attention identifies the source model's completely transferable channels, preserving their responses and identifying the non-transferable channels to dynamically modulate their signals, increasing the target model's generalization capacity. Specifically, the attentional system characterizes the distance between the source/target model through the feature maps' outputs and incorporates that distance to regularize the loss function. Optimization normally affects the weights of the neural network and assigns generalization capacity to the target model. Regularization modulated by attention on high and low semantic stimuli manages to take important steps in the semantic problem to plug in external knowledge.


The \textbf{DCN attention prediction} group uses attention directly in the prediction process. Various attentional systems capture features from different convolutional layers as input and generate a prediction as an output. Voting between different predictors generates the final prediction. Reusing activations of CNNs feature maps to find the most informative parts of the image at different depths makes prediction tasks more discriminative. Each attentional system learns to relate stimuli and part-based fine-grained features, which, although correlated, are not explored together in classical approaches. Zheng et al. \cite{zheng2017learning} proposed a multi-attention mechanism to group channels, creating part classification sub-networks. The mechanism takes as input feature maps from convolutional layers and generates multiple single clusters spatially-correlated subtle patterns as a compact representation. The sub-network classifies an image by each individual part. The attention mechanism proposed in \cite{rodriguez_painless_2018} uses a similar approach. However, instead of grouping features into clusters, the attentional system has the most relevant feature map regions selected by the attention heads. The output heads generate a hypothesis given the attended information, and the confidence gates generate a confidence score for each attention head.

% DCN attention pool - falar e falar do DCN attention input
Finally, the \textbf{DCN attention pool} group replaces classic pooling strategies with attention-based pooling. The objective is to create a non-linear encoding to select only stimuli relevant to the task, given that classical strategies select only the most contrasting stimuli. To modulate the resulting stimuli, attentional pooling layers generally capture different relationships between feature maps or between different layers. For example, Wang et al. \cite{linlin_wang_zhu_cao_gerard_de_melo_zhiyuan_liu:_relation_nodate} created an attentional mechanism that captures pertinent relationships between convoluted context windows and the relation class embedding through a correlation matrix learned during training. The correlation matrix modulates the convolved windows, and finally, the mechanism selects only the most salient stimuli. A similar approach is also followed in \cite{yin2016abcnn} for modeling sentence pairs.






% falar da recorrencia como um processo DCN attention out 
%4) DCN Attention Recurrent Input -- represents the category of recurrent attention processes. The mechanism generates the attentional mask using the features maps from some layers of the convolutional network. It later applies this mask to the input by selecting an area of interest. This region of interest is an entry for a new classifier;

%Todo, falta indicar de onde vem essa imagem. Adaptada de onde? Indicar que vamos seguir uma variante desta notacao.
%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.7\linewidth]{img/cnn_classica_zoo%.jpg}
%\caption{Classic CNNs architectures.}
%\label{fig:cnns_classic}
%\end{center}
%\end{figure}

%\subsubsection{\textbf{DCN Attention}}
%\label{sub:dcn_att}

%To analyze the use of attention modules in the DCNs, we %selected the most impactful works for this proposal (Figure %\ref{fig:dcns_architectures}). Regarding how attention is %implemented in classic architectures, DCNs can be of the type 

%todo: explicar o caption
%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.95\linewidth]{img/dcn_attention_architectures.jpg%}
%\caption{Attention CNNs.}
%\label{fig:dcns_architectures}
%\end{center}
%\end{figure}

%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.95\linewidth]{img/dcn_attention_t%ypes.jpg}
%\caption{DCN Attention architectures.}
%\label{fig:dcn_attention_types}
%\end{center}
%\end{figure}

%\subsubsection*{\textbf{DCN Attention Pool}}
%No DCN Attention Pool mecanismo atencional substitui o mecanismo clássico de pooling da CNN. Em vez de um pooling regular, usa-se um pool de atenção como estratégia para determinar a importância de cada indivíduo em uma determinada janela do feature map. A premissa é de que apenas algumas dessas janelas são realmente significativas e devem ser selecionadas com respeito à um determinado objetivo. 


%No DCN Attention Input os módulos atencionais são máscaras de filtragem dos dados de entrada. Essa máscara atribui pesos baixos a regiões que são irrelevantes para o processamento da rede neural e pesos altos para regiões relevantes. Essa estrutura é similar ao mecanimo visual de multiglimpse e atenção visual dos seres humanos. O mecanismo de atenção visual humano possui capacidade de explorar diferenças locais em uma imagem e destacar as principais partes. Isso significa que uma pessoa concentra atenção em uma parte da imagem por vez, e o multiglimpse se refere a capacidade de digitalizar rapidamente toda a imagem e encontrar as principais áreas durante o processo de reconhecimento. Nesse processo, a relação interna das diferentes regiões guia o movimento dos olhos para encontrar a próxima área. Ignorar as partes irrelevantes torna mais fácil aprender na presença de desordem. Por isso, a visão humana possui um desempenho incomparável no reconhecimento de objetos.

%In DCN Attention Input, the attentional modules are filter masks for the input data. This mask assigns low weights to regions irrelevant to neural network processing and high weights to relevant areas. This structure is similar to the multiglimpse visual mechanism and visual attention of human beings. The human visual attention mechanism is capable of exploring local differences in an image and highlighting the main parts. This means that one person focuses attention on one part of the image at a time. The multiglimpse refers to the ability to quickly scan the entire image and find the main areas during the recognition process. In this process, the internal relationship of the different regions guides the movement of the eyes to find the next area. Ignoring the irrelevant parts makes it easier to learn in the presence of disorder. For this reason, human vision has an incomparable performance in object recognition.

%Outra vantagem do glimpse e da atenção visual é a robustez. Se os nossos olhos visualizam um objeto em uma cena do mundo real, as partes que estão longe do objeto são ignoradas. Portanto, o fundo distante do objeto fixo não interfere no reconhecimento. No entanto, os métodos de classificação tradicionais usando CNN tratam igualmente todas as partes da imagem. As partes redudantes e irrelevantes contribuem para confundir a classificação e torná-la sensível aos ambientes visuais, incluindo fundo, ponto de vista da câmera e condições de iluminação. Então, as principais contribuições e motivações para introduzir mecanismos de atenção visual e multiglimpse diretamente sobre os dados de entrada da rede neural são:

%Another advantage of glimpse and visual attention is its robustness. If our eyes see an object in a real-world scene, parts that are far from the object are ignored. Therefore, the distant background of the fixed object does not interfere with recognition. However, traditional classification methods using CNN treat all parts of the image equally. Reductive and irrelevant parts contribute to confuse the classification and make it sensitive to visual environments, including background, camera point of view, and lighting conditions. So, the main contributions and motivations for introducing visual and multiglimpse mechanisms directly on the input data of the neural network are:

%\begin{itemize}
    %\item Gerar uma arquitetura de CNN mais escalável, em que a quantidade de parâmetros não varie linearmente de acordo com o tamanho da imagem de entrada.
    %\item Generate a more scalable CNN architecture, in which the number of parameters does not vary linearly according to the size of the input image.
    %\item Gerar resultados de classificação mais robustos, pois a rede seleciona apenas as partes mais relevantes da entrada e elimina distratores, minimiza o efeito de mudança de iluminação e escala, assim como reduz o efeito das mudanças de ponto de vista da câmera.
    %\item Generate more robust classification results. The network selects only the most relevant parts of the entrance and eliminates distractors, minimizes the effect of changing lighting and scale, and reduces the impact of changes in the camera's point of view.
    %\item Permite resultados mais robustos de fine-grained classification.
    %\item It generates more robust fine-grained classification results.
%\end{itemize}

%There are few approaches in the literature exploring the use of attentive masks directly over the input image. The few existing strategies make use of reinforcement learning. \cite{zhao_deep_2017} proposes an approach that fits this architecture. A more detailed view of the architecture and attentional module is illustrated in Figure \ref{fig:dcn_attention_input}.

%No DCN Attention Layer XXXXX


%\subsubsubsection*{\textbf{DCN Attention Layer}}

%A categoria de DCN Attention Recurrent Input representa a categoria de processos recorrentes de atenção. O mecanismo gera a máscara atencional utilizando os features maps de alguma camada da rede convolucional e posteriormente aplica essa máscara a entrada selecionando uma área de interesse. Essa região de interesse é entrada para um novo classificador. Ao final do processo, existem \textit{n} resultados de classificação provenientes de \textit{n} classificadores. A ponderação desses resultados define a classe dos elementos. Os mecanismos dessa categoria surgiram pelas deficiências e problemas de aplicar a atenção diretamente sobre os dados de entrada. A principal vantagem dessa abordagem é a simplicidade e o fato dos mecanismos serem diferenciáveis. No entanto, essa estrutura é computacionalmente cara, pois é necessário executar vários classificadores \textit{n} vezes.

%The DCN Attention Recurrent Input category represents the category of recurrent attention processes. The mechanism generates the attentional mask using the features maps from some layers of the convolutional network. It later applies this mask to the input by selecting an area of interest. This region of interest is an entry for a new classifier. At the end of the process, there are \textit{n} classification results from \textit{n} classifiers. The weighting of these results defines the class of elements. This category's mechanisms arose from the deficiencies and problems of applying attention directly to the input data. The main advantage of this approach is simplicity and the fact that the mechanisms are differentiable. However, this structure is computationally expensive, as it is necessary to run several classifiers \textit{n} times.

%One of the main goals of DCN Attention Input architectures is to perform the fine-grained classification robustly. Despite the good results, these methods are more computationally costly, with a longer inference time than desired. In an attempt to achieve good results, DCN Attention Prediction mechanisms extract features maps at different levels to generate spatial attention masks and use them to generate a class hypothesis based on local information and a confidence index (C). The final forecast consists of the average of all the hypotheses weighted by the normalized confidence scores. The main advantages of this approach are:

%\begin{itemize}
%    \item The attention mechanisms in this category can be %replicated at each layer in any convolutional network, and it %is easy to adapt the module to the task in question.
%    \item The core mechanisms in this category easily accept %pre-trained architectures.
%    \item The mechanisms are simple, have low computational %cost, and are differentiable.
%    \item Simple way to build an ensemble structure.
%\end{itemize}

%\subsubsection*{\textbf{DCN Attention Out}}
%\label{sub:dcn_att_out} O mecanismo de atenção extrai informações do feature maps da CNN em %todos os níveis ou em pelo menos um nível, e a saída 

%Por outro lado, no DCN Residual Attention extracts information from the feature maps and presents a residual input connection to the next layer. This information is used to construct an attentional mask that is applied to the incoming neural network data, the filtered data is used to feed a new convolutional network. The motivation for this architecture is also due to CNNs' inability to handle fine-grained sorting tasks. Because applying masking directly to input data typically uses reinforcement learning approaches, another way in the literature to apply masking over data without using reinforcement learning is to use the DCN Top Down architecture model. Input The main advantage of this type of architecture over DCN Attention Input is that the architecture is end-to-end trainable and attention calculation is not computationally costly. However, several convolutional neural networks end up being trained in the recurrence process, instead of just one, this can be quite laborious and computationally costly. Também não há muitas abordagens utilizando essa abordagem de gerar várias redes neurais convolucionais recorrentes utilizando como entrada a máscara atencional da rede anterior. A principal arquitetura na literatura que utiliza essa abordagem é a RA-CNN \cite{fu_look_2017}. 
%Como ilustrado na Figura X, além do pipeline da rede convolucional padrão a arquitetura possui uma segunda tarefa que é prever um conjunto de coordenadas para deliminar a região a ser utilizada como imagem de entrada na próxima rede convolucional. Essa função é dada pelo módulo de atenção e ela aproxima 3 parâmetros:

%On the other hand, DCN Residual Attention extracts information from the feature maps and presents a residual input connection to the next layer. This information is used to construct an attentional mask applied to the incoming neural network data. The filtered data feed a new convolutional network. The motivation for this architecture is also due to CNNs' inability to handle fine-grained sorting tasks. Because applying masking directly to input data typically uses reinforcement learning approaches, another way in the literature to apply masking over data without using reinforcement learning is to use the DCN Top-Down architecture model. Input The main advantage of this type of architecture over DCN Attention Input is that the architecture is end-to-end trainable, and attention calculation is not computationally costly. However, several convolutional neural networks end up being trained in the recurrence process, instead of just one. This can be quite laborious and computationally costly and not many approaches generate multiple recurrent convolutional neural networks using the attentional mask from the previous network as an input. The main architecture in the literature that follows this approach is RA-CNN \cite{fu_look_2017}.


%Por fim, no \textbf{DCN Attention Out} Um módulo atencional substitui as camadas de pooling tradicionais existentes nas redes convolucionais. A camada de pooling nas CNNs clássicas tem como objetivo reduzir a dimensão da imagem para capturar relações espaciais mais distantes entre os dados nas camadas convolucionais mais profundas. Além disso, os métodos de pooling padrão selecionam as informações de alto gradiente do mapa de características, por elas serem mais significativas na etapa de extração de características, ajudando a reduzir também a quantidade de parâmetros nas camadas posteriores. No entanto, a seleção das informações de alto gradiente não leva em consideração a importância dos dados e de certas regiões do mapa de características dada a tarefa atribuída a rede neural. As camadas de pooling tradicionais não consideram a importância dos dados dado um determinado contexto de tarefa. Se a seleção das informações de cada camada for direcionada a regiões fundamentais da imagem o modelo pode atingir resultados mais promissores. Essa é a motivação da criação da camada de pooling atencional. Ela funciona como uma extensão do average pool, mas utilizando ponderações com pesos específicos dado pelo sistema atencional.

%Finally, in \textbf{DCN Attention Out}, an attentional module replaces the traditional pooling layers existing in convolutional networks. The pooling layer on classic CNNs aims to reduce the size of the image to capture more distant spatial relationships between data in the deeper convolutional layers. Also, standard pooling methods select high gradient information from the feature map, as they are more significant in the feature extraction stage, helping reduce the number of parameters in the later layers. However, the selection of high gradient information does not consider the importance of the data and some areas of the characteristic map given the task assigned to the neural network. Traditional pooling layers do not consider the importance of data given a given task context. If the selection of information for each layer is driven to the image's key regions, the model can achieve more promising results. This is the motivation for creating the attentional pooling layer. It works as an extension of the average pool but using weightings with specific weights given by the attentional system.

==> PART_I_subs/attention_based_generative.tex <==
%esther: check 1

\subsection{Attention-based Generative Models}
\label{subsec:attention_generative_models}

Attention emerges in generative models essentially to augmented memory. Currently, there are not many ways to use attention on generative models. Since GANs are not a neural network architecture but a framework, we do not discuss the use of attention in GANs but autoencoders. We divided the uses of attention into three distinct groups (Figure \ref{fig:generative_models}): 1) Autoencoder input attention -- attention provides spatial masks corresponding to all the parts for a given input, while a component autoencoder (e.g., AE, VAE, SAE) independently models each of the parts indicated by the masks. 2) Autoencoder memory attention -- attention module acts as a layer between the encoder-decoder to augmented memory., 3) Autoencoder attention encoder-decoder -- a fully attentive architecture acts on the encoder, decoder, or both.
 

%figuras das arquiteturas
\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.90\linewidth]{img/autoencoder_types.pdf}
\caption{Attention-based generative models. The Autoencoder input attention group uses attention to facilitate the decomposition of scenes in abstract building blocks. The input components extracted by the masks share significant properties and help to imagine new scenarios. This approach is very efficient for the network to learn to decompose challenging scenarios between semantically significant components. Autoencoder memory attention group handles a memory buffer that allows read/writes operations and is persistent over time. Such models generally handle input and output to the memory buffer using write/read operations guided by the attention system. The use of attention and memory history in autoencoders helps to increase the generalizability of architecture. Autoencoder attention encoder-decoder using a model (usually self-attentive model) to increase the ability to generalize.}
\label{fig:generative_models}
\end{center}
\end{figure}


%explica as categorias, explica os ganhos, explica um pouquinho das arquiteturas

%categoria 1
%falo o que é, fala rapidamente os ganhos de colocar a atenção nesse ponto da rede e link com os trabalhos e faz referências


MONet \cite{burgess2019monet} is one of the few architectures to implement attention at the VAE input. A VAE is a neural network with an encoder parameterized by $\phi $ and a decoder parameterized by $\theta$. The encoder parameterizes a distribution over the component latent $z_{k}$, conditioned on both the input data \textit{x} and an attention mask $m_{k}$. The mask indicates which regions of the input the VAE should focus on representing via its latent posterior distribution, $q\phi(z_{k}|x, m_{k})$. During training, the VAE's
decoder likelihood term in the loss $p_{\theta}(x|z_{k})$ is weighted according to the mask, such that it is
unconstrained outside of the masked regions. In \cite{li2016learning}, the authors use soft attention with learned memory contents to augment models to have more parameters in the autoencoder. In \cite{bartunov2016fast}, Generative Matching Networks use attention to access the exemplar memory, with the address weights computed based on a learned similarity function between an observation at the address and a function of the latent state of the generative model. In \cite{rezende2016one}, external memory and attention work as a way of implementing one-shot generalization by treating the exemplars conditioned on as memory entries accessed through a soft attention mechanism at each step of the incremental generative process similar to DRAW \cite{draw}. Although most approaches use soft attention to address the memory, in \cite{bornschein2017variational} the authors use a stochastic, hard attention approach, which allows using variational inference about it in a context of few-shot learning. 

In \cite{escolano2018self}, self-attentive networks increase the autoencoder ability to generalize. The advantage of using this model instead of other alternatives, such as recurrent or convolutional encoders, is that this model is based only on self-attention and traditional attention over the whole representation created by the encoder. This approach allows us to easily employ the different components of the networks (encoder and decoder) as modules that, during inference, can be used with other parts of the network without the need for previous step information.

==> PART_I_subs/attention_based_rnns.tex <==
%esther: check 1

\subsection{Attention-based Recurrent Neural Networks (RNNs)}
\label{subsec:attention_rnn}

Attention in RNNs is mainly responsible for capturing long-distance dependencies. Currently, there are not many ways to use attention on RNNs. RNNSearch's mechanism for encoder-decoder frameworks inspires most approaches \cite{bahdanau_neural_2014}. We divided the uses of attention into three distinct groups (Figure \ref{fig:rnn_attention}): 1) Recurrent attention input -- the first stage of attention to select elementary input stimulus, i.e., elementary features, 2) Recurrent memory attention -- the first stage of attention to historical weight components, 3) Recurrent hidden attention -- the second stage of attention to select categorical information to the decode stage.

\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.95\linewidth]{img/rnn_family.pdf}
\caption{Attention-based recurrent neural networks. The architecture is a classic recurrent network or a Bi-RNN when hidden layers are recurrent cells. When the hidden layer is a recurrent memory, the architecture is an LSTM or Bi-LSTM. Finally, the architecture is a GRU when the hidden layer is a gated memory cell. The recurrent attention input group uses attention to filter input data. Recurrent hidden attention groups automatically select relevant encoder hidden states across all time steps. Usually, this group implements attention in encoder-decoder frameworks. The recurrent memory attention group implements attention within the memory cell. There are not many architectures in this category as far as we know, but the main uses are related to filtering the input data and the weighting of different historical components for predicting the current time step.}
\label{fig:rnn_attention}
\end{center}
\end{figure}


%falar dos trabalhos de atencao de Recurrent attention input
The \textbf{recurrent attention input} group main uses are item-wise hard, local-wise hard, item-wise soft, and local-wise soft selection. In table \ref{tab:recurrent_att_input}, we classify some representative work according to their attention input group operation. \textbf{Item-wise hard} selects discretely relevant input data for further processing, whereas \textbf{location-wise hard} discretely focuses only on the most relevant features for the task. \textbf{Item-wise soft} assigns a continuous weight to each input data given a sequence of items as input,  and  \textbf{location-wise soft} assigns a continuous weight between input features. Location-wise soft estimates high weights for features more correlated with the global context of the task. Hard selection for input elements are applied more frequently in computer vision approaches \cite{mnih_recurrent_2014} \cite{marcus_edel;joscha_lausch_capacity_2016}. On the other hand, soft mechanisms are often applied in other fields, mainly in Natural Language Processing. The soft selection normally weighs relevant parts of the series or input features, and the attention layer is a feed-forward network differentiable and with a low computational cost. Soft approaches are interesting to filter noise from time series and to dynamically learn the correlation between input features and output \cite{qin2017dual}\cite{geoman_2018}\cite{du2017rpan}. Besides, this approach is useful for addressing graph-to-sequence learning problems that learn a mapping between graph-structured inputs to sequence outputs, which current Seq2Seq and Tree2Seq may be inadequate to handle \cite{xu2018graph2seq}.    

\begin{table}[htb]
\begin{threeparttable}
\tiny
\fontfamily{pcr}\selectfont
\begin{tabular*}{0.48\textwidth}{llllllllll}
\hline
\small

\tiny \textbf{Architecture} & \textbf{Task}                                                                       & \multicolumn{3}{c}{
\textbf{Mechanism}}                                                       & \multicolumn{4}{c}{\textbf{Use of Attention}}                                                                                                  &   \\ \hline
\multicolumn{1}{l}{}  & \multicolumn{1}{l}{}                                                                 & \textbf{soft}        & \multicolumn{1}{c}{\textbf{hard}} & \multicolumn{1}{c}{\textbf{self}} & \multicolumn{1}{c}{\textbf{I}} & \multicolumn{1}{c}{\textbf{II}} & \multicolumn{1}{c}{\textbf{III}} & \multicolumn{1}{c}{\textbf{IV}} \\ \hline
DA-RNN\cite{qin2017dual}         &  \begin{tabular}[c]{@{}c@{}}Forecasting \\ time series\end{tabular}                                                                             &    \multicolumn{1}{c}{\checkmark}                  &                                   &                                   &                                &                                 &            \multicolumn{1}{c}{\checkmark}                      &                      \\ \hline
GeoMAN\cite{geoman_2018}               & \begin{tabular}[c]{@{}c@{}}Forecasting \\ time series\end{tabular}                                                                               &     \checkmark                 &                                   &                                   &                                &                                 &                                  &      \multicolumn{1}{c}{\checkmark}                    \\ \hline
Policy\cite{baker2019emergent}              & Others                                                                               &                      &                                   &               \multicolumn{1}{c}{\checkmark}                     &                                &                                 &       \multicolumn{1}{c}{\checkmark}                            &         \\ \hline
RPAN\cite{du2017rpan}      &      \begin{tabular}[l]{@{}l@{}}Action \\ Recognition\end{tabular}                                         &          \multicolumn{1}{c}{\checkmark}            &                                   &                                   &                                &                                 &          \multicolumn{1}{c}{\checkmark}                        &                               \\ \hline
RAM\cite{mnih_recurrent_2014}                 &   \begin{tabular}[l]{@{}l@{}}Image \\ Classification\end{tabular}                                                                     & \multicolumn{1}{l}{}  &           \multicolumn{1}{c}{\checkmark}                       &                                   &   \multicolumn{1}{c}{\checkmark}                             &                                 &                                  &                  \\ \hline
CRAM\cite{marcus_edel;joscha_lausch_capacity_2016}              & 
\begin{tabular}[l]{@{}l@{}}Image \\ Classification\end{tabular}  &                      &              \multicolumn{1}{c}{\checkmark}                     &                                   &   \multicolumn{1}{c}{\checkmark}                              &                                &                                  &                  \\ \hline
Cheng\cite{cheng2016long}               & \begin{tabular}[l]{@{}l@{}}Natural \\ Language \\Inference\end{tabular}                                                           &      \multicolumn{1}{c}{\checkmark}                &                                   &                                   &                                &                                 &                 \multicolumn{1}{c}{\checkmark}                 &                                 \\ \hline
Graph2Seq\cite{xu2018graph2seq}          & \begin{tabular}[l]{@{}l@{}}Natural \\ Language\\ Generation\end{tabular}                                     & \multicolumn{1}{l}{\checkmark} &                                   &                                   &                                &                                 &              \multicolumn{1}{l}{\checkmark}                    &                   \\ \hline
Ba Jimmy\cite{ba_multiple_2014}         & \begin{tabular}[l]{@{}l@{}}Object \\ Recognition\end{tabular}                                     & \multicolumn{1}{l}{} &     \checkmark                              &                                   &                          \checkmark      &                                 &              \multicolumn{1}{l}{}                    &                   \\ \hline
\end{tabular*}
\begin{tablenotes}
        \item[I] Item-wise hard. 
        \item[II] Local-wise hard. 
        \item[III] Item-wise soft. 
        \item[IV] Local-wise soft.
    \end{tablenotes}
\end{threeparttable}
\caption{The shortlist of works representative of attention uses for recurrent input attention group. Item-wise hard and local-wise-hard are discrete selections. Item-wise soft and local-wise soft are continuous selections.}
\label{tab:recurrent_att_input}
\end{table}







Hard mechanisms take inspiration from how humans perform visual sequence recognition tasks, such as reading by continually moving the fovea to the next relevant object or character, recognizing the individual entity, and adding the knowledge to our internal representation. A deep recurrent neural network, at each step, processes a multi-resolution crop of the input image, called a glimpse. The network uses information from the glimpse to update its internal representation and outputs the next glimpse location. The Glimpse network captures salient information about the input image at a specific position and region size. The internal state is formed by the hidden units $h_{t}$ of the recurrent neural network, which is updated over time by the core network. At each step, the location network estimates the next focus localization, and action networks depend on the task (e.g., for the classification task, the action network's outputs are a prediction for the class label.). Hard attention is not entirely differentiable and therefore uses reinforcement learning.

RAM \cite{mnih_recurrent_2014} was the first architecture to use a recurrent network implementing hard selection for image classification tasks. While this model has learned successful strategies in various image data sets, it only uses several static glimpse sizes. CRAM \cite{marcus_edel;joscha_lausch_capacity_2016} uses an additional sub-network to dynamically change the glimpse size, with the assumption to increase the performance, and in Jimmy et al. \cite{ba_multiple_2014} explore modifications in RAM for real-world image tasks and multiple objects classification. CRAM is a similar RAM model except for two key differences: Firstly, a dynamically updated attention mechanism restrains the input region observed by the glimpse network and the next output region prediction from the emission network -- a network that incorporates the location and capacity information as well as past information.  In simple terms, the sub-network decides at each time-step what the focus region's capacity should be. Secondly, the capacity sub-network outputs are successively added to the emission network's input that will ultimately generate the information for the next focus region—allowing the emission network to combine the information from the location and the capacity networks.

%falar dos trabalhos de atencao da Recurrent Hidden Attention
%%% esther aqui
Nearly all important works in the field belong to the \textbf{recurrent hidden attention} group, as shown in Figure \ref{fig:recurrent_attention_table}. In this category, the attention mechanism selects elements that are in the RNN's hidden layers for inter-alignment, contextual embedding, multiple-input processing, memory management, and capturing long-term dependencies, a typical problem with recurrent neural networks. Table \ref{tab:recurrent_hidden_attention_table} presents a list of the main works that explore such uses. Inter-alignment involves the encoder-decoder framework, and the attention module between these two networks is the most common approach. This mechanism builds a context vector dynamically from all previous decoder hidden states and the current encoder hidden state. Attention in inter-alignment helps minimize the bottleneck problem, with RNNSearch \cite{bahdanau_neural_2014} for machine translation tasks as its first representative. Further, several other architectures implemented the same approach in other tasks \cite{cheng2016long}\cite{yang2016hierarchical}\cite{seo_bidirectional_2016}. For example, Zichao Yang et al. \cite{yang2016hierarchical} extended the soft selection to the hierarchical attention structure, which allows the calculation of soft attention at the word level and the sentence level in the GRU networks encoder for document classification.

\begin{figure}[htb]
\begin{center}
    \includegraphics[width=1\linewidth]{img/redes_recorrentes_correta.pdf}
\caption{Attention-based recurrent neural networks main architectures by task and attention use.}
\label{fig:recurrent_attention_table}
\end{center}
\end{figure}


To create contextual embeddings and to manipulate multimodal inputs, co-attention is highly effective for text matching applications. Co-attention enables the learning of pairwise attention, i.e., learning to attend based on computing word-level affinity scores between two documents. Such a mechanism is designed for architectures comprised of queries and context, such as questions and answers and emotions analysis. Co-attention models can be fine-grained or coarse-grained. Fine-grained models consider each element of input concerning each element of the other input. Coarse-grained models calculate attention for each input, using an embedding of the other input as a query. Although efficient, co-attention suffers from information loss from the target and the context due to the anticipated summary. Attention flow emerges as an alternative to summary problems. Unlike co-attention, attention flow links and merges context and query information at each stage of time, allowing embeddings from previous layers to flow to subsequent modeling layers. The attention flow layer is not used to summarize the query and the context in vectors of unique features, reducing information loss. Attention is calculated in two directions, from the context to the query and from the query to the context. The output is the query-aware representations of context words. Attention flow allows a hierarchical process of multiple stages to represent the context at different granularity levels without an anticipated summary.

\begin{table}[htb]
\begin{threeparttable}
\tiny
\fontfamily{pcr}\selectfont
\begin{tabular*}{0.48\textwidth}{llllllllll}
\hline
\textbf{Architecture} & \textbf{Field}                                                                                       & \multicolumn{3}{c}{\textbf{Mechanism}}                                                       & \multicolumn{5}{c}{\textbf{Use of Attention}}                                                                                                      \\ \hline
\multicolumn{1}{l}{}  & \multicolumn{1}{l}{}                                                                                 & \textbf{soft}        & \multicolumn{1}{c}{\textbf{hard}} & \multicolumn{1}{c}{\textbf{self}} & \multicolumn{1}{c}{\textbf{I}} & \multicolumn{1}{c}{\textbf{II}} & \multicolumn{1}{c}{\textbf{III}} & \multicolumn{1}{c}{\textbf{IV}} & \multicolumn{1}{c}{\textbf{V}} \\ \hline
 Chen\cite{huimin_chen;maosong_sun;cunchao_tu;yankai_lin;zhiyuan_liu_neural_2016}          & \begin{tabular}[l]{@{}l@{}}Sentiment\\ classification \end{tabular}                                                                               &     \multicolumn{1}{l}{\checkmark}                 &                                   &                                   &                                &       \multicolumn{1}{l}{\checkmark}                          &         \multicolumn{1}{l}{\checkmark}                         &                                 &   \\ \hline
RNNSearch\cite{bahdanau_neural_2014}    & \begin{tabular}[l]{@{}l@{}}Machine\\ translation \end{tabular}                                                     &      \multicolumn{1}{l}{\checkmark}                & \multicolumn{1}{c}{}              &                                   &           \multicolumn{1}{l}{\checkmark}                     &                                 &                                  &                                 &  \multicolumn{1}{l}{\checkmark} \\ \hline
Cheng\cite{cheng2016long}      & \begin{tabular}[l]{@{}l@{}}Natural language\\ inference \end{tabular}                                                                              &       \multicolumn{1}{l}{\checkmark}               &                                   &                                   &          \multicolumn{1}{l}{\checkmark}                      &                                 &                                  &                                 & \multicolumn{1}{l}{\checkmark}  \\ \hline
Sdnet\cite{chenguang_zhu;michael_zeng;xuedong_huang_sdnet:_2019}                & Question-answering                                                                                   &     \multicolumn{1}{l}{\checkmark}                 &                                   &                                   &                                &           \multicolumn{1}{l}{\checkmark}                      &           \multicolumn{1}{l}{\checkmark}                       &                                 &   \\ \hline
SAB\cite{ke_sparse_2018}   & \begin{tabular}[l]{@{}l@{}}Image classification\\ Transfer learning\\ Algorithmic tasks\end{tabular} & \multicolumn{1}{l}{} &        \multicolumn{1}{l}{\checkmark}                           &                                   &                                &                                 &                                  &             \multicolumn{1}{l}{\checkmark}                    &  \multicolumn{1}{l}{\checkmark} \\ \hline
TCAN\cite{li2019topical}           & Recommender systems                                                                                  &    \multicolumn{1}{l}{\checkmark}                  &                                   &                                   &                                &          \multicolumn{1}{l}{\checkmark}                       &       \multicolumn{1}{l}{\checkmark}                           &                                 &   \\ \hline
AVS\cite{ji2019video}          & Video Summarization                                                                                  &     \multicolumn{1}{l}{\checkmark}                 &                                   &                                   &              \multicolumn{1}{l}{\checkmark}                  &                                 &            \multicolumn{1}{l}{\checkmark}                      &                                 &   \\ \hline
HAN\cite{yang2016hierarchical}            & \begin{tabular}[l]{@{}l@{}}Document\\ Classification \end{tabular}             &     \multicolumn{1}{l}{\checkmark}                 &                                   &                                   &                               &                                 &            \multicolumn{1}{l}{\checkmark}                      &                                 &   \\ \hline
BiDAF\cite{seo_bidirectional_2016}                  & Question-answering           &     \multicolumn{1}{l}{\checkmark}                 &                                   &                                   &                               &   \multicolumn{1}{l}{\checkmark}                               &            \multicolumn{1}{l}{\checkmark}                      &                                 &   \\ \hline

\end{tabular}
\begin{tablenotes}
        \item[I] Inter-alignment. 
        \item[II] Contextual Embedding Creation. 
        \item[III] Multiple input processing. 
        \item[IV] Manage internal memory.
        \item[V] Capture long-term dependencies.
    \end{tablenotes}
\end{threeparttable}
\caption{The shortlist of works representative of attention uses for recurrent hidden attention group.}
\label{tab:recurrent_hidden_attention_table}
\end{table}


Hard attention mechanisms do not often occur on recurrent hidden attention networks. However, Nan Rosemary et al. \cite{ke_sparse_2018} demonstrate that hard selection to retrieve past hidden states based on the current state mimics an effect similar to the brain's ability. Humans use a very sparse subset of past experiences and can access them directly and establish relevance with the present, unlike classic RNNs and self-attentive networks. Hard attention is an efficient mechanism for RNNs to recover sparse memories. It determines which memories will be selected on the forward pass, and therefore which memories will receive gradient on the backward pass during training. At time $t$, RNN receives a vector of hidden states $h^{t-1}$, a vector of cell states $c^{t-1}$, and an input $x^{t}$, and computes new cell states $c^{t}$ and a provisional hidden state vector $\widetilde{h}^{t}$ that also serves as a provisional output. First, the provisional hidden state vector $\widetilde{h}^{t}$ is concatenated to each memory vector $m_{i}$ in the memory $M$. MLP maps each vector to an attention weight $ a^{t}_{i}$, representing memory relevance $i$ in current moment $t$. With attention weights $ a^{t}_{i}$ sparse attention computes a hard decision. The attention mechanism is differentiable but implements a hard selection to forget memories with no prominence over others. This is quite different from typical approaches as the mechanism does not allow the gradient to flow directly to a previous step in the training process. Instead, it propagates to some local timesteps as a type of local credit given to a memory.


%falar dos trabalhos de atencao da Recurrent Memory Attention

Finally, \textbf{recurrent memory attention} groups implement attention within the memory cell. As far as our research goes, there are not many architectures in this category. Pengfei et al. \cite{zhang2018adding} proposed an approach that modulates the input adaptively within the memory cell by assigning different levels of importance to each element/dimension of the input shown in Figure \ref{fig:recurrent_memory_attention}a. Dilruk et al. \cite{perera2020lstm} proposed mechanisms of attention within memory cell to improve the past encoding history in the cell's state vector since all parts of the data history are not equally relevant to the current prediction. As shown in Figure \ref{fig:recurrent_memory_attention}b, the mechanism uses additional gates to update LSTM's current cell.  


\begin{figure}[h]
\begin{center}
    \includegraphics[width=0.95\linewidth]{img/recurrent_memory_attention.pdf}
\caption{Recurrent memory attention approaches. a) Illustration of Element-wise-Attention Gate in GRU. Specifically, the input modulation is adaptable to the content and is performed in fine granularity, element-wise rather than input-wise. b) Gate attention in LSTM. The model calculates attention scores to weigh the relevance of different parts of history. There are two additional gates for updating the current cell using the previous state $h_{A}^{t-1}$. The first, input attention gate layer, analyzes the current input $i^{\triangle t}$ and $h_{A}^{t-1}$ to determine which values to be updated in current cell $C^{t}$. The second, the modulation attention gate, analyzes the current input $i^{\triangle t}$ and $h_{A}^{t-1}$. Then computes the set of candidate values that must be added when updating the current cell state $C^{t}$. The attention mechanisms in the memory cell help to more easily capture long-term dependencies and the problem of data scarcity.}
\label{fig:recurrent_memory_attention}
\end{center}
\end{figure}


%Nós selecionamos um conjunto de arquiteturas impactantes da área que implementam a atenção nas RNNs (Figure \ref{fig:recurrent_attention_table}). Dividimos essas arquiteturas em três categorias: Recurrent Attention Input, Recurrent Hidden %Attention, and Recurrent Memory Attention (Figure \ref{fig:recurrent_attention_architecture}). 


%We selected a set of impactful architectures in the area that implement attention in the RNNs (Figure \ref{fig:recurrent_attention_table}). We divided these architectures into three categories: \textbf{Recurrent Attention Input, Recurrent Hidden Attention, and Recurrent Memory Attention (Figure \ref{fig:recurrent_attention_architecture})}. 

%apresentar a classificacao figuras






%explicar os usos da atenção nas rnns:
%apresentar a arquitetura
%apresentar como eu dividi os grupos - apresento os trabalhos e apresento as divisoes
%falar um pouquinho dos grupos 
%falar de cada grupo separadamente:
% fala de cada abordagem existente:
% - o que que a abordagem é
% - porque a abordagem está sendo usada (qual a problemática que a abordagem busca resolver), pegar trechos dos trabahos que apontam as melhorias
% - pode apontar tabelas, figuras, explicar algum tabalho


%apresentar cada categoria 
%falar um pouquinho dos usos da atencao em cada trabalho
%Algumas teorias da atenção humana argumentam que os resultados comportamentais são melhor modelados por dois estágios de mecanismos de atenção [X]: o primeiro estágio seleciona elementary stimulus, i.e., elementary features. Já o segundo estágio seleciona informações categóricas to decode stimulus. As redes do tipo Recurrent Attention Input e Recurrent Memory Attention implementam a atenção no primeiro estágio, selecionando as features mais relevantes da entrada da rede, enquanto que as redes Recurrent Hidden Attention automatically select relevant encoder hidden states across all time steps. Normalmente as redes Recurrent Hidden Attention implementam a atenção em frameworks do tipo encoder-decoder.




%vou falar especificamente de cada categoria e do nível de features que é extraído, apresentar uma tabela mostrando quais são as abordagens e as diferenças entre as abordagens %existentes, depois falar as vantagens e desvantagens dessa abordagem. Depois falar especificamente dos trabalhos. 
%Nas redes \textbf{Recurrent Attention Input (RAI)} o mecanismo de atenção está na entrada da rede neural. Os principais usos da atenção na entrada são input elements selection, features selection, input elements weight, local features weight, and global features weigth, como mostra a Tabela \ref{tab:recurrent_att_input}. No input elements selection o mecanismo atencional escolhe um conjunto de elementos da entrada relevantes para o processamento subsequente. No features selection o mecanismo seleciona o conjunto de features mais relevante para a tarefa e elimina as features desnecessárias. Input elements weight o mecanismo atribui um peso diferente a cada elemento da entrada, atribuindo pesos menores para os elementos irrelevantes para a tarefa. Em local features weigth o mecanismo atribui um peso diferente para cada feature de cada elemento da entrada. Por fim, no global features weigth o mecanismo calcula a correlação entre as features de entrada ou entre cada feature e a saída para ponderar as features mais relevantes no contexto global da tarefa. 







%Na literatura, os mecanismos hard para input elements selection são aplicados com maior frequência nas abordagens de visão computacional. Enquanto os mecanismos soft são frequentemente aplicados em outras áreas, principalmente em Natural Language Processing. A seleção soft (Figure \ref{fig:recurrent_attention_input_approaches} in a)) normalmente pondera partes relevantes da série ou features de entrada. A camada de atenção é uma rede ou um conjunto de redes do tipo feed-foward, o modelo é totalmente diferenciável e de baixo custo computacional. Essa abordagem se mostra intessante para filtrar ruído das séries temporais e para aprender dinamicamente a correlação entre as features de entrada e a saída [X][X]. Quando mais de uma modalidade sensorial é usada, o soft attention é útil para capturar correlações dinâmicas entre diferentes modalidades sensoriais e a saída [X]. Besides, this approach is useful to address graph-to-sequence learning problems that learns a mapping between graph-structured inputs to sequence outputs, which current Seq2Seq and Tree2Seq may be inadequate to handle [X].




%Na \textbf{Recurrent Hidden Attention (RHA)} estão a maioria das arquiteturas. Nessa categoria o mecanismo de atenção seleciona elementos que estão nas camadas ocultas da rede recorrente. Os principais usos da atenção nas redes RHA são o inter-alignment as way to help the target network review source information, o contextual embedding para criar representações contextuais envolvendo múltiplas entradas que muitas vezes possuem modalidades sensoriais diferentes, o multiple input processing para selecionar e relacionar corretamente features de diferentes fontes, o manage memory para utilizar a memória interna das redes recorrentes de uma forma biologicamente plausível. Por fim, para capturar dependências de longas distâncias entre longas sequências, um problema típico das redes neurais recorrentes. A tabela \ref{tab:recurrent_hidden_attention_table} apresenta uma lista não muito extensa dos principais trabalhos de atenção que exploram cada um dos principais usos descritos.



%A maior parte das abordagens nas redes do tipo RHA envolve aplicações com o framework encoder-decoder utilizando mecanismos soft ou self attention para inter-alignment. A abordagem mais comum é a do framework encoder-decoder em que o módulo de atenção está entre as duas redes (Figure \ref{fig:recurrent_hidden_attention_1}). A partir do estado oculto anterior do decoder e os estados ocultos do encoder o mecanismo pondera dinamicamente quais os estados ocultos mais relevantes para a predição da próxima palavra, construindo um vetor de contexto de tamanho fixo e dinâmico, em que os pesos dos estados ocultos se alteram a cada nova predição. O uso da atenção para inter-alignment ajuda a minimizar o problema do gargalo de informação dos frameworks encoder-decoder e permite o uso de sequências longas sem degradar o aprendizado. A primeira arquitetura a utilizar a atenção para inter-alignment foi a RNNSearch [X] em tarefas de tradução de máquina. Posteriormente, várias outras arquiteturas que implementaram a mesma abordagem em outras aplicações surgiram na literatura [X][X][X]. Por exemplo, Zichao Yang et. al. [X] estendeu a seleção soft do framework encoder-decoder para a estrutura hierarchical attention que permite o cáculo de atenção soft a nível de palavra e a nível de sentença no encoder de GRU networks para classificação de documentos.





%desenha
%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.55\linewidth]{img/recurrent_hidd%en_attention-1.jpg}
%\caption{Main Recurrent Hidden Attention approach. Soft %attention in traditional encoder-decoder framework.}
%\label{fig:recurrent_hidden_attention_1}
%\end{center}
%\end{figure}

%Há outras abordagens que exploram mecanismos soft attention mais complexos nas redes do tipo RHA. O foco dessas abordagens normalmente é criar embeddings contextuais e manipular múltiplas entradas ou entradas multimodais para alimentar níveis mais profundos da rede neural. O co-attention, por exemplo, é um mecanismo do tipo soft que é altamente eficaz para text matching applications. Co-attention enables the learning of pairwise attentions, i.e., learning to attend based on computing word-level affinity scores between two documents. Esse mecanismo é projetado para arquiteturas em que há uma query e um contexto, como perguntas e respostas e análise de sentimentos. Co-attention models can be fine-grained (Figure \ref{fig:recurrent_hidden_attention_2} em a)) or coarse-grained (Figure \ref{fig:recurrent_hidden_attention_2} em b)). Fine-grained models consideram cada elemento de uma entrada com respeito a cada elemento da outra entrada. Coarse-grained models calculam a atenção para cada entrada, usando um embedding da outra entrada como uma query. Apesar de eficiente, umas das desvantagens do co-attention é a perda de informações do target e do contexto por conta do resumo antecipado.



%colocar a figura com as abordagens e explicar como são as diferentes abordagens

%colocar a tabela com as abordagens 

%linkar um pouco com os tipos de aprendizado

%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.95\linewidth]{img/recurrent_hidd%en_attention_2.jpg}
%\caption{Recurrent Hidden Attention co-attention approaches. %a) Fine-grained co-attention.  b) Coarse-grained %co-attention.}
%\label{fig:recurrent_hidden_attention_2}
%\end{center}
%\end{figure}

%O attention flow, também um mecanismo de seleção soft, surge como uma abordagem para o problema do resumo antencipado nas arquiteturas que usam informações de contexto e consulta. Ao contrário do co-attention, o attention flow vincula e funde informações de contexto e consulta em cada etapa de tempo permitindo também que os embeddings das camadas anteriores fluam para camadas de modelagem subsequente, como mostra a Figura \ref{fig:recurrent_hidden_attention_2}. A camada de attention flow não é usada para resumir a consulta e o contexto em vetores de features únicos, isso reduz a perda de informações. A atenção é calculada em duas direções, do contexto para a query e da query para o contexto e a saída are the query-aware representations of context words. O attention flow permite um processo hieráquico de múltiplos estágios para representar o contexto em diferentes níveis de granularidade sem o recurso de resumo antecipado das informações.




%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.55\linewidth]{img/recurrent_hidd%en_attention-3.jpg}
%\caption{Recurrent Hidden Attention approaches. Attention %Flow.}
%\label{fig:recurrent_hidden_attention_2}
%\end{center}
%\end{figure}

%Os mecanismos hard attention não ocorrem com frequência nas redes Recurrent Hidden Attention. Nan Rosemary et. al. [X] demonstram que a seleção hard quando utilizada para recuperar estados ocultos do passado com base no estado atual da rede recorrente imita um efeito similar a capacidade do cérebro de recuperar reativamente memórias do passado com base no contexto atual. Humanos usam um subconjunto muito esparso de experiências passadas e são capazes de acessá-las diretamente e estabelecer relevância com o presente, diferentemente do que ocorre nas redes recorrentes clássicas e nas self-attentive networks (e.g., Transformer [X]). O hard attention é um mecanismo eficiente para as RNNs na recuperação de memórias esparsas. It determines which memories will be selected on the forward pass (Figure \ref{fig:recurrent_hidden_attention_3}), and therefore also which memories will receive gradient on the backward pass during training.




%At time $t$, RNN receives a vector of hidden states $h^{t-1}$, a vector of cell states $c^{t-1}$, and an input $x^{t}$, and computes new cell states $c^{t}$ and a provisional hidden state vector $\widetilde{h}^{t}$ that also serves as a provisional output. First, the provisional hidden state vector $\widetilde{h}^{t}$ is concatenated to each memory vector $m_{i}$ in the memory $M$. MLP maps each vector to an attention weight $ a^{t}_{i}$, representing memory relevance $i$ in current moment $t$. Com os pesos brutos de atenção $ a^{t}_{i}$ calcula-se a atenção esparsa passando o resultado através de uma função ReLU, normalizando os pesos para somar 1. Esse mecanismo é diferenciável mas implementa uma decisão hard para esquecer memórias que não tem proeminência sobre outras. Isso é bastante diferente dos mecanismos típicos de atenção que utilizam ponderações da função softmax. No processo de treino o mecanismo não permite que o gradiente flua diretamente para um passo passado, mas para alguns timesteps locais, como um tipo de crédito local dado à uma memória. 



%\begin{figure}[h]
%\begin{center}
%    \includegraphics[width=0.55\linewidth]{img/recurrent_hidd%en_attention-4.jpg}
%\caption{Recurrent Hidden Attention approach. Hard %Attention.}
%\label{fig:recurrent_hidden_attention_3}
%\end{center}
%\end{figure}


%Por fim, na categoria \textbf{Recurrent Memory Attention} estão as arquiteturas que implementam a atenção dentro da célula de memória da rede recorrente. Não existem muitas arquiteturas nessa categoria até o nosso conhecimento, mas os principais usos de atenção estão relacionados a filtragem dos dados de entrada e a ponderação de diferentes componentes históricos da rede para a predição na etapa de tempo atual. Pengfei et. al. [X] propôs uma abordagem que modula a entrada adaptativamente dentro da célula de memória atribuindo diferentes níveis de importância a cada elemento/dimensão da entrada. Como mostra a Figura \ref{fig:recurrent_memory_attention} em a), o módulo de atenção modula a entrada dentro de uma GRU. Especificamente, a modulação da entrada é adaptável ao conteúdo e é realizada em fine granularity, being element-wise rather than input-wise. 




%Dilruk et. al. [X] propôs mecanismos de atenção dentro de toda estrutura da célula de memória de uma LSTM para melhorar a codificação de todo o histórico no vetor de estado da célula, pois todas as partes do histórico dos dados não são igualmente relevantes para a predicão atual. Como mostra a Figura \ref{fig:recurrent_memory_attention} em b), o modelo calcula os scores de atenção para pesar a relevância de diferentes partes do histórico passado. Basicamente, existem dois gates adicionais para atualizar a célula atual usando o estado anterior $h_{A}^{t-1}$. O primeiro, oinput attention gate layer, analisa a entrada atual $i^{\triangle t}$ e $h_{A}^{t-1}$ para determinar quais valores serão atualizados no estado da célula atual $C^{t}$. O segundo, o modulation attention gate, analisa a entrada atual $i^{\triangle t}$ e $h_{A}^{t-1}$, e então computa o conjunto de valores candidatos que devem ser adicionados na atualização do estado da célula atual $C^{t}$. Os mecanismos atenção na célula de memória ajudam a capturar mais facilmente as dependências de longo prazo e o problema de escassez de dados. No entanto, essas alterações são mais complexas na estrutura da rede neural que as abordagens das categorias Recurrent Attention Input e Recurrent Hidden Attention.






==> PART_I_subs/attention_mechanisms.tex <==
%esther: check 1
\section{Attention Mechanisms}
\label{sub:attention_mechanisms}

Deep attention mechanisms can be categorized into soft attention (global attention), hard attention (local attention), and self-attention (intra-attention). 

\textbf{Soft Attention}. Soft attention assigns a weight of 0 to 1 for each input element. It decides how much attention should be focused on each element, considering the interdependence between the input of the deep neural network's mechanism and target. It uses softmax functions in the attention layers to calculate weights so that the entire attentional model is deterministic and differentiable. Soft attention can act in the spatial and temporal context. The spatial context operates mainly to extract the features or the weighting of the most relevant features. For the temporal context, it works by adjusting the weights of all samples in sliding time windows, as samples at different times have different contributions. Despite being deterministic and differentiable, soft mechanisms have a high computational cost for large inputs. Figure \ref{fig:soft_attention_example} shows an intuitive example of a soft attention mechanism.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{img/soft_attention_example.pdf}
  \caption{An intuitive example of Soft Attention. Visual QA architecture outputs an answer given an image and a textual question as input. It uses a soft attention mechanism that weighted visual features for the task for further processing. The premise is that the norm of the visual features correlates with their relevance. Besides, those feature vectors with high magnitudes correspond to image regions that contain relevant semantic content.}
  \label{fig:soft_attention_example}
\end{figure}


\textbf{Hard Attention}. Hard attention determines whether a part of the mechanism's input should be considered or not, reflecting the interdependence between the input of the mechanism and the target of the deep neural network. The weight assigned to an input part is either 0 or 1. Hence, as input elements are either seen, the objective is non-differentiable. The process involves making a sequence of selections on which part to attend. In the temporal context, for example, the model attends to a part of the input to obtain information and decide where to attend in the next step based on the known information. A neural network can make a selection based on this information. However, as there is no ground truth to indicate the correct selection policy, the hard-attention type mechanisms are represented by stochastic processes. As the model is not differentiable, reinforcement learning techniques are necessary to train models with hard attention. Inference time and  computational costs are reduced compared to soft mechanisms once the entire input is not being stored or processed. Figure \ref{fig:hard_attention_example} shows an intuitive example of a hard attention mechanism.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{img/hard_attention_example.pdf}
  \caption{An intuitive example of Hard Attention. Given an image and a textual question as input, the Visual QA architecture outputs an answer. It uses a hard attention mechanism that \textbf{selects only} the important visual features for the task for further processing. }
  \label{fig:hard_attention_example}
\end{figure}

\textbf{Self-Attention}. Self-attention quantifies the interdependence between the input elements of the mechanism. This mechanism allows the inputs to interact with each other "self" and determine what they should pay more attention to. The self-attention layer's main advantages compared to soft and hard mechanisms are parallel computing ability for a long input. This mechanism layer checks the attention with all the same input elements using simple and easily parallelizable matrix calculations. Figure \ref{fig:self_attention_example} shows an intuitive example of a self-attention mechanism.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{img/self_attention_example.pdf}
  \caption{Self-Attention examples. a) Self-attention in sentences
  b) Self-attention in images. The first image shows five representative query locations with color-coded dots with the corresponding color-coded arrows summarizing the most-attended regions.}
  \label{fig:self_attention_example}
\end{figure}

==> PART_I_subs/overview.tex <==
%esther: check 1
\section{Overview}
\label{sub:attention_overview}

%In this section, we present a brief overview of Attention in Deep Learning. 

Historically, research in computational attention systems has existed since the 1980s. Only in mid-2014, the Neural Attentional Networks (NANs) emerged in Natural Language Processing (NLP), where attention provided significant advances, bringing promising results through scalable and straightforward networks. Attention allowed us to move towards the complex tasks of conversational machine comprehension, sentiment analysis, machine translation, question-answering, and transfer learning, previously challenging. Subsequently, NANs appeared in other fields equally important for artificial intelligence, such as computer vision, reinforcement learning, and robotics. There are currently numerous attentional architectures, but few of them have a significantly higher impact, as shown in Figure \ref{fig:main_architectures_field}. In this image, we depict the most relevant group of works organized according to citation levels and innovations where RNNSearch \cite{bahdanau_neural_2014}, Transformer \cite{vaswani_attention_2017}, Memory Networks \cite{weston_2014_memory}, ``show, attend and tell'' \cite{xu_show_2015}, and RAM \cite{mnih_recurrent_2014} stand out as key developments.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{img/principais_arquiteturas_ok_2.pdf}
    \caption{Main Neural Attention Networks (NAN). Each circle corresponds to an architecture. The radius of the circles is defined based on the impact of the NAN on the field. The impact was defined by the citation number and the architecture innovation level. The greater the radius of the circle, the more significant the impact of architecture, and vice versa. Architectures labels are color-coded as follows: orange - natural language processing, red - computer vision, dark brown - computer vision and natural language processing, dark yellow - reinforcement learning and computer vision, light yellow - reinforcement learning and natural language processing, blue - imitation learning and robotics, and purple - others. }
    \label{fig:main_architectures_field}
\end{figure}


The \textit{bottleneck problem} in the classic encoder-decoder framework worked as the initial motivation for attention research in Deep Learning. In this framework, the encoder encodes a source sentence into a fixed-length vector from which a decoder generates the translation. The main issue is that a neural network needs to compress all the necessary information from a source sentence into a fixed-length vector. Cho et al.  \cite{cho2014properties} showed that the performance of the classic encoder-decoder deteriorates rapidly as the size of the input sentence increases. To minimize this bottleneck, Bahdanau et al. \cite{bahdanau_neural_2014} proposed \textbf{RNNSearch}, an extension to the encoder-decoder model that learns to align and translate together. RNNSearch generates a translated word at each time-step, looking for a set of positions in the source sentence with the most relevant words. The model predicts a target word based on the context vectors associated with those source positions and all previously generated target words. The main advantage is that RNNSearch does not encode an entire input sentence into a single fixed-length vector. Instead, it encodes the input sentence into a sequence of vectors, choosing a subset of these vectors adaptively while generating the translation. The attention mechanism allows extra information to be propagated through the network, eliminating the fixed-size context vector's information bottleneck. This approach demonstrated that the attentive model outperforms classic encoder-decoder frameworks for long sentences for the first time.

RNNSearch was instrumental in introducing the first attention mechanism, \textbf{soft attention} (Section \ref{sub:attention_mechanisms}). This mechanism has the main characteristic of smoothly selecting the network's most relevant elements. Based on RNNSearch, there have been numerous attempts to augment neural networks with new properties. Two research directions stand out as particularly interesting - \textbf{attentional interfaces} and \textbf{end-to-end attention}. Attentional interfaces treat attention as a module or set of elective modules, easily plugged into classic Deep Learning neural networks, just like RNNSearch. So far, this is the most explored research direction in the area, mainly for simplicity, general use, and the good results of generalization that the attentional interfaces bring. End-to-end attention is a younger research direction, where the attention block covers the entire neural network. High and low-level attentional layers act recursively or cascaded at all network abstraction levels to produce the desired output in these models. End-to-end attention models introduce a new class of neural networks in Deep Learning. End-to-end attention research makes sense since no isolated attention center exists in the human brain, and its mechanisms are used in different cognitive processes.

\subsection{Attentional interfaces}
\label{sub:attentional_interfaces}
%falar da atenção como interface apenas em RNNs
RNNSearch is the basis for research on attentional interfaces. The attentional module of this architecture is widely used in several other applications. In voice recognition \cite{chan2015listen}, allowing one RNN to process the audio while another examines it focusing on the relevant parts as it generates a description. In-text analysis \cite{vinyals2015grammar}, it allows a model to look at the words as it generates an analysis tree. In conversational modeling \cite{vinyals_neural_nodate}, it allows the model to focus on the last parts of the conversation as it generates its response. There are also important extensions to deal with other information bottlenecks in addition to the classic encoder-decoder problem. \textbf{BiDAF} \cite{seo_bidirectional_2016} proposes a multi-stage hierarchical process to question-answering. It uses the bidirectional attention flow to build a multi-stage hierarchical network with context paragraph representations at different granularity levels. The attention layer does not summarize the context paragraph in a fixed-length vector. Instead, attention is calculated for each step, and the vector assisted at each step, along with representations of previous layers, can flow to the subsequent modeling layer. This reduces the loss of information caused by the early summary. At each stage of time, attention is only a function of the query and the paragraph of the context in the current stage and does not depend directly on the previous stage's attention. The hypothesis is that this simplification leads to a work division between the attention layer and the modeling layer, forcing the attention layer to focus on learning attention between the query and the context.

% speak of HAN
Yang et al. \cite{yang2016hierarchical} proposed the \textbf{Hierarchical Attention Network (HAN)} to capture two essential insights about document structure. Documents have a hierarchical structure: words form sentences, sentences form a document. We, likewise, construct a document representation by first building representations of sentences and then aggregating them into a document representation. Different words and sentences in a document are differentially informative. Moreover, the importance of words and sentences is highly context-dependent, i.e., the same word or sentence may have different importance in different contexts. To include sensitivity to this fact, HAN consists of two levels of attention mechanisms - one at the word level and one at the sentence level - that let the model pay more or less attention to individual words and sentences when constructing the document's representation. Xiong et al. \cite{xiong2016dynamic} created a coattentive encoder that captures the interactions between the question and the document with a dynamic pointing decoder that alternates between estimating the start and end of the answer span. To learn approximate solutions to computationally intractable problems, \textbf{Ptr-Net} \cite{vinyals2015pointer} modifies the RNNSearch's attentional mechanism to represent variable-length dictionaries. It uses the attention mechanism as a pointer.

See et. al. \cite{see_get_2017} used a hybrid  between classic sequence-to-sequence attentional models and a Ptr-Net \cite{vinyals2015pointer} to abstractive text summarization. The hybrid pointer-generator \cite{see_get_2017} copies words from the source text via pointing, which aids accurate reproduction of information while retaining the ability to produce novel words through the generator. Finally, it uses a mechanism to keep track of what has been summarized, which discourages repetition. FusionNet \cite{huang_fusionnet:_2018} presents a novel concept of "history-of-word" to characterize attention information from the lowest word-embedding level up to the highest semantic-level representation. This concept considers that data input is gradually transformed into a more abstract representation, forming each word's history in human mental flow. FusionNet employs a fully-aware multi-level attention mechanism and an attention score-function that takes advantage of the history-of-word. Rocktäschel et al. \cite{rocktaschel_reasoning_2015} introduce two-away attention for  recognizing textual entailment (RTE). The idea is to allow the model to attend over past output vectors, solving the LSTM's cell state bottleneck. The LSTM with attention does not need to capture the premise's whole semantics in the LSTM cell state. Instead, attention generates output vectors while reading the premise and accumulating a representation in the cell state that informs the second LSTM which of the premises' output vectors to attend to determine the RTE class. Luong, et al. \cite{luong_effective_2015}, proposed global and local attention in machine translation. Global attention is similar to soft attention, while local is an improvement to make hard attention differentiable - the model first provides for a single position aligned to the current target word, and a window centered around the position is used to calculate a vector of context. %%%esther



% Attentional interfaces para visao
Attentional interfaces have also emerged in architectures for computer vision tasks. Initially, they are based on human saccadic movements and robustness to change. The human visual attention mechanism can explore local differences in an image while highlighting the relevant parts. One person focuses attention on parts of the image simultaneously, glimpsing to quickly scan the entire image to find the main areas during the recognition process. In this process, the different regions' internal relationship guides the eyes' movement to find the next area to focus. Ignoring the irrelevant parts makes it easier to learn in the presence of disorder. Another advantage of glimpse and visual attention is its robustness. Our eyes can see an object in a real-world scene but ignore irrelevant parts. Convolutional neural networks (CNNs) are extremely different. CNNs are rigid, and the number of parameters grows linearly with the size of the image. Also, for the network to capture long-distance dependencies between pixels, the architecture needs to have many layers, compromising the model's convergence. Besides, the network treats all pixels in the same way. This process does not resemble the human visual system that contains visual attention mechanisms and a glimpse structure that provides unmatched performance in object recognition.

RAM \cite{mnih_recurrent_2014} and STN are pioneering architectures with attentional interfaces based on human visual attention. \textbf{RAM} \cite{mnih_recurrent_2014} can extract information from an image or video by adaptively selecting a sequence of regions, glimpses, only processing the selected areas at high resolution. The model is a Recurrent Neural Network that processes different parts of the images (or video frames) at each instant of time \textit{t}, building a dynamic internal representation of the scene via Reinforcement Learning training. The main model advantages are the reduced number of parameters and the architecture's independence to the input image size, which does not occur in convolutional neural networks. This approach is generic. It can use static images, videos, or a perceptual module of an agent that interacts with the environment. \textbf{STN (Spatial Transformer Network)} \cite{jaderberg_spatial_2015} is a module robust to spatial transformation changes. In STN, if the input is transformed, the model must generate the correct classification label, even if it is distorted in unusual ways. STN works as an attentional module attachable -- with few modifications -- to any neural network to actively spatially transform feature maps. STN learns transformation during the training process. Unlike pooling layers, where receptive fields are fixed and local, a Spatial Transformer is a dynamic mechanism that can spatially transform an image, or feature map, producing the appropriate transformation for each input sample. The transformation is performed across the map and may include changes in scale, cut, rotations, and non-rigid body deformations. This approach allows the network to select the most relevant image regions (attention) and transform them into a desired canonical position by simplifying recognition in the following layers.

Following the RAM approach, the \textbf{Deep Recurrent Attentive Writer (DRAW)} \cite{draw} represents a change to a more natural way of constructing the image in which parts of a scene are created independently of the others. This process is how human beings draw a scene by recreating a visual scene sequentially, refining all parts of the drawing for several iterations, and reevaluating their work after each modification. Although natural to humans, most approaches to automatic image generation aim to generate complete scenes at once. This means that all pixels are conditioned in a single latent distribution, making it challenging to scale large image approaches. DRAW belongs to the family of variational autoencoders. It has an encoder that compresses the images presented during training and a decoder that reconstructs the images. Unlike other generative models, DRAW iteratively constructs the scenes by accumulating modifications emitted by the decoder, each observed by the encoder. DRAW uses RAM attention mechanisms to attend to parts of the scene while ignoring others selectively. This mechanism's main challenge is to learn where to look, which is usually addressed by reinforcement learning techniques. However, at DRAW, the attention mechanism is differentiable, making it possible to use backpropagation. 


\subsection{Multimodality}
\label{sub:multimodality}

%falo que essa é uma ferramenta poderosa para multimodalidade
The first attention interfaces' use in DL were limited to  NLP and computer vision domains to solve isolated tasks. Currently, attentional interfaces are studied in multimodal learning. Sensory multimodality in neural networks is a historical problem widely discussed by the scientific community \cite{ramachandram2017deep} \cite{gao2020survey}. Multimodal data improves the robustness of perception through complementarity and redundancy. The human brain continually deals with multimodal data and integrates it into a coherent representation of the world. However, employing different sensors present a series of challenges computationally, such as incomplete or spurious data, different properties (i.e. dimensionality or range of values), and the need for data alignment association. The integration of multiple sensors depends on a reasoning structure over the data to build a common representation, which does not exist in classical neural networks. Attentional interfaces adapted for multimodal perception are an efficient alternative for reasoning about misaligned data from different sensory sources.

%escrever um parágrafo das abordagens de aprendizado multimodal -> falar da abordagem clássica e aprensentar o grafico
The first widespread use of attention for multimodality occurs with the attentional interface between a convolutional neural network and an LSTM in image captioning \cite{xu_show_2015}. In this model, a CNN processes the image, extracting high-level features, whereas the LSTM consumes the features to produce descriptive words, one by one. The attention mechanism guides the LSTM to relevant image information for each word's generation, equivalent to the human visual attention mechanism. The visualization of attention weights in multimodal tasks improved the understanding of how architecture works. This approach derived from countless other works with attentional interfaces that deal with video-text data \cite{yao_describing_2015} \cite{wu_hierarchical_2018} \cite{fakoor2016memory}, image-text data \cite{tian2018diagnostic} \cite{pu_adaptive_2018}, monocular/RGB-D images \cite{liu2017global} \cite{zhang2018attention} \cite{zhang2018adding}, RADAR \cite{zhang2018attention}, remote sensing data \cite{xiangrong_zhang;xin_wang;xu_tang;huiyu_zhou;chen_li_description_2019} \cite{bei_fang;ying_li;haokui_zhang;jonathan_cheung-wai_chan_hyperspectral_2019} \cite{qi_wang;shaoteng_liu;jocelyn_chanussot;xuelong_li_scene_2019} \cite{xiaoguang_mei;erting_pan;yong_ma;xiaobing_dai;jun_huang;fan_fan;qinglei_du;hong_zheng;jiayi_ma_spectral-spatial_2019}, audio-video \cite{hori_attention-based_2017} \cite{zhang2019deep}, and diverse sensors \cite{zadeh2018memory} \cite{zadeh2018multi} \cite{santoro2018relational}, as shown in Figure \ref{fig:modalities}.   

\begin{figure*}[htb]
    \centering
    \includegraphics[clip, trim=0.3cm 6cm 0.5cm 6cm, width=1.00\textwidth]{img/modalidades_ultimo_editado.pdf}
    \caption{A diagram showing sensory modalities of neural attention models. Radial segments correspond to attention architectures, and each track corresponds to a modality. Modalities are: (A) audio, (B) biomedical signals, (I) image, (O) other sensors, (L) LiDAR, (R) remote sensing data, (T) text, and (V) video. The following coloring convention is used for the individual segments: white (the modality is not implemented), light yellow (CNN), light orange (RNN), orange (Self-attentive networks), red (Memory networks), dark red (framework), and brown (GNN). This diagram emphasizes multimodal architectures so that only the most representative single modality (i.e., text or image) architectures are shown. Most multimodal architectures use the image/text or video/text modalities.}
    \label{fig:modalities}
\end{figure*}

Zhang et al. \cite{zheng_zhang;lizi_liao;minlie_huang;xiaoyan_zhu;tat-seng_chua_neural_2019} used an adaptive attention mechanism to learn to emphasize different visual and textual sources for dialogue systems for fashion retail. An adaptive attention scheme
automatically decided the evidence source for tracking dialogue states
 based on visual and textual context. \textbf{Dual Attention Networks} \cite{nam_dual_2017} presented attention mechanisms to capture the fine-grained interplay between images and textual information. The mechanism allows visual and textual attention to guide each other during collaborative inference. \textbf{HATT} \cite{wu_hierarchical_2018} presented a new attention-based hierarchical fusion to explore the complementary features of multimodal features progressively, fusing temporal, motion, audio, and semantic label features for video representation. The model consists of three attention layers. First, the low-level attention layer deals with temporal, motion, and audio features inside each modality and across modalities. Second, high-level attention selectively focuses on semantic label features. Finally, the sequential attention layer incorporates hidden information generated by encoded low-level attention and high-level attention. Hori et. al. \cite{hori_attention-based_2017} extended simple attention multimodal fusion. Unlike the simple multimodal fusion method, the feature-level attention weights can change according to the decoder state and the context vectors, enabling the decoder network to pay attention to a different set of features or modalities when predicting each subsequent word in the description. Memory Fusion Network \cite{zadeh2018memory} presented the Delta-memory Attention module for multi-view sequential learning. First, an LSTM system, one for each of the modalities, encodes the modality-specific dynamics and interactions. Delta-memory attention discovers both cross-modality and temporal interactions in different memory dimensions of LSTMs. Finally, Multi-view Gated Memory (unifying memory) stores the cross-modality interactions over time.

Huang et al. \cite{noauthor_bi-directional_nodate} investigated the problem of matching image-text by exploiting the bi-directional attention with fine-granularity correlations between visual regions and textual words. \textbf{Bi-directional attention} connects the word to regions and objects to words for learning mage-text matching. Li et. al. \cite{yehao_li;ting_yao;yingwei_pan;hongyang_chao;tao_mei_pointing_2019} introduced \textbf{Long Short-Term Memory with Pointing} (LSTM-P) inspired by humans pointing behavior \cite{matthews2012origins}, and Pointer Networks \cite{vinyals2015pointer}. The pointing mechanism encapsulates dynamic contextual information (current input word and LSTM cell output) to deal with the image captioning scenario's novel objects. Liu et. al. \cite{noauthor_improving_nodate} proposed a cross-modal attention-guided erasing approach for referring expressions. Previous attention models focus on only the most dominant features of both modalities and neglect textual-visual correspondences between images and referring expressions. To tackle this issue, cross-modal attention discards the most dominant information from either textual or visual domains to generate difficult training samples and drive the model to discover complementary textual-visual correspondences. Abolghasemi et al. \cite{pay_attention} demonstrated an approach for augmenting a deep visuomotor policy trained through demonstrations with \textbf{Task Focused Visual Attention} (TFA). Attention receives as input a manipulation task specified in natural language text, an image with the environment, and returns as output the area with an object that the robot needs to manipulate. TFA allows the policy to be significantly more robust from the baseline policy, i.e., no visual attention. Pu et al. \cite{pu_adaptive_2018} adaptively select features from the multiple CNN layers for video captioning. Previous models often use the output from a specific layer of a CNN as video features. However, this attention model adaptively and sequentially focuses on different layers of CNN features.

\subsection{Attention-augmented memory}
\label{sub:attention_memory}

Attentional interfaces also allow the neural network iteration with other cognitive elements (i.e., memories, working memory). Memory control and logic flow are essential for learning. However, they are elements that do not exist in classical architectures. The memory of classic RNNs, encoded by hidden states and weights, is usually minimal and is not sufficient to remember facts from the past accurately. Most Deep Learning models do not have a simple way to read and write data to an external memory component. The \textbf{Neural Turing Machine} (NTM) \cite{graves_neural_2014} and Memory Networks (MemNN) \cite{weston_2014_memory} - a new class of neural networks - introduced the possibility for a neural network dealing with addressable memory. NTM is a differentiable approach that can be trained with gradient descent algorithms, producing a practical learning program mechanism. NTM memory is a short-term storage space for information with its rules-based manipulation. Computationally, these rules are simple programs, where data are those programs' arguments. Therefore, an NTM resembles a working memory designed to solve tasks that require rules, where variables are quickly linked to memory slots. NTMs use an attentive process to read and write elements to memory selectively. This attentional mechanism makes the network learn to use working memory instead of implementing a fixed set of symbolic data rules.

\textbf{Memory Networks} \cite{weston_2014_memory} are a relatively new framework of models designed to alleviate the problem of learning long-term dependencies in sequential data by providing an explicit memory representation for each token in the sequence. Instead of forgetting the past, Memory Networks explicitly consider the input history, with a dedicated vector representation for each history element, effectively removing the chance to forget. The limit on memory size becomes a hyper-parameter to tune, rather than an intrinsic limitation of the model itself. This model was used in question-answering tasks where the long-term memory effectively acts as a (dynamic) knowledge base, and the output is a textual response. Large-scale question-answer tests were performed, and the reasoning power of memory networks that answer questions that require an in-depth analysis of verb intent was demonstrated. Mainly due to the success of MemNN, networks with external memory are a growing research direction in DL, with several branches under development as shown in figure \ref{fig:memory_networks_family}.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{img/memory_networks_family.pdf}
  \caption{Memory-based neural networks (MemNN). Architectures labels are color-coded as follows: orange - natural language processing, red - computer vision, purple - others. The end-to-End Memory networks is the first end-to-end differentiable version of MemNN. GMN \cite{khasahmadi2020memory} and MemGNN \cite{khasahmadi2020memory} are the first graph networks with memory. DMN \cite{xiong_dynamic_2016}, MemGNN \cite{khasahmadi2020memory}, Episodic graph memory networks \cite{lu2020video}, Episodic CAMN \cite{abdulnabi2017episodic}, are the first instances of the episodic memory framework.}
  \label{fig:memory_networks_family}
\end{figure}


\textbf{End-to-end Memory Networks} \cite{sukhbaatar2015end} is the first version of MemNN applicable to realistic, trainable end-to-end scenarios, which requires low supervision during training. Aug Oh. et al. \cite{oh2019video} extends Memory Networks to suit the task of semi-supervised segmentation of video objects. Frames with object masks are placed in memory, and a frame to be segmented acts as a query. The memory is updated with the new masks provided and faces challenges such as changes, occlusions, and accumulations of errors without online learning. The algorithm acts as an attentional space-time system calculating when and where to meet each query pixel to decide whether the pixel belongs to a foreground object or not. Kumar et al. \cite{kumar_ask_2015} propose the first network with episodic memory - a type of memory extremely relevant to humans - to iterate over representations emitted by the input module updating its internal state through an attentional interface. In \cite{lu2020video}, an episodic memory with a key-value retrieval mechanism chooses which parts of the input to focus on thorough attention. The module then produces a summary representation of the memory, taking into account the query and the stored memory. Finally, the latest research has invested in Graph Memory Networks (GMN), which are memories in GNNs \cite{wu2020comprehensive}, to better handle unstructured data using key-value structured memories \cite{miller2016key} \cite{khasahmadi2020memory} \cite{khasahmadi2020memory} \cite{moon2019memory}.


\subsection{End-to-end attention models}
\label{sub:end_to_end_attention_models}
% Falar que em meados de 2017 a comunidade cientifica percebeu que a atenção como uma simples interface poderia ser melhorado.
In mid-2017, research aiming at end-to-end attention models appeared in the area. The Neural Transformer (NT) \cite{vaswani_attention_2017} and Graph Attention Networks \cite{velickovic_graph_2018} - purely attentional architectures - demonstrated to the scientific community that attention is a key element for the future development in Deep Learning. The Transformer's goal is to use self-attention (Section \ref{sub:attention_mechanisms}) to minimize traditional recurrent neural networks' difficulties. The \textbf{Neural Transformer} is the first neural architecture that uses only attentional modules and fully-connected neural networks to process sequential data successfully. It dispenses recurrences and convolutions, capturing the relationship between the sequence elements regardless of their distance. Attention allows the Transformer to be simple, parallelizable, and low training cost \cite{vaswani_attention_2017}. \textbf{Graph Attention Networks} (GATs) are an end-to-end attention version of GNNs \cite{wu2020comprehensive}. They have stacks of attentional layers that help the model focus on the unstructured data's most relevant parts to make decisions. The main purpose of attention is to avoid noisy parts of the graph by improving the signal-to-noise ratio (SNR) while also reducing the structure's complexity. Furthermore, they provide a more interpretable structure for solving the problem. For example, when analyzing the Attention of a model under different components in a graph, it is possible to identify the main factors contributing to achieving a particular response condition.

There is a growing interest in NT and GATs, and some extensions have been proposed \cite{wang2019heterogeneous} \cite{wang2019graph} \cite{abu2018watch} \cite{li2019relation}, with numerous Transformer-based architectures as shown figure \ref{fig:transformer_family}. These architectures and all that use self-attention belong to a new category of neural networks, called Self-Attentive Neural Networks. They aim to explore self-attention in various tasks and improve the following drawbacks: 1) a Large number of parameters and training iterations to converge; 2) High memory cost per layer and quadratic growth of memory according to sequence length; 3) Auto-regressive model; 4) Low parallelization in the decoder layers. Specifically, Weighted Transformer \cite{weighted_transformer} proposes modifications in the attention layers achieving a 40 \% faster convergence. The multi-head attention modules are replaced by modules called branched attention that the model learns to match during the training process. The Star-transformer \cite{qipeng_guo;xipeng_qiu;pengfei_liu;yunfan_shao;xiangyang_xue;zheng_zhang_star-transformer_2019} proposes a lightweight alternative to reduce the model's complexity with a star-shaped topology. To reduce the cost of memory, Music Transformer \cite{music_transformer}, and Sparse Transformer \cite{rewon_child;scott_gray;alec_radford;ilya_sutskever_generating_2019} introduces relative self-attention and factored self-attention, respectively. Lee et al. \cite{lee2018set} also features an attention mechanism that reduces self-attention from quadratic to linear, allowing scaling for high inputs and data sets.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.45\textwidth]{img/Transformer_family.pdf}
  \caption{Transformer-based neural networks. Architectures labels are color-coded as follows: orange - natural language processing, red - computer vision, purple - others.}
  \label{fig:transformer_family}
\end{figure}

Some approaches adapt the Transformer to new applications and areas. In natural language processing, several new architectures have emerged, mainly in multimodal learning. Doubly Attentive Transformer \cite{doubly_attentive_transformer} proposes a multimodal machine-translation method, incorporating visual information. It modifies the attentional decoder, allowing textual features from a pre-trained CNN encoder and visual features. The Multi-source Transformer \cite{multi_source_transformer} explores four different strategies for combining input into the multi-head attention decoder layer for multimodal translation. Style Transformer \cite{style_transformer}, Hierarchical Transformer \cite{hierarchical_transformer}, HighWay Recurrent Transformer \cite {highway_transformer}, Lattice-Based Transformer \cite {lattice_transformer}, Transformer TTS Network \cite {li2019neural}, Phrase-Based Attention \cite{phrase_attention} are some important architectures in style transfer, document summarization and machine translation. Transfer Learning in NLP is one of Transformer's major contribution areas. BERT \cite{devlin_bert:_2018}, GPT-2 \cite{radford2019language}, and GPT-3 \cite{brown2020language} based NT architecture to solve the problem of Transfer Learning in NLP because current techniques restrict the power of pre-trained representations. In computer vision, the generation of images is one of the Transformer's great news. Image Transformer \cite{parmar2018image}, SAGAN \cite{zhang2018self}, and Image GPT \cite{chen2020generative} uses self-attention mechanism to attend the local neighborhoods. The size of the images that the model can process in practice significantly increases, despite maintaining significantly larger receptive fields per layer than the typical convolutional neural networks. Recently, at the beginning of 2021, OpenAi introduced the scientific community to DALL·E \cite{unpublished2021dalle}, the Newest language model based on Transformer and GPT-3, capable of generating images from texts extending the knowledge of GPT-3 for viewing with only 12 billions of parameters.





\subsection{Attention today}
\label{sub:attention_today}


Currently, hybrid models that employ the main key developments in attention's use in Deep Learning (Figure \ref{fig:timeline}) have aroused the scientific community's interest. Mainly, hybrid models based on Transformer, GATs, and Memory Networks have emerged for multimodal learning and several other application domains. Hyperbolic Attention Networks (HAN) \cite{gulcehre_hyperbolic_2018}, Hyperbolic Graph Attention Networks (GHN) \cite{zhang2019hyperbolic}, Temporal Graph Networks (TGN) \cite{rossi2020temporal} and Memory-based Graph Networks (MGN) \cite{khasahmadi2020memory} are some of the most promising developments. Hyperbolic networks are a new class of architecture that combine the benefits of self-attention, memory, graphs, and hyperbolic geometry in activating neural networks to reason with high capacity over embeddings produced by deep neural networks. Since 2019 these networks have stood out as a new research branch because they represent state-of-the-art generalization on neural machine
translation, learning on graphs, and visual question answering tasks while keeping the neural representations compact. Since 2019, GATs have also received much attention due to their ability to learn complex relationships or interactions in a wide spectrum of problems ranging from biology, particle physics, social networks to recommendation systems. To improve the representation of nodes and expand the capacity of GATs to deal with data of a dynamic nature (i.e. evolving features or connectivity over time), architectures that combine memory modules and the temporal dimension, like MGNs and TGNs, were proposed.
 

\begin{figure*}[h]
 \centering
 \includegraphics[width=\textwidth]{img/main_architecture.pdf}
 \caption{Key developments in Attention in DL Timeline. RNNSearch presented the first attention mechanism. Neural Turing machine and Memory networks introduced memory and dynamic flow control. RAM and DRAW learned to combine multi-glimpse, visual attention, and sequential processing. Spatial Transformer introduced a module to increase the robustness of CNNs to variations in spatial transformations. Show, attend and tell created attention for multimodality. The Pointer network used attention as a pointer. BiDAF, HAN, and DCN presented attentional techniques to align data with different hierarchical levels. ACT introduced the computation time topic. Transformer \cite{vaswani_attention_2017} was the first self-attentive neural network with an end-to-end attention approach. GATs introduced attention in GNNs. BERT \cite{devlin_bert:_2018}, GPT-2 \cite{radford2019language}, GPT-3 \cite{brown2020language}, and DALL·E \cite{unpublished2021dalle} are the state-of-the-art in language models and text-to-image generation. Finally, BRIMs \cite{mittal2020learning} learned to combine bottom-up and top-down signals.}
 \label{fig:timeline}
\end{figure*}


At the end of 2020, two research branches still little explored in the literature were strengthened: 1) explicit combination of bottom-up and top-down stimuli in bidirectional recurrent neural networks and 2) adaptive computation time. Classic recurrent neural networks perform recurring iteration within a particular level of representation instead of using a top-down iteration, in which higher levels act at lower levels. However, Mittal et al. \cite{mittal2020learning} revisited the bidirectional recurrent layers with attentional mechanisms to explicitly route the flow of bottom-up and top-down information, promoting selection iteration between the two levels of stimuli. The approach separates the hidden state into several modules so that upward iterations between bottom-up and top-down signals can be appropriately focused. The layer structure has concurrent modules so that each hierarchical layer can send information both in the bottom-up and top-down directions.

The adaptive computation time is an interesting little-explored topic in the literature that began to expand only in 2020 despite initial studies emerging in 2017. ACT applies to different neural networks (e.g. RNNs, CNNs, LSTMs, Transformers). The general idea is that some complex data might require more computation to produce a final result, while some unimportant or straightforward data might require less. The attention mechanism dynamically decides how long to process network training data. The seminal approach by Graves et al. \cite{graves_adaptive_2016} made minor modifications to an RNN, allowing the network to perform a variable number of state transitions and a variable number of outputs at each stage of the input. The resulting output is a weighted sum of the intermediate outputs, i.e., soft attention. A halting unit decides when the network should stop or continue. To limit computation time, attention adds a time penalty to the cost function by preventing the network from processing data for unnecessary amounts of time. This approach has recently been updated and expanded to other architectures. Spatially Adaptive Computation Time (SACT) \cite{figurnov2017spatially} adapts ACT to adjust the per-position amount of computation to each spatial position of the block in convolutional layers, learning to focus computing on the regions of interest and to stop when the features maps are "good enough". Finally, Differentiable Adaptive Computation Time (DACT) \cite{eyzaguirre2020differentiable} introduced the first differentiable end-to-end approach to computation time on recurring networks.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

